On Scheduling Ring-All-Reduce Learning Jobs in Multi-Tenant GPU Clusters with Communication Contention

Powered by advances in deep learning (DL) techniques, machine learning and artificial intelligence have achieved astonishing successes. However, the rapidly growing needs for DL also led to communication- and resource-intensive distributed training jobs for large-scale DL training, which are typically deployed over GPU clusters. To sustain the ever-increasing demand for DL training, the so-called "ring-all-reduce" (RAR) technologies have recently emerged as a favorable computing architecture to efficiently process network communication and computation load in GPU clusters. The most salient feature of RAR is that it removes the need for dedicated parameter servers, thus alleviating the potential communication bottleneck. However, when multiple RAR-based DL training jobs are deployed over GPU clusters, communication bottlenecks could still occur due to contentions between DL training jobs. So far, there remains a lack of theoretical understanding on how to design contention-aware resource scheduling algorithms for RAR-based DL training jobs, which motivates us to fill this gap in this work. Our main contributions are three-fold: i) We develop a new analytical model that characterizes both communication overhead related to the worker distribution of the job and communication contention related to the co-location of different jobs; ii) Based on the proposed analytical model, we formulate the problem as a non-convex integer program to minimize the makespan of all RAR-based DL training jobs. To address the unique structure in this problem that is not amenable for optimization algorithm design, we reformulate the problem into an integer linear program that enables provable approximation algorithm design called SJF-BCO (Smallest Job First with Balanced Contention and Overhead); and iii) We conduct extensive experiments to show the superiority of SJF-BCO over existing schedulers.

==> MobiHoc'22_Communication_Contention_Tech_Report/Abstract/Abstract.tex <==
% !TEX root = ../Communication_Contention_MobiHoc22.tex

\begin{abstract}
Powered by advances in deep learning (DL) techniques, machine learning and artificial intelligence have achieved astonishing successes.
However, the rapidly growing needs for DL also led to communication- and resource-intensive distributed training jobs for large-scale DL training, which are typically deployed over GPU clusters.
To sustain the ever-increasing demand for DL training, the so-called ``ring-all-reduce'' (RAR) technologies have recently emerged as a favorable computing architecture to efficiently process network communication and computation load in GPU clusters.
The most salient feature of RAR is that it removes the need for dedicated parameter servers, thus alleviating the potential communication bottleneck.
However, when multiple RAR-based DL training jobs are deployed over GPU clusters, communication bottlenecks could still occur due to contentions between DL training jobs. 
So far, there remains a lack of theoretical understanding on how to design contention-aware resource scheduling algorithms for RAR-based DL training jobs, which motivates us to fill this gap in this work.
Our main contributions are three-fold: i) We develop a new analytical model that characterizes both communication overhead related to the worker distribution of the job and communication contention related to the co-location of different jobs; 
ii) Based on the proposed analytical model, we formulate the problem as a non-convex integer program to minimize the makespan of all RAR-based DL training jobs.
To address the unique structure in this problem that is not amenable for optimization algorithm design, we reformulate the problem into an integer linear program that enables provable approximation algorithm design called SJF-BCO (\ul{S}mallest \ul{J}ob \ul{F}irst with \ul{B}alanced \ul{C}ontention and \ul{O}verhead); 
and iii) We conduct extensive experiments to show the superiority of SJF-BCO over existing schedulers.
Collectively, our results contribute to the state-of-the-art of distributed GPU system optimization and algorithm design.
\end{abstract}





==> MobiHoc'22_Communication_Contention_Tech_Report/Appdx_A/Appdx_A.tex <==
% !TEX root = ../ML_Networking_INFOCOM'22.tex
\subsection{Extensions to More Advanced Models}\label{sec:extension}

\begin{figure}[t!]
    \centering
%    \includegraphics[width=0.45\textwidth]{Figures/fig_communication_task.eps}
    \includegraphics[width=0.48\textwidth]{Figures/fig_models_example.eps}
    \caption{A three-layer example of model comparison.}
    \label{fig:comparison}
\end{figure}

%It is worth noting that our work focus on the ``sequential model", i.e., communication and computation are performed in order (See Fig.~\ref{fig:comparison}(a)).
Recall that Eqn.~(\ref{contention_model}) is calculated based on ``sequential model''~\cite{Zhang17:Poseidon} (See Fig.~\ref{fig:comparison}(a)), where communication starts after BP of all layers are done, the RAR is done sequentially from the last layer to the first layer, followed by and FP of the next iteration.
We let $L[j]$ denote the number of layers in DNN model of job $j$.
We use $t_l^c[j]$ to denote the time spent for RAR for layer $l$ of job $j$.
Let $t_l^b[j]$ and $t_l^f[j]$ be the BP and FP computation times for layer $l$ of job $j$, respectively.
We also use $\psi_l[j]$ to denote the start time of gradients communication for layer $l$ of job $j$.
Let $\varphi_l[j]$ be the start time of FP for layer $l$ of job $j$.
For lighter notation, we will omit the job index ``[j]'' in the following derivations.
It is easy to see that the per-iteration training time $t$ for the sequential model can be computed as:
\begin{align*}
t = \sum_{l=1}^L t_l^b + \sum_{l=1}^Lt_l^c + \sum_{l=1}^Lt_l^f.
\end{align*}
%We let $t^b\triangleq\sum_{l=1}^Lt_l^b$, $t^c \triangleq \sum_{l=1}^Lt_l^c$, and $t^f\triangleq\sum_{l=1}^Lt_l^f$.
Note that the key feature of the sequential model is that computation phases (i.e., BP and FP) and communication phase are conducted in a {\it sequential} fashion, which underutilizes the channel.
Thus, more advanced models are proposed to further reduce the training time.
Following the similar method in~\cite{Yu21:INFOCOM}, we could also derive a unified analytical model to characterize all these models based on RAR architecture.

%The sequential model~\cite{} is illustrated in Fig.~\ref{fig:comparison}(a), 
The wait-free model~\cite{Zhang17:Poseidon} as shown in Fig.~\ref{fig:comparison}(b), starting from the final layer, each layer takes turn to conduct RAR after finishing its own BP and the completion of gradient communication of its subsequent layer.
Compared to the sequential model, a key feature in this model is that part of the RAR and computation can be conducted {\it simultaneously}.
We derive per-iteration training time $t$ as follows:
\[
    \psi_l = 
\begin{cases}
    t_L^b,& \text{if } l=L\\
    \max\{\sum_{k=l}^L t_k^b, \psi_{l+1} + t_{l+1}^c\},              & \text{otherwise}
\end{cases}
\]

\[
    \varphi_l = 
\begin{cases}
    \psi_1 + t_1^c,& \text{if } l=1\\
    \varphi_{l-1} + t_{l-1}^f,              & \text{otherwise}
\end{cases}
\]
It thus follows that the per-iteration training time is $t=\varphi_L + t_L^f$.

Note that: 1) If the parameter size is skewed in the wait-free model, layers of larger sizes can introduce larger delay to layers of smaller sizes due to non-preemption. 
2) In the wait-free model, only after gradients communication for the first layer, the FP of the next iteration can get started; thus the gradients exchange of the subsequent layers causes delays to the gradient exchange of the initial layer, which in turn induces delay for the next iteration. 
Also, since the BP progresses in the reverse order of layers (i.e., from the last layer to the first layer), the gradients are also generated and sent in that order. 
As a result, no overlap between computation and RAR is possible during FP (see Fig.~\ref{fig:comparison}(b)).

An insight from the discussions above is that the closer a layer is to the input layer, the higher priority its gradient communication should have. 
The reason is that once the transmission of this layer is completed, the corresponding FP of this layer can start without waiting for all communications to be finished, thus
significantly reducing delay. 
In the priority-based model~\cite{Jayarajan19:P3}, as shown in Fig.~\ref{fig:comparison}(c), the layer with a smaller index (i.e., closer to the input layer) always has a higher priority and its communication can preempt that of layers with larger indices. 
This induces further RAR-computation overlapping and helps the next iteration get started as soon as possible.
%We let $\sigma_l[j]$ be the end time of communication for layer $l$ of job $j$.
We derive the per-iteration training time $t$ as follows:
\[
    \varphi_l = 
\begin{cases}
    t_1^c + \sum_{k=1}^Lt_k^b,& \text{if } l=1\\
    \max\{\varphi_{l-1} + t_{l-1}^f, \sum_{k=l}^Lt_k^b + \sum_{k=1}^lt_k^c\},              & \text{otherwise}
\end{cases}
\]
It thus follows that the per-iteration training time is $t=\varphi_L + t_L^f$.

Note that $t$ has a recursive property. 
Depending on whether the system is computation or communication dominant in each layer, the per-iteration training time could lead to different expressions.

Next, we derive the unified expression for per-iteration training time.
Note that, in both wait-free and priority-based model, the per-iteration training time $t$ is DNN-dependent and determined by each layer’s size. 
Nonetheless, as long as the DNN of a training job is given, we can compute t by using the recursion formulas. 
Also, we note that the communication-computation overlapping in wait-free and priority-based models effectively reduces the BP time, communication time, and FP time to certain fractions of those in the sequential model. 
Thus, the per-iteration training time of all models can be expressed as $t=\eta_1t^f + \eta_2t^b + \eta_3t^c$, where the coefficients $\eta_1$, $\eta_2$, $\eta_3\in(0,1]$ are DNN-model-dependent.


We let $H^f$, $H^b$, $H^c$ be the FP time, BP time and RAR time for processing a sample, respectively.
Then these coefficients are defined as $\eta_1\triangleq\frac{H^f}{\sum_{l=1}^Lt_l^f}$, $\eta_2\triangleq\frac{H^b}{\sum_{l=1}^Lt_l^b}$, and $\eta_3\triangleq\frac{H^c}{\sum_{l=1}^Lt_l^c}$.
For example, for the wait-free instance in Fig.~\ref{fig:comparison}(b), we can compute the coefficients as $\eta_1=\frac{\sum_{l=1}^3t_l^f}{\sum_{l=1}^3t_l^f}=1$, $\eta_2=\frac{t_3^b}{\sum_{l=1}^3t_l^b}<1$, and $\eta_3=\frac{\sum_{l=1}^3t_l^c}{\sum_{l=1}^3t_l^c}=1$.

In other words, Eqn.~(\ref{contention_model}) can be generalized to these advanced models by introducing some coefficients that used to capture the overlap properties.
%Here, to make this paper self-contained, we give a simple derivation for a model with $L$ layers.
%We use the subscript $l$ to indicate the gradient/parameter size at layer $l$.
%More details can be found in~\cite{Yu21:INFOCOM}.
The per-iteration training time according to Eqn.~(\ref{contention_model}) is:

\begin{align*}
\tau &= \frac{\frac{m}{w}\cdot2(w-1)}{b/f(\boldsymbol{\alpha}, k)}+\frac{\frac{m}{w}\cdot(w-1)}{C}+\gamma(\y)+ t^fM +t^b\\
&= \frac{\frac{\sum_{l=1}^Lm_l}{w}\cdot2(w\!-\!1)}{b/f(\boldsymbol{\alpha}, k)}+\frac{\frac{\sum_{l=1}^Lm_l}{w}\cdot(w\!-\!1)}{C}+\gamma(\y)+ \sum_{l=1}^L(t_l^f +t_l^b)\\
&=\sum_{l=1}^L\bigg(\underbrace{t_l^f}_{\text{FP}} + \underbrace{t_l^b}_{\text{BP}} + \underbrace{\frac{m_l (w-1)}{w\cdot C} + \frac{2m_l(w-1)f(\boldsymbol{\alpha}, k)}{w\cdot b}}_{\text{RAR: $t_l^c$}}\bigg)+\gamma(\y)\\
&= \eta_1t^fM + \eta_2t^b+\eta_3\bigg(\frac{\frac{m}{w}\cdot(w-1)}{C} + \frac{\frac{m}{w}\cdot2(w-1)}{b/f(\boldsymbol{\alpha}, k)}\bigg)+ \gamma(\y),
\end{align*}
where $\eta_1, \eta_2, \eta_3 \in(0, 1]$, are DNN model dependent.
Note that the sequential model is a special case with $\eta_1 = 1$, $\eta_2 = 1$ and $\eta_3 = 1$.
%More details can be found in~\cite{Yu21:INFOCOM}.



==> MobiHoc'22_Communication_Contention_Tech_Report/Appdx_B/Appdx_B.tex <==
% !TEX root = ../ML_Networking_INFOCOM'20.tex

\section{Proof Sketch of Theorem~\ref{thm_Competitive}} \label{appdx:thm_Competitive}

Due to space limitation, we provide a proof sketch for Theorem~\ref{thm_Competitive} in here.
From Theorem~\ref{thm_Alg4}, we know that Algorithm~4 is a $\frac{3G}{\delta}$-approximate algorithm.
Then, by induction, we can show that the dynamic programming approach in Algorithm~3 is also a $\frac{3G}{\delta}$-approximate algorithm.


Now, let $\hat{\pi}_{i}$ denote the approximate schedule obtained by Algorithm~2, which inexactly solves Problem D-R-DMLRS.
Let $P_{i}$ and $D_{i}$ be the primal and dual objective values of Problems R-DMLRS and D-RMLRS after determining the schedule $\hat{\pi}_{i}$ in Algorithm~1.
Then, we have $P_{i} - P_{i-1} = u_{i}(\tilde{t}_{\hat{\pi}_{i}} - a_{i})$.
Let $\hat{\lambda}_{i}$ be the dual price that corresponds to $\hat{\pi}_{i}$.
% such that $\hat{\lambda}_{i} \geq u_{i}(\tilde{t}_{\hat{\pi}_{i}}-a_{i}) -\sum_{t\in\mathcal{T}(\hat{\pi}_{i})} \sum_{h\in\mathcal{H}(\hat{\pi}_{i}[t])} \sum_{r\in\mathcal{R}} (\alpha_{i}^{r} w_{ht}^{\hat{\pi}_{i}} + \beta_{i}^{r} s_{ht}^{\hat{\pi}_{i}})$.
Also, we let $\Theta^{*}(\tilde{t}_{\hat{\pi}_{i}}, V_{i})$ be the true minimum cost under $\tilde{t}_{\hat{\pi}_{i}}$.
Suppose that job $i$ is admitted, we then have $u_{i}(\tilde{t}_{\hat{\pi}_{i}}-a_{i}) - \frac{\delta}{3G}\Theta(\tilde{t}_{\hat{\pi}_{i}}, V_{i}) \geq u_{i}(\tilde{t}_{\hat{\pi}_{i}}-a_{i}) - \Theta^{*}(\tilde{t}_{\hat{\pi}_{i}}, V_{i}) \geq u_{i}(\tilde{t}_{\hat{\pi}_{i}}-a_{i}) - \Theta(\tilde{t}_{\hat{\pi}_{i}}, V_{i}) = \hat{\lambda}_{i}$,
which implies $u_{i}(\tilde{t}_{\hat{\pi}_{i}}-a_{i}) \geq \hat{\lambda}_{i} + \frac{\delta}{3G}\Theta(\tilde{t}_{\hat{\pi}_{i}}, V_{i})$.

Also, note that $D_{i} - D_{i-1} = \hat{\lambda}_{i} + \sum_{t} \sum_{h} \sum_{r} (p_{h}^{r,i}[t] - p_{h}^{r,i-1}[t]) C_{h}^{r}$.
Then, following similar arguments in \cite{Buchbinder09,Bao18:ML_INFOCOM}, we can show that the following allocation-cost relationship holds under price function (\ref{eqn_cost_update_fn}): $\Theta(\tilde{t}_{\hat{\pi}_{i}}, V_{i}) \geq \frac{\delta/3G}{\min_{r\in\mathcal{R}}(1,\ln\frac{U^r}{L})} \sum_{t} \sum_{h} \sum_{r} (p_{h}^{r,i}[t] \!\!-\!\! p_{h}^{r,i-1}[t]) C_{h}^{r}$, which further implies $P_{i} - P_{i-1} \geq \frac{\delta/3G}{\min_{r\in\mathcal{R}}(1,\ln\frac{U^r}{L})} (D_{i}-D_{i-1})$.
Then, by telescoping on $P_{i}-P_{i-1}$ from $1$ to $I$ and using weak duality with the fact that $D_{0} \leq \frac{1}{2}OPT$ (due to the choice of constant $L$ in the cost function), we reach the final competitive ratio in Theorem~\ref{thm_Competitive} and the proof is complete.




==> MobiHoc'22_Communication_Contention_Tech_Report/Sec1_Intro/Sec1_Intro.tex <==
% !TEX root = ../Communication_Contention_MobiHoc22.tex

\section{Introduction} \label{sec:intro}

%Paragraph1: Background and current state
{\bf Background and Motivation:} 
In recent years, the rise of deep learning has driven an ever-increasing need for large-scale distributed training in GPU clusters, which leverages massive parallelism to speed up the training processes.
This has been evidenced by the popularity of several prevailing distributed deep learning (DDL) frameworks (e.g., TensorFlow~\cite{TensorFlow} and PyTorch~\cite{Paszke19:PyTorch}).
%Distributed deep learning (DDL)~\cite{Dean12:DDL} with the data parallelism using synchronous stochastic descent (SGD) is typically adopted to expedite the training process.
%One of the widely utilized frameworks to support the data parallelism training is parameter-server architecture~\cite{Li14:parameter_server}.
In these DDL frameworks, the traditional and most widely adopted computing-networking structure is based on the sever-worker (SW) architecture, where DDL training jobs are decomposed into and executed in parallel by a set of workers under the coordination of a parameter server.
However, %as modern DDL training jobs becoming more complex and requiring more workers, 
as the number of workers increases, the SW architecture suffers from serious scalability limitations since the server acts as a communication bottleneck and a single-point-of-failure.
%
To address the scalability limitations of the SW architecture, the ring-all-reduce (RAR)~\cite{Patarasuk09:Ring-AllReduce} architecture has attracted increasing attention in recent years.
The key idea of RAR is that, by forming a ring and working collaboratively, the workers can update the learning model parameters {\em without} needing any parameter server, thus removing the communication bottleneck and alleviating the single point of failure.
Moreover, it can be shown that the RAR architecture enjoys the highly desirable ``bandwidth optimality'' in the sense that, as the number of workers increases, the amount of information exchanged in the network is asymptotically {\em independent} of the number of workers (see Section~\ref{sec:Preliminaries} for details). 

However, despite all these salient features, the performance of deploying RAR-based training jobs in {\em multi-tenant} GPU clusters remains far from being satisfactory in practice~\cite{Wang20:contention}.
The fundamental reason is that the bandwidth optimality of RAR architecture only happens when there is only a single training job in the system (i.e.,  a contention-free environment).
In a multi-tenant GPU cluster, however, such an ideal contention-free condition is rarely satisfied.
As a result, significant communication bottleneck links could occur when deploying RAR-based training jobs in the system.
For example, researchers in~\cite{Wang20:contention} have found that on a cluster of four-GPU servers connected by 10 Gbps Ethernet, when only one RAR training job is executed with four GPUs in the cluster, the job completion time is 295 seconds.
In comparison, when four jobs of the same type are executed simultaneously with each job still using four GPUs but scheduled across GPU servers, each job's completion time dramatically increases to 675 seconds due to the extensive communication contention.
These empirical performance results of RAR indicate that developing efficient and effective scheduling for RAR-based DDL training jobs is well warranted to mitigate contention-induced communication bottlenecks.
However, in the literature so far, there remains a lack of theoretical understanding on how to design contention-aware resource scheduling algorithms for RAR-based DDL training jobs.
In light of the rapidly growing importance of RAR-based DDL deployment, our goal in this paper is to fill this gap and develop contention-aware scheduling algorithms for RAR-based training jobs in multi-tenant GPU clusters.


%The utilization of powerful hardware accelerators (e.g., GPUs) contributes to the success of DDL.
%However, in contrast to the fast-evolving computing capability of hardware accelerators and the high transmission rate enabled by intra-server interconnect technique like NVLink~\cite{Foley17:NVLink}, the inter-node communication, typically connected by Ethernet, often becomes the system bottleneck~\cite{Zhang17:Poseidon,Shi18:DDL}.
%Further, if the resources (e.g., bandwidth) are shared among different DDL training jobs, the network contention will emerge and thus prolong the communication time~\cite{Jeon2018:multi-tenant}.
%As a result, the system performance with respect to training time and resource utilization can be greatly degraded.
%
%In order to reduce the training time, some existing works proposed efficient DDL training algorithms by overlapping the computation and communication~\cite{Jia18:imagenet,Shi19:MG-WFBP,Cho19:BlueConnect}, or conducting the model or gradient compression~\cite{Lin18:compression,Shi19:SGD}.
%However, due to the existence of communication contention from different jobs in a resource-shared cluster, the performance could be greatly undermined if the training jobs are not properly scheduled.


\smallskip
{\bf Technical Challenges:}
We note, however, that due to a number of technical difficulties, developing contention-aware scheduling algorithms for RAR-based DDL jobs in multi-tenant GPU clusters is highly challenging.
\emph{First and foremost}, just as any network optimization problems that deal with contentions and interferences, the completion time of an RAR-based training job depends not only on its resource allocation decisions (i.e., the number of ring-forming workers and their locality), but also on the number of {\em concurrent} RAR-based DDL jobs that (partially or completely) share the communication links of this job.
The complex communication coupling between concurrent RAR-based training jobs renders it {\em intractable} to compute the per-iteration execution time of an RAR-based DDL job in closed-form.
\emph{Second}, there exists a fundamental trade-off in terms of job locality.
On one hand, co-locating all workers of an RAR-based DDL job on the same server enjoys a faster intra-server communication speed, but could lead to resource fragmentation. %\textcolor{red}{since the job tends to open new servers to schedule its workers instead of fully utilizing shared servers' capacity}.
On the other hand, spreading the ring of an RAR job over multiple servers could also result in more contentions of communication links and overhead in establishing connections between servers.
\emph{Last but not least}, due to the resource constraints of each server and the iterative nature of DDL training workload, the resource allocation decision for each RAR-based training job is subject to a mix of packing and covering types of constraints, both of which are known to be NP-hard.

%Paragraph3: Contributions
\smallskip
{\bf Our Contributions:}
In this paper, we overcome the above challenges and design a suite of scheduling algorithmic techniques for efficient RAR-based DDL training in multi-tenant GPU clusters with theoretical makespan performance guarantees.
The key idea of our algorithmic design is to transfer the structural complexity of the intractable  per-iteration running evaluation in the original scheduling problem to the dimensional complexity of an equivalent reformulated problem, which has a much cleaner integer linear program structure to work with.
Our main results and technical contributions are summarized as follows:

%\vspace{-.1in}
\begin{list}{\labelitemi}{\leftmargin=1.5em \itemindent=-0.0em \itemsep=.2em}
\item We first propose a new analytical framework for RAR-based DDL training resource allocation and scheduling that characterizes both communication contention and overhead under the RAR architecture in a multi-tenant GPU cluster.
This analytical modeling serves as the foundation to enable us to formulate the scheduling optimization framework to minimize the makespan of all RAR-based training jobs.

\item As mentioned earlier, due to the complex resource contentions and couplings between RAR-based DDL jobs, it is intractable to determine the closed-form expression for the per-iteration execution time for each DDL job.
To address this challenge, we further reformulate the original problem into an equivalent integer problem, which has a cleaner problem structure.
Doing so allows us to convert the structural complexity of the original problem to the exponential dimensionality complexity in the reformulated problem, which is more amenable for low-complexity search-based optimization algorithm design.

\item Based on the above problem reformulation, we propose an efficient scheduling algorithm called SJF-BCO (\ul{s}mallest \ul{j}ob \ul{f}irst with \ul{b}alanced \ul{c}ontention and \ul{o}verhead) with theoretical approximation ratio guarantee.
%Our SJF-BCO algorithm contains two control parameter to balance between the contention and overhead and achieve .
We conduct extensive experiments to verify the performance of our proposed SJF-BCO algorithm and compare with existing scheduling policies to show the superiority of SJF-BCO over these baselines.
%Also, we inspect the impact of $\kappa$, $\lambda_j$ (see Alg.~\ref{alg:ff}) and contention level, i.e., increase the level by reducing the number of servers, on the makespan performance.
\end{list}
Collectively, our results contribute to a comprehensive and fundamental understanding of RAR-based DDL resource scheduling optimization.
The roadmap of the rest of the paper is as follows.
In Section~\ref{sec:Related}, we review the related literature.
Section~\ref{sec:Preliminaries} present preliminaries to familiar readers with the necessary background.
Section~\ref{sec:model_formulation} introduces the system model and problem formulation.
Section~\ref{sec:alg} demonstrates our algorithms and Section~\ref{sec:Performance} provides their performance analysis.
Section~\ref{sec:numerical} presents numerical results and Section~\ref{sec:conclusion} concludes this paper.




==> MobiHoc'22_Communication_Contention_Tech_Report/Sec2_Related/Sec2_Related.tex <==
% !TEX root = ../Communication_Contention_MobiHoc22.tex

\section{Related Work} \label{sec:Related}


As mentioned in Section~\ref{sec:intro}, DDL training job scheduling algorithms have received growing interest recently.
Research in this area aims to schedule DDL jobs and manage computing resources efficiently in multi-tenant GPU computing clusters.
Early attempts in this field were mostly heuristic approaches based on empirical observations and models to conduct the resource scheduling (e.g.,~\cite{Gu19:Tiresias,Mahajan20:Themis,Mei17:energy,Chau17:energy}). 
For example, Gandiva~\cite{Xiao18:Gandiva} considered GPU time-slicing and job scheduling by predicting DDL training jobs characteristics.
Optimus~\cite{Peng18:Optimus} leveraged performance models through online-fitting to guide the job scheduling aiming to minimize training completion time.
Rather than using prediction models, another line of research is to take advantage of the model-less data-riven learning methods for DDL job scheduling (e.g.,~\cite{Bao19:Harmony,Hu19:Spear,Wang20:Metis}).
For instance, Harmony~\cite{Bao19:Harmony}, a deep-reinforcement-learning-based  scheduler considered minimizing the job completion time.
Hu.~{\it et al.}~\cite{Hu19:Spear} designed a new scheduling framework called Spear to minimize the makespan of jobs by leveraging the deep reinforcement learning techniques.
%of complex jobs by considering the task dependencies and heterogeneous resource demands.
However, these works do not provide theoretical performance guarantee.
Also, none of these works considered RAR-based DDL job scheduling.

The most related work to this paper is GADGET~\cite{Yu22:GAGET}, which characterized RAR-based DDL job scheduling based on the assumption that the bandwidth of each job is reserved.
As a result, there is no need to consider communication contention in~\cite{Yu22:GAGET}. We note that a limitation of the reserved bandwidth assumption is that it could lead to resource under-utilization.
%since jobs that have large gradients to communicate are unable to borrow the bandwidth from jobs who are working on the computation.
In contrast, this paper considers communication contention to avoid this limitation.
This, however, renders the scheduling problem far more challenging.
Lastly, Wang et al.~\cite{Wang20:contention} also considered contention under various all-reduce architectures, including RAR.
However, they also relied on a system-dependent online-fitting model to predict the execution time and did not explicitly formulate any scheduling optimization problem.
Their solution was based on heuristics without theoretical performance guarantee.
In contrast, we develop an analytical model to facilitate the job scheduling as a rigorous optimization problem, which in turn entails approximation algorithm design with theoretical performance guarantee.

==> MobiHoc'22_Communication_Contention_Tech_Report/Sec3_Preliminaries/Sec3_Preliminaries.tex <==
% !TEX root = ../Communication_Contention_MobiHoc22.tex
\section{Ring-All-Reduce (RAR)-Based Distributed Learning: A Primer}\label{sec:Preliminaries}

In this section, we  provide a quick overview on the RAR-based distributed learning 
%and communication-contention-aware GPU performance modeling 
to familiarize readers with necessary background and fix the terminologies that are useful in the rest of the paper.

\begin{figure}[t!]
\includegraphics[width=.48\textwidth]{Figures/fig_rar_color.eps}
\caption{A three-worker illustrative example of the ring-all-reduce (RAR) process.}
\label{fig:ringallreduce}
\vspace{-.1in}
\end{figure}

%\subsection{Distributed Learning Training}

\smallskip
{\bf 1) SGD-Based Distributed Learning:}
The training of many ML problems is typically in the form of an empirical risk minimization (ERM) problem: $\min_{\w \in\mathbb{R}^d} \bar{L}(\w)\triangleq\frac{1}{P} \sum_{i=1}^{P} L(\w,\delta_i)$, where $\w$ contains the model parameters to be learned, $L(\w,\delta_i)$ is a loss function, 
%that evaluates the discrepancy between the output of a learning model (e.g., a deep neural network) and the ground truth of sample $\xi_i$, 
and $P$ is the total number of samples.
Due to the high-dimensionality and the large dataset size of many ERM problems (e.g., in deep learning), the stochastic gradient descent (SGD) method has become the most widely adopted method.
The SGD method can be written as the following iterative process: $\w_{k+1} = \w_k  -  (\eta_k/Q)\sum_{i\in\mathcal{Q}_k} \g_k^i$, where $\eta_k$ denotes the learning rate in the $k$-th iteration, $\mathcal{Q}_k$ represents the mini-batch in the $k$-th iteration with $|\mathcal{Q}_k| =Q$, and $\g_k^i$ is a stochastic gradient based on a random sample $\delta_i \in \mathcal{Q}_k$.
The finite-sum and mini-batch structure of SGD naturally lends itself to a {\em distributed} implementation in a $Q$-worker DDL system coordinated by a parameter server as follows:
First, the dataset is partitioned by $Q$ workers.
%Let $\mathcal{D}_j$ denote the $j$-th partition of the dataset trained by a worker $j\in \{1,\ldots,w\}$.
In each iteration $k$, each worker retrieves the current model parameters from the server and randomly draws a sample from its local dataset, and then computes a stochastic gradient (e.g., using the backpropagation method).
Then, all workers send their gradients to the server to be aggregated.


\smallskip
{\bf 2) The Ring-All-Reduce (RAR) Architecture:}
It can be seen from the above discussions that SGD-based distributed learning naturally implies a server-worker (SW) architecture.
However, as mentioned in Section~\ref{sec:intro}, the SW architecture suffers from scalability limitations as the number of workers increases.
This is because all workers need to communicate with the server, which creates a bottleneck.
Specifically, a $w$-worker SW system that solves a $d$-dimensional ERM problem requires $2wd$ amount of data exchange per iteration (each worker sends and receives a $d$-dimensional vectors per iteration), which scales {\em linearly} with respect to $w$.

To address this scalability limitation, the RAR~\cite{Patarasuk09:Ring-AllReduce} has been proposed to {\em remove the server}.
Under RAR, the workers form a ring to exchange and aggregate data collaboratively. %\textcolor{red}{without information exchange with the server.}
For a $w$-worker RAR system, each worker splits its stochastic gradient into $w$ sub-vectors (see Fig.~\ref{fig:ringallreduce} for an example with $w=3$).
Each iteration of RAR has $2(w-1)$ steps that can be divided into two phases.
In the first phase (steps $1,\ldots,w-1$), workers perform gradients reduction (i.e., summation), where each worker receives a gradient subvector from its upstream worker and sends its local reduction result to its downstream worker (Share-Reduce phase).
In the second phase (steps $w,\ldots,2w-2$), each worker circulates its resultant sub-vectors following the same token to obtain its final resultant gradients vector (Share-Only phase).
Since each worker sends $\frac{d}{w}$ amount of data for $2(w-1)$ times, the total amount of data any worker receives is $\frac{2d(w-1)}{w}$, which is asymptotically {\em independent} of $w$ as $w$ increases (also referred to as being {\em bandwidth-optimal} in the literature).














==> MobiHoc'22_Communication_Contention_Tech_Report/Sec4_Model/Sec4_Model.tex <==
% !TEX root = ../Communication_Contention_MobiHoc22.tex


\section{System Model and Problem Formulation} \label{sec:model_formulation}

In this section, we first introduce our system model in Section~\ref{subsec:sys_model} and then present the problem formulation for RAR-based DDL scheduling optimization in multi-tenant GPU clusters in Section~\ref{subsec:formulation}.


\subsection{System Model} \label{subsec:sys_model}


{\bf 1) Scheduling Model:}
Consider a multi-tenant GPU cluster that contains a set of servers $\mathcal{S}$.
Each server is equipped with a set of homogeneous (i.e., of equal computation speed) and synchronized GPUs.
The servers in $\mathcal{S}$ are connected by a network and the network topology can be modeled as a connected graph.
In the beginning of a scheduling horizon $\mathcal{T}$ of length $|\mathcal{T}| = T$ time-slots, there is a set of RAR-based DDL jobs $\mathcal{J}$ waiting to be scheduled for training over $\mathcal{T}$. 
Each job $j \in \mathcal{J}$ is associated with a number of GPUs $G_j$ and a total number of training iterations $F_j$ from its users, both of which are requested by its users.\footnote{In practice, to prevent spending excessively long time waiting for the training process of a DDL job to converge, a maximum number of training iterations is usually given.}

In this paper, we consider the ``gang-scheduling'' discipline that is widely adopted in practical large-scale GPU clusters~\cite{Mahajan20:Themis,Gu19:Tiresias,Wang20:contention}.
Under gang scheduling, all workers (i.e., GPUs) of an RAR-based DDL job should be allocated {\em simultaneously.}
Moreover, once a job is scheduled to start, all GPUs allocated for this job will run to the job's completion and no preemption/migration is allowed.\footnote{Besides the overhead and complication added for both software and hardware, it has been shown that  frequent job preemption and migration may lead to significant performance degradation~\cite{Gu19:Tiresias}.}
Upon the job's completion, the occupied resource will also be released simultaneously.
Each GPU can only be occupied by one worker of some job at any given time.
As shown in Fig.~\ref{fig:example}, the workers of a job can be allocated within a single server or across multiple servers, as long as there exists a path in the underlying network that connects these workers and forms a ring topology to perform the RAR process. 
Note that Fig.~\ref{fig:example}(a) allocates the workers in the same server for each job, thus having no communication overhead.
On the contrary, Fig.~\ref{fig:example}(b) allocates workers across different servers for each job, which introduces communication contention when the two jobs happen to perform RAR communication concurrently.

\begin{figure}[t!]
    \centering
%    \includegraphics[width=0.45\textwidth]{Figures/fig_communication_task.eps}
    \includegraphics[width=0.45\textwidth]{Figures/fig_example.eps}
    \caption{An example of worker placement.}
    \label{fig:example}
    \vspace{-.1in}
\end{figure}

In this system, the control decisions of the scheduler are: i) determine a feasible scheduling for all jobs in $\mathcal{J}$ subject to network resource capacity; and ii) determine each job's starting time.
Specifically, consider an RAR-based DDL job $j$ scheduled with $w_j$ workers and its gradient size is $m_j$.
Let $y_{js}[t] \in \mathbb{Z}^{+}$ denote the number of GPUs scheduled for job $j$ on server $s$ in time-slot $t \in \mathcal{T}$.
Then, a scheduling decision in time-slot $t$ can be fully defined by the vector $\y[t] \triangleq [y_{js}[t], \forall j, s]$.
Let $a_j=\arg\min_t\{y_{js}[t]>0, \forall s\}$ be the starting time of job $j$ (to be determined) by the scheduling and let $T_j$ be the resultant completion time of job $j$.
Let $\mathcal{J}[t]\triangleq\{j | t\in[a_j,T_j]\}$ represent the set of {\it active jobs} (jobs being executed) in time slot $t$.
Clearly, to satisfy the $G_j$ number of GPUs requested for job $j$ during its training time,
% and the allocated GPUs can be migrated throughout the entire training process,
we have:
\begin{align}
    %  \label{eqn:gpu}&\sum_{s\in\mathcal{S}}\sum_{g\in\mathcal{G}_j}y_{gs}^j[t] = G^j\cdot x_j, \quad\forall d_j \leq t\leq \hat{t}_j,j\in\mathcal{J}, \\
    \label{eqn:gpu}&\sum_{s\in\mathcal{S}}y_{js}[t] = G_j, \quad \forall j\in\mathcal{J}[t], t\in\mathcal{T}.
    %  \label{eqn:gang}&y_{gs}^j[t]=y_{gs}^j[t+1], \quad \forall d_j\leq t<\hat{t}_j, g\in\mathcal{G}_j, s\in\mathcal{S},  j\in\mathcal{J}.
\end{align}
%{\bf 2) Resource Constraint Modeling:}
%We use a binary variable $\chi_s[t]$ to indicate whether server $s$ is chosen to schedule GPUs in the current interval in time slot $t$.
Also, scheduling decisions $\y[t]$, $\forall t$ are subject to GPU resource constraints.
Let $O_s$ represent the GPU capacity of server $s$.
To ensure that the allocated GPUs do not exceed each server's limit, we have:
\begin{align}
    \label{eqn:cap}&\sum_{j\in\mathcal{J}[t]}y_{js}[t]\leq O_s, \quad\forall s\in\mathcal{S}, t\in\mathcal{T}.
\end{align}
Also, under the non-preemptive gang scheduling, we have:
\begin{align}
y_{js}[t] = y_{js}[t-1], \quad\forall s\in\mathcal{S}, j\in\mathcal{J}[t], a_j < t\leq T_j.
\end{align}
Finally, to ensure that no workers should be allocated for non-active jobs and positive integer number of workers should be assigned to active jobs, we have:
\begin{align}
&y_{js}[t] = 0, \quad \forall s\in\mathcal{S}, j\not\in\mathcal{J}[t], t\in\mathcal{T}, \\    
\label{eqn:int}&y_{js}[t]\in\mathbb{Z}^{++},  \quad \forall s\in\mathcal{S}, j\in\mathcal{J}[t], t\in\mathcal{T}.
\end{align}


\smallskip
{\bf 2) Communication Contention Modeling:} 
With the above scheduling model, we are now in a position to present our communication contention model.
We assume that no communication contention will be introduced if at most one server is used for the job.
For example, in Fig.~\ref{fig:example}(a), jobs 1 and 2 both use intra-server communication and does not incur any communication contention.
%while other jobs uses inter-connect communication since at least two servers are chosen to place their workers.
%In addition, no communication contention is introduced for Job 3 since no other jobs conduct inter-connect communication between server 1 and server 2.
By contrast, in Fig.~\ref{fig:example}(b), jobs 1 and 2 induce communication contention since they both compete for inter-server link bandwidth between servers 1 and 2.
%We define $k_j[t]$ as the maximum number of concurrent running communication tasks associated with job $j$ in time slot $t$.
We let $p_j[t]$ denote the largest number of concurrently running jobs that share an inter-server communication link with job $j$ in time slot $t$, which can be computed as:
\begin{align}
\label{eqn:p_j}p_j[t] &=\max_{s\in\mathcal{S}}\bigg\{\mathds{1}\{0<y_{js}[t]<G_j\}\sum_{j'\in\mathcal{J}[t]}\mathds{1}\{0\!<\!y_{j's}[t]<G_{j'}\}\bigg\}, \nonumber\\
&\hspace{1.7in}\forall j\in\mathcal{J}[t], t\in\mathcal{T}.
\end{align}
In \eqref{eqn:p_j}, the first term $\mathds{1}\{0<y_{js}[t]<G_j\}$ indicates that only active jobs using inter-server communication on server $s$ will be considered.
The second term $\sum_{j'\in\mathcal{J}[t]}\mathds{1}\{ 0<y_{j's}[t]<G_{j'}\}$ represents the number of different jobs that compete for  inter-server communication on server $s$.
%We use $\mathcal{J}[t]$ be the {\it active} job set in time slot $t$, which includes all jobs that are not completed by time slot $t$.
Since job $j$ may not be transmitting at all times (due to switching between communication and computation modes), we let $k_j[t]$ be the actual largest number of {\em contending} jobs on average with job $j$ in time-slot $t$, which can be assumed to be statistically linearly proportional to $p_j[t]$, i.e.,
\begin{align}
k_j[t] = \xi_1 p_j[t], \quad\forall j\in\mathcal{J}[t], t\in\mathcal{T},
\end{align}
where $\xi_1\in(0,1]$ is a positive constant.

\smallskip
{\bf 3) RAR-Based DDL Training Completion Time Modeling:}
To evaluate the job completion time $T_j$ of job $j$, we need to first characterize the RAR training speed.
Note that the per-iteration RAR operation time of each DDL job can be decomposed into three parts: i) information exchange time, ii) computation time, and iii) communication overhead.
Next, we will model the operation time of each part individually.

\smallskip
{\em 2-1) Information Exchange Time:}
We use $B^{\{\omega_{j,1},\omega_{j,2}\}}(\mathbf{y}[t])$ to denote the bandwidth between two successive workers $\omega_{j,1}$ and $\omega_{j,2}$ in job $j$'s ring in time-slot $t$ under a scheduling decision $\y[t]$, where $\omega_{j,2}$ is the downstream worker of $\omega_{j,1}$.
Note that, unlike~\cite{Yu22:GAGET}, we do not reserve bandwidth for each job in this paper, and this bandwidth is determined by communication contention with other jobs under the scheduling decisions $\y[t]$ (see Fig.~\ref{fig:example}(b)).
We let $B_j(\y[t])\triangleq\min_{(\omega_{j,1},\omega_{j,2})\in\mathcal{L}_j} B^{\{\omega_{j,1},\omega_{j,2} \}}(\mathbf{y}[t])$ represent the bandwidth of the {\em bottleneck} link of job $j$ under scheduling decision $\y[t]$, where $\mathcal{L}_j$ is the set of all links  of job $j$.
Recall from Section~\ref{sec:Preliminaries} that the amount of information exchanged in each time-slot can be computed as $\frac{2m_j}{w_j}(w_j-1)$.
Thus, the number of time-slots for information exchange can be computed as $\frac{2m_j}{w_j}(w_j-1)/B_j(\y[t])$.

Clearly, the bottleneck link of job $j$ occurs in those links that are shared by the largest number of other concurrently running jobs.
We let $b^e$ and $b^i$ be the link bandwidth between and within servers, respectively, where $b^i\gg b^e$ in practice~\cite{Zhang17:Poseidon,Shi18:DDL}.
Recall that $k_j[t]$ denotes the actual {\it largest} number of contending jobs on average with job $j$ in time-slot $t$.
Ideally, each job on this bottleneck link has an equal share of bandwidth $b^e/k_j[t]$ under communication contention.
In practice, however, the bandwidth performance often degrades when multiple jobs compete for a link, which results in each job having less than $b^e/k_j[t]$ share of bandwidth if $k_j[t]\geq 2$~\cite{Wang20:contention}.
To model this effect, we use a function $f(\boldsymbol{\alpha}, k_j[t])$ to represent the ``bandwidth sharing degradation factor'' under communication contention, where $\boldsymbol{\alpha}\in\mathbb{R}^d$ captures all parameters that could lead to degradation.
We assume that $f(\boldsymbol{\alpha}, k_j[t])$ satisfies the following properties: i) $f(\boldsymbol{\alpha}, 1) = 1$ and ii) $f(\boldsymbol{\alpha}, k_j[t])$ is an increasing function of $k_j[t]$.
For example, if $f(\boldsymbol{\alpha}, k_j[t])$ is a linear function $k_j[t] + \alpha(k_j[t]-1)$, then $B_j(\y[t])= b^e/f(\boldsymbol{\alpha}, k_j[t])  = b^e/( k_j[t] + \alpha(k_j[t] -1))$.

Recall that in the special case where all workers of a job $j$ are co-located within a single server, there is no contention.
%there is no contention incurred.
%Recall that if all workers of the job are allocated within a server, we do not consider the contention.
Further, intra-server communication is typically enabled by fast interconnect techniques (e.g., NVLink~\cite{Foley17:NVLink}). 
Hence, we have $B_j(\y[t])=b^i$. %since there is no bottleneck link.


\smallskip
{\em 2-2) Computation Time:}
To characterize the computation time in the RAR operation, we use $C$ to denote the computational speed of a GPU unit (defined as the amount of data processed in each time-slot).
Since there are $\frac{m_j}{w_j}(w_j-1)$ amount of data for reduction in each RAR operation, the number of time-slots to complete all reductions can be computed as $\frac{m_j}{w_j}(w_j-1)/C$.
In addition to the all-reduce operation time, the computation time also includes the forward pass (FP) time and the backward pass (BP) time to compute a stochastic gradient.
We let $\Delta^f_j$ ($\Delta^b_j$) denote the duration of one FP (BP) of job $j$.
Note that the FP time is proportional to the mini-batch size $M_j$, which can be calculated as $\Delta^f_jM_j$ (the size of a mini-batch multiplied by the FP processing time of one sample).
Meanwhile, the BP time $\Delta^b_j$ is usually not relevant to the mini-batch size $M_j$ and is typically fixed.
Thus, the total number of time-slots for per-iteration computation can be computed as $\frac{m_j}{w_j}(w_j-1)/C + \Delta^f_jM_j + \Delta^b_j$.


\smallskip
{\em 2-3) Communication Overhead:}
In practice, it has been observed that typically, the more servers an RAR-based DDL job uses to perform the training, the larger the latency due to communication overhead (e.g., ACK time for message transmission, negotiation time among all workers before conducting all-reduce~\cite{Sergeev18:Horovod}) can be~\cite{Wang20:contention}.
In this paper, we use  $\gamma_j(\mathbf{y}_j[t])$ to denote the latency of job $j$ caused by communication overhead in time-slot $t$.
We assume that the latency is linear proportional to the number of servers in use, i.e., $\gamma_j(\y_j[t])=\xi_2\sum_s\mathds{1}\{y_{js}[t] > 0\}$, where $\y_j[t]= [y_{js}[t]>0, \forall s]$ and $\xi_2\in(0, 1]$ is a positive constant.

Lastly, putting 2-1) -- 2-3) together, we can compute the RAR operation time of job $j$ under  scheduling decision $\y[t]$ as follows:
%which is dependent on the placement $\mathbf{y}$.
%Particularly, the more number of servers the job uses, the larger the communication overhead will be.b/f(\boldsymbol{\alpha}, k_j[t])
\begin{align} \label{contention_model}
\!\!\! \tau_j[t] \!=\!\frac{\frac{m_j}{w_j}\cdot2(w_j\!-\!1)}{B_j(\y[t])}\!+\!\frac{\frac{m_j}{w_j}\cdot(w_j\!-\!1)}{C}\!+\!\gamma_j(\y_j[t])\!+\!\Delta^f_jM_j + \Delta^b_j.
\end{align}
%For notational compactness, we rewrite \eqref{contention_model} as $\tau_j[t] = \mathbf{h}\cdot\boldsymbol{\mathcal{F}}(k) + d + \gamma(\mathbf{y})$, where $\mathbf{h}\in\mathbb{R}^r$, $d\in\mathbb{R}$ are constants related to $m,w,\boldsymbol{\alpha}, C, M, \Delta^f_j, \Delta^b_j$, and $\boldsymbol{\mathcal{F}}(k)$ is a $r$-dimensional vector that each dimension is a mono-increasing function determined by $k_j[t]$. 
Hence, the RAR training speed $\phi_j[t]$ (i.e., the number of mini-batch iterations completed by job $j$) in time-slot $t$ can be computed as $\phi_j[t]\triangleq\lfloor (\tau_j[t])^{-1} \rfloor$.
% where $t'$ is the time duration for each time slot $t$ (e.g., 10 minutes).
Recall that $F_j$ is the requested number of iterations for training job $j$.
Thus, job $j$'s completion time can be calculated as:
\begin{align} \label{eqn:completion}
%\sum_{t\in\mathcal{T}_j}\frac{t'}{t_j[t]}=F_j, \quad \forall j\in\mathcal{J}.
T_j=a_j+\arg\min_t \big\{\sum\nolimits_{t\in\mathcal{T}}\phi_j[t]\geq F_j \big\}, \quad\forall j\in\mathcal{J}[t].
\end{align}


\subsection{Problem Statement} \label{subsec:formulation}
In this paper, our goal is to determine the scheduling decisions $\y[t]$ to minimize the makespan (i.e., $\max_j T_j$), which is one of the most useful metrics to measure the efficiency of multi-tenant GPU clusters~\cite{Grandl16:OSDI,Grandl16-2:OSDI}.
%Note that $a_j=\arg\min_t\{y_{js}[t]>0\}$, i.e., the decision variables are $y_{js}[t], \forall j, t, s$ in Problem~DDLRS.
Putting all modeling constraints and the objective together, the RAR-based DDL job scheduling problem (RAR-DDLS) can be formulated as the following optimization problem:
\begin{align*}
\text{\bf RAR-DDLS:} \underset{}{\ \min_{y_{js}[t], \forall j, s, t} } \max_{j\in\mathcal{J}} &\ T_j\\
    \text{subject to } 
    &\text{Constraints}~(\ref{eqn:gpu})-(\ref{eqn:completion}).  
\end{align*}

We note that Problem RAR-DDLS is an integer non-convex program with packing and covering constraints, which is NP-Hard.
In addition, the non-convex constraint in~(\ref{eqn:p_j}) involves indicator functions and the $\max$ operator, which cannot be written in a closed-from expression and hence is not amenable to conventional optimization techniques.
Due to these challenges, we will pursue an approximation algorithmic approach in Section~\ref{sec:alg} that offers provable approximation ratio guarantee.
%We summarize the key notations in Table~\ref{table:notation}.
To conclude this section, we summarize the key notations in this paper in Table~\ref{table:notation}.

\begin{table}[t!]
\centering
\caption{Notation.}
\label{table:notation}
\vspace{-.1in}
{\small
\begin{tabular}{| c | l|}
\hline
$\mathcal{T}/G_j$ &Scheduling time horizon/\# of GPUs requested by job j\\ \hline
$\mathcal{S}$/$\mathcal{N}$ &Set of servers/GPUs in the cluster\\ \hline
%$\mathcal{N}$ &The set of all GPUs in the cluster\\ \hline
$\mathcal{J}[t]$ & The set of active jobs in time-slot t \\ \hline
%$G_j$ & Number of GPUs requested by job j\\ \hline
$k_j[t]$ &  \begin{tabular}[c]{@{}l@{}l@{}}Actual largest number of contending jobs on average with\\ job j in time-slot $t$\end{tabular}\\ \hline
$\tau_j[t]$ &Per-iteration training time of job j in time-slot t\\ \hline
$y_{js}[t]$ &\# of GPUs scheduled on server $s$ for job j in time-slot $t$\\ \hline
$O_s$ &GPU capacity of server $s$\\ \hline
$a_j/T_j$ & Starting/completion time slot of job $j$ \\ \hline
%$T_j$ & Completion time slot of job $j$ \\ \hline
$\mathcal{Y}$ &  \begin{tabular}[c]{@{}l@{}l@{}}The set of feasible scheduling schemes over $\mathcal{T}$\end{tabular}\\ \hline
$\y_j^k$ & \begin{tabular}[c]{@{}l@{}l@{}} A schedule of job $j$ indexed with $k$\end{tabular}\\ \hline
$\rho(\y_j^k)$ & Actual execution time of job $j$ when schedule $\y_j^k$ is used\\ \hline
$\hat{\rho}(\y_j^k)$ & \begin{tabular}[c]{@{}l@{}l@{}}Estimated execution time of job $j$ when schedule $\y_j^k$ is used\end{tabular}\\ \hline
$\mathcal{G}(\y_j^k)$ & \begin{tabular}[c]{@{}l@{}l@{}}Set of GPUs allocated for job $j$ when schedule $\y_j^k$ is used\end{tabular}\\ \hline
$x_j^k$ & \begin{tabular}[c]{@{}l@{}l@{}}Indicate whether job $j$ follows schedule $\y_j^k$ or not\end{tabular}\\ \hline
$W_{jg}^k$ & \begin{tabular}[c]{@{}l@{}l@{}}Execution time added to GPU $g$ by job $j$ if job j follows $\y_j^k$\end{tabular}\\ \hline
$U_s^g$ & \begin{tabular}[c]{@{}l@{}l@{}} The accumulative execution time of worker $g$ on server $s$\end{tabular}\\ \hline
%
%$q_{ij}$ & \begin{tabular}[c]{@{}l@{}l@{}} \# of unit time for parameter update  at layer $j$ of job $i$
%\end{tabular}\\ \hline
%$b_j[i]$ & \begin{tabular}[c]{@{}l@{}l@{}}\# of unit time for BP  at layer $j$ of job $i$ 
%\end{tabular}\\ \hline
%$f_j[i]$ & \begin{tabular}[c]{@{}l@{}l@{}} \# of unit time for FP at layer $j$ of job $j$
%\end{tabular}\\ \hline
\end{tabular}
}
\vspace{-.1in}
\end{table}







==> MobiHoc'22_Communication_Contention_Tech_Report/Sec4_Model/Sec4_Model_backup.tex <==
% !TEX root = ../ML_Networking_INFOCOM'20.tex


\section{System Model and Problem Formulation} \label{sec:model_formulation}

In this section, we first introduce our system model, then present our general problem formulation for DDL training on shared, multi-tenant GPU clusters.
\subsection{System Model}
We consider a GPU cluster consists of servers that has limited network resources and takes the communication contention into consideration for job scheduling.
% connected with a network switch of sufficiently large bandwidth.
We let $\mathcal{S}$ represent the set of servers in the GPU cluster.
Each server $s\in\mathcal{S}$ has configured with various number of GPU capacity.
Assume that GPUs are homogeneous and synchronized.
The network performance of each server is modelled by Eqn.~(\ref{contention_reduce}) and shared among different jobs.
The GPU cluster accepts DL job requests from users, and rent GPU resource from the cluster for running the jobs.
We assume that the jobs are processed periodically and 
we use $\mathcal{J}$ to represent the set of {\em active} jobs to be trained in the current scheduling interval. 
% and let $d_j$ denote the submission time-slot of job $j\in\mathcal{J}$.
% The jobs are executed over a large time span $T$ in a time-slotted system where the scheduling time-horizon is denoted as $\mathcal{T}$. 
% The length of a time slot is potentially much larger than the duration of a training epoch, for the repeated training of the input dataset in each time slot.
% We assume the  at least one jobs is being executed at each scheduling time slot.
% There is no available information about the future upcoming jobs.
The number of GPUs of each job is specified by the user upon its submission. 
%and remains unchanged throughout the entire training process.
% We use $\mathcal{G}_j$ and $G^j$ be the set of GPUs and the number of GPUs required by job $j\in\mathcal{J}$, respectively.
% We use $G_j$ to denote the number of GPUs required by job $j\in\mathcal{J}$.
The set of GPUs can be allocated within the same server or across different servers, and will remain unchanged throughout the entire training process.
We also assume each GPU can only be occupied by one worker at any time.
% The jobs may complete at certain time slot, and we employ the dynamic scheduling.
% The job scheduling is in an online fashion, and the scheduling problem is solved at each time slot.
% Moreover, no preemption is allowed in the system, i.e., once the jobs gets started, it can not be interrupted.
% We assume that the system should be able to reassign the resources freed from the terminated jobs efficiently.
% Also, when a job runs to completion, the running jobs either can continue their training with the same number of GPUs on the same or different servers.
% Since the GPU resource is very expensive as well as avoid fragmentation, which is reserved for jobs require larger number of GPUs, the cloud is potentially assign ``just enough" servers to process the submitted jobs.

% We do not consider overall GPU resource capacity constraint in the cluster, as a cloud typically provides sufficient resources for serving a large number of customers.

% \section{Problem Formulation}

% \begin{align}
%     \text{Minimize } &c\sum_jF_jt_j\!+\!\mu\big[\sum_h(N_h\chi_h\!-\!\sum_jy_h^j)\!+\!\sum_k(N_k\chi_k\!-\!\sum_jz_k^j)\big]\\
%     \text{subject to }
%     &\sum_jy_h^j\leq N_h, \forall h\in\mathcal{H},\\
%     &\sum_jz_k^j\leq N_k, \forall k\in\mathcal{K},\\
%     &\sum_hy_h^j+\sum_kz_k^j=G_j, \forall j\in\mathcal{J},\\
%     &\sum_hy_h^j\big /\sum_kz_k^j=\gamma_j, \forall j\in\mathcal{J},\\
%     \label{eqn:k}&k=\alpha\max\{\max_h\sum_jy_h^j,\max_k\sum_jz_k^j\},\\
%     &t_j=a_j+kb_jM_j+(k-1)\eta_jM_j,\forall j\in\mathcal{J},\\
%     \label{eqn:chi_h}&\chi_h\geq \mathbbm{1}\{y_h^j\geq 1\}, \forall h\in\mathcal{H}, j\in\mathcal{J},\\
%     \label{eqn:chi_k}&\chi_k\geq \mathbbm{1}\{z_h^j\geq 1\}, \forall k\in\mathcal{K}, j\in\mathcal{J},\\
%     &\chi_h,\chi_k\in\{0,1\}, y_h^j,z_k^j\in\mathbb{Z}^+.
% \end{align}

% {\em 1)} Transformation of Eqn.~(\ref{eqn:k})

% \begin{align*}
%     k&\geq \alpha\sum_jy_h^j, \forall h\in\mathcal{H},\\
%     k&\geq \alpha\sum_jz_k^j, \forall k\in\mathcal{K}.
% \end{align*}

% {\em 2) } Transformation of Eqns.~(\ref{eqn:chi_h}) and (\ref{eqn:chi_k})

% \begin{align*}
%     y_h^j&\geq 1+ G_j(x_h^j-1), \forall h\in\mathcal{H}, j\in\mathcal{J},\\
%     z_k^j&\geq 1+ G_j(x_k^j-1), \forall k\in\mathcal{K}, j\in\mathcal{J},\\
%     x_h^j&\geq \frac{y_h^j}{G_j}, \forall h\in\mathcal{H}, j\in\mathcal{J},\\
%     x_k^j&\geq \frac{z_k^j}{G_j}, \forall k\in\mathcal{K}, j\in\mathcal{J},\\
%     \chi_h&\geq x_h^j, \forall h\in\mathcal{H}, j\in\mathcal{J},\\
%     \chi_k&\geq x_k^j, \forall k\in\mathcal{K}, j\in\mathcal{J}.
% \end{align*}



\subsection{Problem Formulation}

\begin{figure}[t]
    \centering
    \includegraphics[width=0.45\textwidth]{Figures/fig_placement.eps}
    \caption{Scenarios on different placement schemes.}\label{fig:placement}
%        \vspace{-.1in}
\end{figure}

{\bf 1) Learning Job Modeling:} 
% We use a binary variable $x_j$ to indicate whether job $j$ is executed ($x_j=1$) or not ($x_j=0$).
We use $y_{js}$ to denote the number of GPUs scheduled to server $s\in\mathcal{S}$ of job $j$.
We also use $\mathcal{S}_j$ to denote the set of servers that are used to place GPUs of job $j$.
We let $G_j$ be the number of GPUs required by job $j$.
Let $k_j$ be the maximum number of concurrent running communication tasks over all servers that associated with job $j$.
Here, we assume that $k_j$ is proportional to the max number of inter-connect communication jobs over all servers, which can be viewed as the expectation result.
%including sending or receiving gradients.
The intuition is that as the number of jobs increases, the number of concurrent running communication tasks should also be increased.
We use $\alpha$ to denote such linear coefficient.
In order to calculate $k_j$, we need to consider following two cases: 1) When all job $j$'s GPUs are placed to the same server, where its workers using intra-connect communication to training the job; 2) At least two servers are scheduled to place job $j$'s servers,  where its workers utilizing inter-connect communication.
Then the server that becomes the  bottleneck (i.e., has maximum number of scheduled jobs) needs to be found.
Take Fig.~\ref{fig:placement} as an example, Job 1 requires two GPU, which uses intra-connect communication ($|\mathcal{S}_1|=1$), and no resource contention is introduced.
Job 3 places each of its GPU into two servers (server 1 and 2), and it uses inter-connect communication.
However, no other inter-connect communication jobs are placed to server 1 and 2, thus no resource contention occurs.
With respect to job 2 and 4, their GPUs are placed to both server 3 and 4, and as a result,  the resource contention happens between these two jobs.
We can see from the figure that both server 3 and 4 has two different jobs (job 2 and 4), thus the bottleneck server in this case lies in both servers.


Based on the above discussion, we can compute $k_j$ as follows:
\begin{align}
    \label{eqn:k_j}k_j\!=\!\begin{cases}
    0, \quad\text{if }|\mathcal{S}_j|=1,\\
%    \alpha \max_{s\in\mathcal{S}_j}\sum_{j'\in\mathcal{J}}\mathbbm{1}\{y_{j's}\geq 1\},  \quad\text{if } |\mathcal{S}_j|>1.
	\alpha p_j,  \quad\text{if } |\mathcal{S}_j|>1,
    \end{cases}
\end{align}
%The first case corresponds to workers of job $j$ using internal communication since there exists some server that is scheduled to place all its GPUs.
%And the second case corresponds to workers of job $j$ using external communication since at lease two servers are arranged to host its $G_j$ workers.

% We Let $M_j$ to denote the mini-batch size of job $j$.
% Let $m^j$ denote the model size for the DNN training job $j$.
% Let $k[t]$ be the maximum number of concurrent running jobs over all the servers in time slot $t$, which can be computed as $k[t]=\max_{s\in\mathcal{S}}\{\sum_{j\in\mathcal{J}}y_s^j[t]>0\},\forall t\in\mathcal{T}$.
% We use $p_j$ to denote the computation time for each minibatch of job $j$.
where $p_j\triangleq \max_{s\in\mathcal{S}_j}\sum_{j'\in\mathcal{J}}\mathbbm{1}\{y_{j's}\geq 1\}$, i.e., the maximum number of inter-connect communication jobs over all servers associated with job $j$.

Next we can derive the per-iteration time of job $j$ by following the performance modeling Eqn~(\ref{contention_model}).
Note that the message size  $m_j$ (i.e., the size of gradients) is related to mini-batch size and the DNN model characteristics (e.g., number of layers, number of neurons at each layer).
%Here, we assume the gradient size $m_j$ is linear proportional to mini-batch size $M_j$, i.e., $m_j=\beta_jM_j$.
And we can obtain the following per-iteration time of job $j$:
\begin{align}
    \label{eqn:t_j}t_j=d_j+h_jk_j, \quad\forall j\in\mathcal{J},
\end{align}
%where $d_j\!\triangleq\! a_j+(\tau_j\beta_j+t_j^f-\eta_j\beta_j)M_j+t_j^b$ and $e_j\!\triangleq\! \beta_j(b_j+\eta_j)$.
where $d_j\triangleq a_j-\eta_jm_j+t_j^fM_j+t_j^b$ and $h_j\triangleq (e_j-\eta_j)m_j$.

% Let $\mathcal{T}_j$ be the set of time slots that job $j$ is executing.
% We use $\hat{t}_j$ to denote the completion time slot for job $j$.
% Note that if $y_s^j[t]>0$ over some server $s$ in time slot $t$, then job $j$ is being processed, thus we can use $\mathbbm{1}\{y_s^j[t]>0\}$ as the decision variable to indicate whether the job is running or not.
To ensure that there are exactly $G_j$ number of GPUs scheduled to job $j$ during its training time,
% and the allocated GPUs can be migrated throughout the entire training process,
we have:

\begin{align}
    %  \label{eqn:gpu}&\sum_{s\in\mathcal{S}}\sum_{g\in\mathcal{G}_j}y_{gs}^j[t] = G^j\cdot x_j, \quad\forall d_j \leq t\leq \hat{t}_j,j\in\mathcal{J}, \\
    \label{eqn:gpu}&\sum_{s\in\mathcal{S}}y_{js} = G_j, \quad \forall j\in\mathcal{J}.
    %  \label{eqn:gang}&y_{gs}^j[t]=y_{gs}^j[t+1], \quad \forall d_j\leq t<\hat{t}_j, g\in\mathcal{G}_j, s\in\mathcal{S},  j\in\mathcal{J}.
\end{align}
% We use $F_j\triangleq E_jG_jM_j$ to denote the total number of mini-batch training iterations for job $j$. 
% % which is specified by the user on submission.\footnote{In practice, to prevent spending excessively long time to wait the DNN training process to converge, a maximum number of iterations is usually set by the user.}
% In the DDL training setting, each worker (GPU) then needs to train $E^j\triangleq F^j/G_j$ if $G^j$ number of workers are scheduled for job $j$.
% Here we estimate the training iterations with the possible maximum number of GPUs can be deployed (we will show later that at least $G^j-1$ GPUs will be scheduled for each job).
% Since in practice, the model usually converges when only around 40\% of specified training iterations are conducted\cite{cite}.
% In other words, even with at most one fewer worker actually placed, the model typically can have good enough performance with the fewer number of training iterations.
% To make sure the total number of iterations trained for job $j$ over the entire training horizon does not exceed the specified number of iterations, which indicates that there is no extra utility to train more than $E^j$ iterations, we have:
% \begin{align}
%     \label{eqn:iter}&\sum_{t\in\mathcal{T}}e^j[t]\leq E^j,\quad\forall j\in\mathcal{J}.
%     % \label{eqn:iter}&\sum_{t\in\mathcal{T}}\frac{1}{t_f^jb^j\!+\!t_b^j\!+\!a^j\!+\!k[t]b^jm^j\!+\!(k[t]\!-\!1)\eta^j m^j}\!\geq\!E^jx_j,\quad\forall j\in\mathcal{J}.    
% \end{align}

{\bf 2) Chosen Server  Modeling: }
We use a binary variable $\chi_s$ to indicate whether server $s$ is chosen to schedule GPUs in the current interval.
Note that as long as some GPU is placed to server $s$, then $\chi_s=1$, thus we can have the following equation:
\begin{align}
    &\label{eqn:chi_s}\chi_s=\mathbbm{1}\{\sum_{j\in\mathcal{J}}y_{js}\geq 1\},\quad \forall s\in\mathcal{S}.
\end{align}

{\bf 3) Resource Constraint Modeling:} We use $N_s$ to denote the maximum number of GPUs can be scheduled to server $s\in\mathcal{S}$.
To ensure that the allocated GPUs do not exceed each server's capacity, we have:
\begin{align}
    \label{eqn:cap}&\sum_{j\in\mathcal{J}}y_{js}\leq N_s, \quad\forall s\in\mathcal{S}.
\end{align}

Finally, to define the decision variables domain, we have:

\begin{align}
    \label{eqn:int}&y_{js}, \in\mathbb{Z}^+, k_j, t_j\geq 0, \chi_s\in\{0,1\},
    \forall s\in\mathcal{S}, j\in\mathcal{J}.
\end{align}
% Note that for job $j$, its completion time $\hat{t}_j$ corresponds to the latest time-slot where there remain some active workers allocated for it.
% Therefore, we have:
% \begin{align}
%     \label{eqn:t}&\hat{t}_j = \arg\max_{t\in\mathcal{T}}\{\sum_{s\in\mathcal{S}}\sum_{g\in\mathcal{G}_j}y_{gs}^j[t]>0\},\quad\forall j\in\mathcal{J}.
% \end{align}

% Lastly, to ensure that there is no workers allocated before $j$'s arrival, we have:
% \begin{align}
%   \label{eqn:pri_arr}&y_{s}^j[t]=0,\quad\forall t<d_j, s\in\mathcal{S},j\in\mathcal{J}.
%   \label{eqn:pri_arr}&y_{s}^j[t]\in \mathbb{Z}^+,\quad\forall t\in\mathcal{T}, s\in\mathcal{S},j\in\mathcal{J}.
%   &y_{s}^j[t]\in \mathbb{Z}^+\text{ and }  \label{eqn:pri_arr}y_{s}^j[t]\leq G^j ,\quad\forall t\in\mathcal{T}, s\in\mathcal{S},j\in\mathcal{J}.
% \end{align}

{\bf 3) Objective Function and Problem Statement: } 
% We use the function  $f_j(\sum_{t\in\mathcal{T}}e^j[t])$ to denote the concave utility function for job $j$, which can deliver the results with respect to partial training iterations $\sum_{t\in\mathcal{T}}e^j[t]$.
In this paper, our goal is to minimize the overall operations cost, including the execution cost and the fragmentation cost, for all jobs from the system's perspective.
% We let $c_1$ be the time unit price paid by users, and let $c_2$ be the time unit operations cost.
We let $c$ be the time unit execution cost for running the GPUs in the cluster.
Let $E_j$ be the number of epochs to be trained of job $j$, and then  $F_j=E_jG_jM_j$ is the number of mini-batch iterations to be trained of job $j$.
The term $\sum_{j\in\mathcal{J}}cF_jt_j$ corresponds to the overall execution cost associated with each job, which is proportional to the training time.
% Thus $c\sum_{j\in\mathcal{J}}F_jt_j$ will be the total benefit by running GPUs, where $c\triangleq c_1-c_2$.
Also the term $\mu\sum_{s\in\mathcal{S}}(N_s\chi_s-\sum_{j\in\mathcal{J}}y_{js})$ is the fragmentation cost, which is measured by the difference between the number of allocated GPUs and the number of available GPUs from each selected server $s$, and $\mu$ is a penalty coefficient for unused GPUs.
On one hand, the system tends to avoid the resource contention to minimize the overall execution cost, i.e., spreading jobs over all servers.
On the other hand, the system also tends to pack jobs into servers to reduce the fragmentation cost.
Hence, to minimize the operations cost of the objective function, the system tends to find a balance between spread jobs over servers and exploit all available GPU resources for each selected server.
% In other words, the system tries to avoid too much server fragmentation, which can save internal communication for coming jobs that require larger number of GPUs.
Putting all constraints and the objective function together, the offline distributed DDL job scheduling problem~DDLJS can be formulated as:
\begin{align*}
{\bf DDLJS: } \underset{\mathbf{y,k,t,\chi}}{\text{ Minimize }} &c\sum_{j\in\mathcal{J}}F_jt_j+\mu\sum_{s\in\mathcal{S}}(N_s\chi_s-\sum_{j\in\mathcal{J}}y_{js})\\
    \text{subject to } 
    &\text{Constraints}  (\ref{eqn:k_j})-(\ref{eqn:int}).  
\end{align*}
It can be seen that Problem~DDLJS is a mixed integer nonlinear program (MINLP), which is NP-hard in general.
It involves a non-deterministic constraint~(\ref{eqn:k_j}), and two indicator functions in constraints~(\ref{eqn:k_j})(\ref{eqn:chi_s}), which are not amenable for conventional optimization techniques.
Overcoming these challenges constitutes the main subjects in the next section.
To conclude this section, we summarize the key notation used in this paper in Table~\ref{table:notation} for easy reference.

\begin{table}[t!]
\centering
\caption{Notation.}
\label{table:notation}
\begin{tabular}{|c|l|}\hline
$\mathcal{J}$ & The set of active jobs in the current scheduling interval \\ \hline
% $\tilde{t}_{j}$ & Completion time of job $j$ \\ \hline
$t_j^f$ &Average FP time to train a sample for job $j$ \\ \hline
$t_j^b$ &Average BP time to train a mini-batch for job $j$ \\ \hline
%$f_j(\cdot)$ & Job $j$'$s$ utility function \\ \hline
$M_j$ & Mini-batch size for job $j$ \\ \hline
$m_j$ & Gradient size at each mini-batch iteration for job $j$ \\ \hline
$\mathcal{S}$ & Set of servers in the GPU cluster\\ \hline 
$\chi_s$ & Binary variable to indicate whether server $s$ is chosen or not \\ \hline
$E_{j}$ & Number of training epochs for job $j$ \\ \hline
%$M_{i}$ & Number of mini-batches in a data chunk for job $i$ \\ \hline
$N_s$ & Capacity of GPUs resource on server $s$ \\ \hline
$\mathcal{G}_j$ &Set of GPUs requested by job $j$ \\ \hline
$G_j$ &Number of GPUs requested by job $j$ \\ \hline
$F_j$ &Number of mini-batch iterations to be trained of job $j$ \\ \hline
$\mathcal{S}_j$ &Set of servers used to place GPUs job $j$ \\ \hline
$y_{js}$ &Number of GPUs scheduled to server $s$ of job $j$ \\ \hline
$x_{js}$ &\begin{tabular}[c]{@{}l@{}}Binary variable to indicate whether job $j$ introduces external\\ communication in server $s$ \end{tabular}\\ \hline
$z_{jgs}$ & \begin{tabular}[c]{@{}l@{}} Binary variable to indicate whether server $s$ is selected\\ to schedule GPU $g$ for job $j$ or not\end{tabular}\\ \hline
$k_j$ &\begin{tabular}[c]{@{}l@{}}The maximum number of concurrent running jobs over all \\servers associated with job $j$\end{tabular} \\ \hline
$p_j$ &\begin{tabular}[c]{@{}l@{}}The maximum number of inter-connect communication jobs \\over all servers associated with job $j$\end{tabular}\\ \hline
%$\alpha$ &\begin{tabular}[c]{@{}l@{}}The coefficient to characterize the number of concurrent \\running communication tasks from number of concurrent \\inter-connect communication running jobs\end{tabular}\\ \hline
%$b_j$ &Transmission time per byte of job $j$\\\hline
%$\tau_j$ &Computation time per byte of job $j$\\\hline
%$a_j$ &\begin{tabular}[c]{@{}l@{}}The latency time caused by communication overhead \\(e.g., ACK time for message transmission) of job $j$\end{tabular}\\\hline
%$d_j$ & Constant defined as $a_j+(\tau_j-\eta_j)m_j++t_j^fM_j+t_j^b$ \\\hline
%$e_j$ &Constant defined as $(b_j+\eta_j)m_j$\\\hline
%$t_j$ &Per-worker-per-iteration time of job $j$\\\hline
%$\mu$ &Penalty coefficient for unused GPUs for the selected sever\\\hline
\end{tabular}
\vspace{-.2in}
\end{table}



==> MobiHoc'22_Communication_Contention_Tech_Report/Sec4_Model/Sec4_Model_backup2.tex <==
% !TEX root = ../ML_Networking_INFOCOM'20.tex


\section{System Model and Problem Formulation} \label{sec:model_formulation}

In this section, we first introduce our system model, then present our general problem formulation for DDL training on shared, multi-tenant GPU clusters.
\subsection{System Model}
We consider a GPU cluster consists of servers that has limited network resources and takes the communication contention into consideration for job scheduling.
% connected with a network switch of sufficiently large bandwidth.
We let $\mathcal{S}$ represent the set of servers in the GPU cluster.
Each server $s\in\mathcal{S}$ has configured with various number of GPU capacity.
Assume that GPUs are homogeneous and synchronized.
The network performance of each server is modelled by Eqn.~(\ref{contention_reduce}) and shared among different jobs.
The GPU cluster accepts DL job requests from users, and allocates GPU resource from the cluster for running the jobs.
We assume that the jobs are processed periodically and 
we use $\mathcal{J}$ to represent the set of {\em active} jobs to be trained in the current scheduling interval. 
% and let $d_j$ denote the submission time-slot for job $j\in\mathcal{J}$.
% The jobs are executed over a large time span $T$ in a time-slotted system where the scheduling time-horizon is denoted as $\mathcal{T}$. 
% The length of a time slot is potentially much larger than the duration of a training epoch, for the repeated training of the input dataset in each time slot.
% We assume the  at least one jobs is being executed at each scheduling time slot.
% There is no available information about the future upcoming jobs.
The number of GPUs of each job is requested by the user upon its submission. 
%and remains unchanged throughout the entire training process.
% We use $\mathcal{G}_j$ and $G^j$ be the set of GPUs and the number of GPUs required by job $j\in\mathcal{J}$, respectively.
% We use $G_j$ to denote the number of GPUs required by job $j\in\mathcal{J}$.
The set of GPUs can be allocated within the same server or across different servers, and will remain unchanged throughout the entire training process.
We also assume each GPU can only be occupied by one worker at any time.
% The jobs may complete at certain time slot, and we employ the dynamic scheduling.
% The job scheduling is in an online fashion, and the scheduling problem is solved at each time slot.
% Moreover, no preemption is allowed in the system, i.e., once the jobs gets started, it can not be interrupted.
% We assume that the system should be able to reassign the resources freed from the terminated jobs efficiently.
% Also, when a job runs to completion, the running jobs either can continue their training with the same number of GPUs on the same or different servers.
% Since the GPU resource is very expensive as well as avoid fragmentation, which is reserved for jobs require larger number of GPUs, the cloud is potentially assign ``just enough" servers to process the submitted jobs.

% We do not consider overall GPU resource capacity constraint in the cluster, as a cloud typically provides sufficient resources for serving a large number of customers.

% \section{Problem Formulation}

% \begin{align}
%     \text{Minimize } &c\sum_jF_jt_j\!+\!\mu\big[\sum_h(N_h\chi_h\!-\!\sum_jy_h^j)\!+\!\sum_k(N_k\chi_k\!-\!\sum_jz_k^j)\big]\\
%     \text{subject to }
%     &\sum_jy_h^j\leq N_h, \forall h\in\mathcal{H},\\
%     &\sum_jz_k^j\leq N_k, \forall k\in\mathcal{K},\\
%     &\sum_hy_h^j+\sum_kz_k^j=G_j, \forall j\in\mathcal{J},\\
%     &\sum_hy_h^j\big /\sum_kz_k^j=\gamma_j, \forall j\in\mathcal{J},\\
%     \label{eqn:k}&k=\alpha\max\{\max_h\sum_jy_h^j,\max_k\sum_jz_k^j\},\\
%     &t_j=a_j+kb_jM_j+(k-1)\eta_jM_j,\forall j\in\mathcal{J},\\
%     \label{eqn:chi_h}&\chi_h\geq \mathbbm{1}\{y_h^j\geq 1\}, \forall h\in\mathcal{H}, j\in\mathcal{J},\\
%     \label{eqn:chi_k}&\chi_k\geq \mathbbm{1}\{z_h^j\geq 1\}, \forall k\in\mathcal{K}, j\in\mathcal{J},\\
%     &\chi_h,\chi_k\in\{0,1\}, y_h^j,z_k^j\in\mathbb{Z}^+.
% \end{align}

% {\em 1)} Transformation of Eqn.~(\ref{eqn:k})

% \begin{align*}
%     k&\geq \alpha\sum_jy_h^j, \forall h\in\mathcal{H},\\
%     k&\geq \alpha\sum_jz_k^j, \forall k\in\mathcal{K}.
% \end{align*}

% {\em 2) } Transformation of Eqns.~(\ref{eqn:chi_h}) and (\ref{eqn:chi_k})

% \begin{align*}
%     y_h^j&\geq 1+ G_j(x_h^j-1), \forall h\in\mathcal{H}, j\in\mathcal{J},\\
%     z_k^j&\geq 1+ G_j(x_k^j-1), \forall k\in\mathcal{K}, j\in\mathcal{J},\\
%     x_h^j&\geq \frac{y_h^j}{G_j}, \forall h\in\mathcal{H}, j\in\mathcal{J},\\
%     x_k^j&\geq \frac{z_k^j}{G_j}, \forall k\in\mathcal{K}, j\in\mathcal{J},\\
%     \chi_h&\geq x_h^j, \forall h\in\mathcal{H}, j\in\mathcal{J},\\
%     \chi_k&\geq x_k^j, \forall k\in\mathcal{K}, j\in\mathcal{J}.
% \end{align*}



\subsection{Problem Formulation}

\begin{figure}[t]
    \centering
    \includegraphics[width=0.45\textwidth]{Figures/fig_placement.eps}
    \caption{Scenarios on different placement schemes.}\label{fig:placement}
%        \vspace{-.1in}
\end{figure}

{\bf 1) Learning Job Modeling:} 
% We use a binary variable $x_j$ to indicate whether job $j$ is executed ($x_j=1$) or not ($x_j=0$).
We use $y_{js}[t]$ to denote the number of GPUs scheduled on server $s\in\mathcal{S}$ in time slot $t$ for job $j$.
We also use $\mathcal{S}_j[t]$ to denote the set of servers that are used to place GPUs in time slot $t$ for job $j$.
We let $G_j$ be the number of GPUs requested by job $j$.
Let $k_j[t]$ be the maximum number of concurrent running communication tasks over all servers that associated with job $j$ in time slot $t$.
Here, we assume that $k_j[t]$ is proportional to the maximum number of inter-connect communication jobs over all servers.
%, which can be viewed as the expectation result.
%including sending or receiving gradients.
The intuition is that as the number for jobs increases, the number of concurrent running communication tasks should also be increased.
We use $\alpha$ to denote such linear coefficient.
In order to calculate $k_j[t]$, we need to consider following three cases:  1) When job $j$ finishes after $T_j$, then $k_j[t]=0$;
2) When all job $j$'s GPUs are placed to the same server in time slot $t$, where its workers using intra-connect communication to training the job; 3) At least two servers are scheduled to place job $j$'s servers in time slot $t$,  where its workers utilizing inter-connect communication.
Then the server that becomes the  bottleneck (i.e., has maximum number of scheduled jobs) needs to be found.
Take Fig.~\ref{fig:placement} as an example, Job 1 requires two GPU, which uses intra-connect communication ($|\mathcal{S}_1|=1$), and no resource contention is introduced.
Job 3 places each of its GPU into two servers (server 1 and 2), and it uses inter-connect communication.
However, no other inter-connect communication jobs are placed to server 1 and 2, thus no resource contention occurs.
With respect to job 2 and 4, their GPUs are placed to both server 3 and 4, and as a result,  the resource contention happens between these two jobs.
We can see from the figure that both server 3 and 4 has two different jobs (job 2 and 4), thus the bottleneck server in this case lies in both servers.


Based on the above discussion, we can compute $k_j[t]$ as follows:
\begin{align}
    \label{eqn:k_j}k_j{\color{red}[t]}=\begin{cases}
    0, \quad\text{if } t>{T}_j,\\
    0, \quad\text{if }|\mathcal{S}_j{\color{red}[t]}|=1, {\color{red}\forall t\leq T_j},\\
%    \alpha \max_{s\in\mathcal{S}_j}\sum_{j'\in\mathcal{J}}\mathbbm{1}\{y_{j's}\geq 1\},  \quad\text{if } |\mathcal{S}_j|>1.
	\alpha p_j{\color{red}[t]},  \quad\text{if } |\mathcal{S}_j{\color{red}[t]}|>1, {\color{red}\forall t\leq T_j},
    \end{cases}
\end{align}
%The first case corresponds to workers for job $j$ using internal communication since there exists some server that is scheduled to place all its GPUs.
%And the second case corresponds to workers for job $j$ using external communication since at lease two servers are arranged to host its $G_j$ workers.

% We Let $M_j$ to denote the mini-batch size for job $j$.
% Let $m^j$ denote the model size for the DNN training job $j$.
% Let $k[t]$ be the maximum number of concurrent running jobs over all the servers in time slot $t$, which can be computed as $k[t]=\max_{s\in\mathcal{S}}\{\sum_{j\in\mathcal{J}}y_s^j[t]>0\},\forall t\in\mathcal{T}$.
% We use $p_j$ to denote the computation time for each minibatch for job $j$.
where $p_j[t]\triangleq \max_{s\in\mathcal{S}_j[t]}\sum_{j'\in\mathcal{J}}\mathbbm{1}\{y_{j's}[t]\geq 1\}$, i.e., the maximum number of inter-connect communication jobs over all servers associated with job $j$ in time slot $t$.

Next we can derive the per-iteration time for job $j$ by following the performance modeling Eqn~(\ref{contention_model}).
Note that the message size  $m_j$ (i.e., the size of gradients) is related to mini-batch size and the DNN model characteristics (e.g., number of layers, number of neurons at each layer).
%Here, we assume the gradient size $m_j$ is linear proportional to mini-batch size $M_j$, i.e., $m_j=\beta_jM_j$.
And we can obtain the following per-iteration time for job $j$:
\begin{align}
	t_j[t]=\begin{cases}
	0, \quad\forall j\in\mathcal{J}, t>{T}_j,\\
	 \label{eqn:t_j}d_j+h_jk_j{\color{red}[t]}, \quad\forall j\in\mathcal{J}, {\color{red}t\leq T_j},
	\end{cases}
   \end{align}
%where $d_j\!\triangleq\! a_j+(\tau_j\beta_j+t_j^f-\eta_j\beta_j)M_j+t_j^b$ and $e_j\!\triangleq\! \beta_j(b_j+\eta_j)$.
where $d_j\triangleq a_j-\eta_jm_j+t_j^fM_j+t_j^b$ and $h_j\triangleq (e_j-\eta_j)m_j$.

% Let $\mathcal{T}_j$ be the set of time slots that job $j$ is executing.
% We use $\hat{t}_j$ to denote the completion time slot for job $j$.
% Note that if $y_s^j[t]>0$ over some server $s$ in time slot $t$, then job $j$ is being processed, thus we can use $\mathbbm{1}\{y_s^j[t]>0\}$ as the decision variable to indicate whether the job is running or not.
To ensure that there are exactly $G_j$ number of GPUs scheduled to job $j$ during its training time,
% and the allocated GPUs can be migrated throughout the entire training process,
we have:

\begin{align}
    %  \label{eqn:gpu}&\sum_{s\in\mathcal{S}}\sum_{g\in\mathcal{G}_j}y_{gs}^j[t] = G^j\cdot x_j, \quad\forall d_j \leq t\leq \hat{t}_j,j\in\mathcal{J}, \\
    \label{eqn:gpu}&\sum_{s\in\mathcal{S}}y_{js}{\color{red}[t]} = G_j, \quad \forall j\in\mathcal{J}, t\leq T_j.
    %  \label{eqn:gang}&y_{gs}^j[t]=y_{gs}^j[t+1], \quad \forall d_j\leq t<\hat{t}_j, g\in\mathcal{G}_j, s\in\mathcal{S},  j\in\mathcal{J}.
\end{align}
% We use $F_j\triangleq E_jG_jM_j$ to denote the total number of mini-batch training iterations for job $j$. 
% % which is specified by the user on submission.\footnote{In practice, to prevent spending excessively long time to wait the DNN training process to converge, a maximum number of iterations is usually set by the user.}
% In the DDL training setting, each worker (GPU) then needs to train $E^j\triangleq F^j/G_j$ if $G^j$ number of workers are scheduled for job $j$.
% Here we estimate the training iterations with the possible maximum number of GPUs can be deployed (we will show later that at least $G^j-1$ GPUs will be scheduled for each job).
% Since in practice, the model usually converges when only around 40\% of specified training iterations are conducted\cite{cite}.
% In other words, even with at most one fewer worker actually placed, the model typically can have good enough performance with the fewer number of training iterations.
% To make sure the total number of iterations trained for job $j$ over the entire training horizon does not exceed the specified number of iterations, which indicates that there is no extra utility to train more than $E^j$ iterations, we have:
% \begin{align}
%     \label{eqn:iter}&\sum_{t\in\mathcal{T}}e^j[t]\leq E^j,\quad\forall j\in\mathcal{J}.
%     % \label{eqn:iter}&\sum_{t\in\mathcal{T}}\frac{1}{t_f^jb^j\!+\!t_b^j\!+\!a^j\!+\!k[t]b^jm^j\!+\!(k[t]\!-\!1)\eta^j m^j}\!\geq\!E^jx_j,\quad\forall j\in\mathcal{J}.    
% \end{align}

%{\bf 2) Chosen Server  Modeling: }
%We use a binary variable $\chi_s$ to indicate whether server $s$ is chosen to schedule GPUs in the current interval.
%Note that as long as some GPU is placed to server $s$, then $\chi_s=1$, thus we can have the following equation:
%\begin{align}
%    &\label{eqn:chi_s}\chi_s=\mathbbm{1}\{\sum_{j\in\mathcal{J}}y_{js}\geq 1\},\quad \forall s\in\mathcal{S}.
%\end{align}

{\bf 3) Resource Constraint Modeling:} We use a binary variable $\chi_s[t]$ to indicate whether server $s$ is chosen to schedule GPUs in the current interval in time slot $t$.
We use $N_s$ to denote the maximum number of GPUs can be scheduled to server $s\in\mathcal{S}$.
To ensure that the allocated GPUs do not exceed each server's capacity, we have:
\begin{align}
    \label{eqn:cap}&\sum_{j\in\mathcal{J}}y_{js}{\color{red}[t]}\leq N_s\chi_s{\color{red}[t]}, \quad\forall s\in\mathcal{S}, t\leq T_j.
\end{align}
We can know from the above equation that if server $s$ is not chosen to do the scheduling in time slot $t$ ($\chi_s[t]=0$), then no GPUs could be placed on the server. 


 {\bf 4) Completion Time Modeling:} We use $T_j$ to denote the completion time slot for job $j$.
 In each time slot $t$, the number of mini-batch iterations can be completed is $\frac{t'}{t_j[t]}$, where $t'$ is the time duration for each time slot $t$ (e.g., 10 minutes).
The smallest time slot that finishes at lest $F_j$ iterations is the completion time for job $j$, we have:
\begin{align}
%\sum_{t\in\mathcal{T}_j}\frac{t'}{t_j[t]}=F_j, \quad \forall j\in\mathcal{J}.
T_j=\arg\min_t \{\sum_{t\in\mathcal{T}}\frac{t'}{t_j[t]}\geq F_j\}, \quad \forall j\in\mathcal{J}.
\end{align}

Next, to ensure the jobs will not be interrupted and the placement scheme remains unchanged during its training process, we have

\begin{align}
y_{js}[t]=\begin{cases}
0, \quad\forall i\in\mathcal{S},j\in\mathcal{J},t>T_j,\\
y_{js}[t-1],  \quad\forall i\in\mathcal{S},j\in\mathcal{J},t\leq T_j.
\end{cases}
\end{align}


Finally, to define the decision variables domain, we have:

\begin{align}
    \label{eqn:int}&y_{js}[t] \in\mathbb{Z}^+, \chi_s[t]\in\{0,1\},
    \forall s\in\mathcal{S}, j\in\mathcal{J},t\in\mathcal{T}.
\end{align}

%{\color{red}
%\begin{align}
%y_{js}[t]=y_{js}[t-1], \forall t\leq T_j, y_{js}[t]=0, \forall t > T_j, s\in\mathcal{S}, j\in\mathcal{J}.
%\end{align}
%}

% Note that for job $j$, its completion time $\hat{t}_j$ corresponds to the latest time-slot where there remain some active workers allocated for it.
% Therefore, we have:
% \begin{align}
%     \label{eqn:t}&\hat{t}_j = \arg\max_{t\in\mathcal{T}}\{\sum_{s\in\mathcal{S}}\sum_{g\in\mathcal{G}_j}y_{gs}^j[t]>0\},\quad\forall j\in\mathcal{J}.
% \end{align}

% Lastly, to ensure that there is no workers allocated before $j$'s arrival, we have:
% \begin{align}
%   \label{eqn:pri_arr}&y_{s}^j[t]=0,\quad\forall t<d_j, s\in\mathcal{S},j\in\mathcal{J}.
%   \label{eqn:pri_arr}&y_{s}^j[t]\in \mathbb{Z}^+,\quad\forall t\in\mathcal{T}, s\in\mathcal{S},j\in\mathcal{J}.
%   &y_{s}^j[t]\in \mathbb{Z}^+\text{ and }  \label{eqn:pri_arr}y_{s}^j[t]\leq G^j ,\quad\forall t\in\mathcal{T}, s\in\mathcal{S},j\in\mathcal{J}.
% \end{align}



%To obtain the time completion time for job $j$, we check the largest time slot that $\sum_{s\in\mathcal{S}}y_{js}[t]>0$, i.e.,
%\begin{align}
%T_j=\arg\max_t\{\sum_{s\in\mathcal{S}}y_{js}[t]>0\}, \quad\forall j\in\mathcal{J}.
%\end{align}

%Also, to ensure the job is not preempted once get started, we have:
%\begin{align}
%t_j[t]>0,
%\end{align}



{\bf 3) Objective Function and Problem Statement: } 
% We use the function  $f_j(\sum_{t\in\mathcal{T}}e^j[t])$ to denote the concave utility function for job $j$, which can deliver the results with respect to partial training iterations $\sum_{t\in\mathcal{T}}e^j[t]$.
In this paper, our goal is to minimize the overall operations cost, including the execution cost and the fragmentation cost, for all jobs from the system's perspective.
% We let $c_1$ be the time unit price paid by users, and let $c_2$ be the time unit operations cost.
We let $c$ be the time unit execution cost for running the GPUs in the cluster.
Let $E_j$ be the number of epochs to be trained for job $j$, and then  $F_j=E_jG_jM_j$ is the number of mini-batch iterations to be trained for job $j$.
The term ${\color{red}c\sum_{j\in\mathcal{J}}T_j}$ corresponds to the overall execution cost associated with each job, which is proportional to the training time.
% Thus $c\sum_{j\in\mathcal{J}}F_jt_j$ will be the total benefit by running GPUs, where $c\triangleq c_1-c_2$.
Also the term ${\color{red}\mu\sum_{t\in\mathcal{T}}\sum_{s\in\mathcal{S}}(N_s\chi_s[t]-\sum_{j\in\mathcal{J}}y_{js}[t])}$ is the fragmentation cost, which is measured by the difference between the number of allocated GPUs and the number of available GPUs from each selected server $s$, and $\mu$ is a penalty coefficient for unused GPUs.
On one hand, the system tends to avoid the resource contention to minimize the overall execution cost, i.e., spreading jobs over all servers.
On the other hand, the system also tends to pack jobs into servers to reduce the fragmentation cost.
Hence, to minimize the operations cost of the objective function, the system tends to find a balance between spread jobs over servers and exploit all available GPU resources for each selected server.
% In other words, the system tries to avoid too much server fragmentation, which can save internal communication for coming jobs that require larger number of GPUs.
Putting all constraints and the objective function together, the offline distributed DDL job scheduling problem~DDLJS can be formulated as:
\begin{align*}
{\bf DDLJS: } \underset{\mathbf{y,\chi}}{\text{ Minimize }} &c\sum_{j\in\mathcal{J}}T_j+\mu\sum_{t\in\mathcal{T}}\sum_{s\in\mathcal{S}}(N_s\chi_s[t]-\sum_{j\in\mathcal{J}}y_{js}[t])\\
    \text{subject to } 
    &\text{Constraints}  (\ref{eqn:k_j})-(\ref{eqn:int}).  
\end{align*}
It can be seen that Problem~DDLJS is a mixed integer nonlinear program (MINLP), which is NP-hard in general.
It involves both non-deterministic and indicator function in constraint~(\ref{eqn:k_j}), which are not amenable for conventional optimization techniques.
Overcoming these challenges constitutes the main subjects in the next section.
To conclude this section, we summarize the key notation used in this paper in Table~\ref{table:notation} for easy reference

\begin{table}[t!]
\centering
\caption{Notation.}
\label{table:notation}
\begin{tabular}{|c|l|}\hline
$\mathcal{J}$ & The set of active jobs in the current scheduling interval \\ \hline
% $\tilde{t}_{j}$ & Completion time for job $j$ \\ \hline
$t_j^f$ &Average FP time to train a sample for job $j$ \\ \hline
$t_j^b$ &Average BP time to train a mini-batch for job $j$ \\ \hline
%$f_j(\cdot)$ & Job $j$'$s$ utility function \\ \hline
$M_j$ & Mini-batch size for job $j$ \\ \hline
$m_j$ & Gradient size at each mini-batch iteration for job $j$ \\ \hline
$\mathcal{S}$ & Set of servers in the GPU cluster\\ \hline 
$\chi_s$ & Binary variable to indicate whether server $s$ is chosen or not \\ \hline
$E_{j}$ & Number of training epochs for job $j$ \\ \hline
%$M_{i}$ & Number of mini-batches in a data chunk for job $i$ \\ \hline
$N_s$ & Capacity of GPUs resource on server $s$ \\ \hline
$\mathcal{G}_j$ &Set of GPUs requested by job $j$ \\ \hline
$G_j$ &Number of GPUs requested by job $j$ \\ \hline
$F_j$ &Number of mini-batch iterations to be trained for job $j$ \\ \hline
$\mathcal{S}_j$ &Set of servers used to place GPUs job $j$ \\ \hline
$y_{js}$ &Number of GPUs scheduled to server $s$ for job $j$ \\ \hline
$x_{js}$ &\begin{tabular}[c]{@{}l@{}}Binary variable to indicate whether job $j$ introduces external\\ communication in server $s$ \end{tabular}\\ \hline
$z_{jgs}$ & \begin{tabular}[c]{@{}l@{}} Binary variable to indicate whether server $s$ is selected\\ to schedule GPU $g$ for job $j$ or not\end{tabular}\\ \hline
$k_j$ &\begin{tabular}[c]{@{}l@{}}The maximum number of concurrent running jobs over all \\servers associated with job $j$\end{tabular} \\ \hline
$p_j$ &\begin{tabular}[c]{@{}l@{}}The maximum number of inter-connect communication jobs \\over all servers associated with job $j$\end{tabular}\\ \hline
%$\alpha$ &\begin{tabular}[c]{@{}l@{}}The coefficient to characterize the number of concurrent \\running communication tasks from number of concurrent \\inter-connect communication running jobs\end{tabular}\\ \hline
%$b_j$ &Transmission time per byte for job $j$\\\hline
%$\tau_j$ &Computation time per byte for job $j$\\\hline
%$a_j$ &\begin{tabular}[c]{@{}l@{}}The latency time caused by communication overhead \\(e.g., ACK time for message transmission) for job $j$\end{tabular}\\\hline
%$d_j$ & Constant defined as $a_j+(\tau_j-\eta_j)m_j++t_j^fM_j+t_j^b$ \\\hline
%$e_j$ &Constant defined as $(b_j+\eta_j)m_j$\\\hline
%$t_j$ &Per-worker-per-iteration time for job $j$\\\hline
%$\mu$ &Penalty coefficient for unused GPUs for the selected sever\\\hline
\end{tabular}
\vspace{-.2in}
\end{table}

\section{Initial Approach}
Without loss of generality, we assume $T_1\leq T_2\hdots \leq T_j \leq\hdots\leq T_J$.

\begin{align*}
T_1&=F_1t_1^{(1)}\\
T_2&=T_1+\big(F_2-\frac{T_1}{t_2^{(1)}}\big)t_2^{(2)}=F_1t_1^{(1)}\big(1-\frac{t_2^{(2)}}{t_2^{(1)}}\big)+F_2t_2^{(2)}\\
T_3&=T_2+\big(F_3-\frac{T_1}{t_3^{(1)}}-\frac{T_2-T_1}{t_3^{(2)}}\big)t_3^{(3)}\\
%&=F_1t_1^{(1)}\bigg((1-\frac{t_3^{(3)}}{t_3^{(2)}})(1-\frac{t_2^{(2)}}{t_2^{(1)}})-\frac{t_3^{(3)}}{t_3^{(1)}}\bigg)\\
%&+F_2t_2^{(2)}(1-\frac{t_3^{(3)}}{t_3^{(2)}})+F_3t_3^{(3)}\\
&\hdots\\
T_j&=T_{j-1}+\big(F_j-\frac{T_1}{t_j^{(1)}}-\frac{T_2-T_1}{t_j^{(2)}}-\hdots-\frac{T_{j-1}-T_{j-2}}{t_j^{(j-1)}}\big)t_j^{(j)}\\
&\hdots\\
T_J&=T_{J-1}+\big(F_J-\frac{T_1}{t_J^{(1)}}-\frac{T_2-T_1}{t_J^{(2)}}-\hdots-\frac{T_{J-1}-T_{J-2}}{t_j^{(J-1)}}\big)t_J^{(J)}
\end{align*}

\begin{align*}
&\sum_{t\in\mathcal{T}}\sum_{j\in\mathcal{J}[t]}(t-\frac{t}{\tau_j[t]}\tau_j^0)\\
&=J*(T_1-\frac{T_1}{\tau_1[t]}\tau_1^0)+(J-1)*(T_2-T_1-\frac{T_2-T_1}{\tau_2[t]}\tau_2^0)\\
&+\hdots+(J-j+1)(T_j-T_{j-1}-\frac{T_j-T_{j-1}}{\tau_j[t]}\tau_j^0)\\
&+\hdots+(T_J-T_{J-1}-\frac{T_{J}-T_{J-1}}{\tau_J[t]}\tau_J^0)\\
&\leq r*\sum_{k=0}^{J-1}(J-k)(T_{k+1}-T_k)
\end{align*}
where $r=max_{k,t}(1-\frac{\tau_k^0}{\tau_k[t]})$ and $T_0=0$.

\begin{align*}
&\sum_{s\in\mathcal{S}}y_{js}=G_j, \quad \forall j\in\mathcal{J}[t],\\
&\sum_{j\in\mathcal{J}[t]}y_{js}\leq N_s, \quad\forall s\in\mathcal{S}.
\end{align*}




==> MobiHoc'22_Communication_Contention_Tech_Report/Sec5_Algorithm/Sec5_Algorithm.tex <==
% !TEX root = ../Communication_Contention_MobiHoc22.tex

\section{Solution Approach} \label{sec:alg}
As mentioned in Section~\ref{sec:model_formulation}, a key challenge to solve Problem~RAR-DDLS is that, due to the mixed covering- and packing-type constraints, the number of job scheduling combinations grows exponentially as the number of servers/jobs increases.
% in constraint~(\ref{eqn:p_j}).
Thus, it is computationally prohibitive to enumerate all possible combinations before the scheduler decides when to start and which GPU(s) should be allocated to achieve the optimal scheduling.
Exacerbating the problem is the fact that communication contention renders a mixed-integer bilinear structure in (\ref{eqn:p_j}), making it intractable to express $p_{j}[t]$ in closed-form.
Due to these challenges, it is difficult to directly solve Problem~RAR-DDLS based on its original formulation.
To overcome this challenge, we propose the following ``indirect'' approach to solve Problem~RAR-DDLS.

\smallskip
{\bf 1) Basic Idea:}
First, we note that, although not in closed-form expressions, the per-iteration time $\tau_j[t]$ for each job can be computed in polynomial time according to (\ref{eqn:p_j})-(\ref{contention_model}) once a schedule (i.e., $\y[t] = \{y_{js}[t], \forall j, s\}$) is given.
Specifically, we note that the per-iteration time $\tau_j[t]$ is determined by $B_j(\y[t])$ and $\gamma_j(\y_j[t])$.
Moreover, $f(\boldsymbol{\alpha}, k_j[t])$ increases as $k_j[t]$ gets larger, and $\gamma_j(\y_j[t])$ increases as $\sum_s\mathds{1}\{y_{js}[t]>0\}$ grows.
Thus, the range of $\tau_j[t]$ can be estimated.
The largest number of $k_j[t]$ is $\max_s O_s$, i.e., the worst case would be each job places one of its workers into the server with the biggest capacity and they all compete for the bandwidth.
Thus, we can have $B_j(\y[t]) \in [b^e/f(\boldsymbol{\alpha}, \max_s O_s), b^i]$.
 In addition, we have $\sum_s\mathds{1}\{y_{js}[t]>0\}\in[1, G_j]$.
 Then by plugging $B_j(\y[t])$ and $\sum_s\mathds{1}\{y_{js}[t]>0\}$ with their lower and upper bounds in Eqn.~(\ref{contention_model}), respectively, we can attain the lower and upper bounds.
 % $\varphi^{\min}_j[t]$ and $\varphi^{\max}_j[t]$ of $\tau_j[t]$.
%\textcolor{red}{We define $\varphi^{\max}_j\triangleq \max_t\varphi^{\max}_j[t]$ and $\varphi^{\min}_j\triangleq \min_t\varphi^{\min}_j[t]$.
%We also define the possible largest ratio over all jobs as $\varphi\triangleq\max_j\varphi^{\max}_j/\varphi^{\min}_j$.}


The above insight suggests that we can solve Problem~RAR-DDLS via the following {\em search-based approach} to circumvent the structural difficulty in (\ref{eqn:p_j})-(\ref{contention_model}) .
We can first search for a schedule $\y$, then $\tau_j[t],\forall t$ can be efficiently evaluated to estimate the makespan.
Then, we repeat the process until we find a ``good enough'' schedule.
Therefore, we can have the algorithmic framework as shown in Fig.~\ref{fig:idea} to obtain an approximate makespan if the search space is given.
Clearly, the search space of $\y$ remains huge and difficult to sample.
Nonetheless, in what follows, we show that Problem~RAR-DDLS can be reformulated to facilitate this search-based approach.

\begin{figure}[t!]
    \centering
    \includegraphics[width=0.45\textwidth]{Figures/fig_idea_overview.eps}
    \caption{Basic idea for solving Problem~RAR-DDLS.}\label{fig:idea}
    \vspace{-.1in}
\end{figure}

\smallskip
{\bf 2) Problem Reformulation:}
In order to enable the search of a schedule, we first reformulate Problem~RAR-DDLS by introducing following notations.
We let $\mathcal{N} = \{1, \hdots, N\}$ be the set of all GPUs in the cluster.
Let $\mathcal{Y}=\{\y^1,\hdots,\y^{|\mathcal{Y}|}\}$ be the set of feasible scheduling schemes for the jobs to be scheduled, where $\y^k=\{\y_1^k,\hdots,\y_J^k\}$ and $\y_j^k=\{y^k_{js}[t], \forall s\in\mathcal{S}, t\in\mathcal{T}\}\in\mathbb{Z}_+^{S\times T}$.
Note that, with a slight abuse of notation, we use $y^k_{js}[t]$ here as a constant (not a variable) to denote the number of workers allocated for job $j$ on server $s$ in time-slot $t$ if  schedule $\y^k$ is used.
We also use $\rho_j(\y^k)$ to denote the execution time of job $j$ if schedule $\y^k$ is used.
Also, we denote the starting time of job $j$ under schedule $\y^k$ as $a_j(\y^k)\triangleq \arg\min\{t | y^k_{js}[t] > 0, \exists s\}$.
%We let $z^k$ be the binary variable to indicate whether scheduling $\y^k$ is chosen ($z^k=1$) or not ($z^k=0$).
Let $x_j^k \in \{0,1\}$ be the binary variable to indicate whether job $j$ follows schedule $\y^k$ ($x_j^k=1$) or not ($x_j^k=0$).
%Let $\mathcal{G}(\y^k)$ be the set of GPUs allocated when using scheduling $\y^k$.
Then Problem~RAR-DDLS can be reformulated as the following integer linear program (ILP):
\begin{align}
\label{problem:makespan}\min_{x_j^k,\forall j,k} \max_j& \ x_j^k\big(a_j(\y^k)+\rho_j(\y^k)\big)\\
\text{subject to. } &\sum_{k\in\{1,\hdots,|\mathcal{Y}|\}}x_j^k = 1,\quad \forall j\in\mathcal{J},\label{eqn:all_placed}\\
&x_j^k = x_{j'}^k, \quad \forall j, j'\in\mathcal{J}, k\in\{1,\hdots,|\mathcal{Y}|\},\label{eqn:placement}\\
&x_j^k\in\{0,1\}, \quad\forall j\in\mathcal{J}, k\in\{1,\hdots,|\mathcal{Y}|\}.\label{eqn:binary}
\end{align}
Constraint~(\ref{eqn:all_placed}) ensures that exactly one schedule is chosen.
Constraint~(\ref{eqn:placement}) ensures that all jobs use the same schedule $\y^k$.
We note that, although Problem~(\ref{problem:makespan}) has a simpler structure compared to Problem~RAR-DDLS, it hides the complexity in the dimensionality of the exponential search space $\mathcal{Y}$, which is intractable to explore.
However, based on this reformulated problem, we will show next that it is possible for one to identify a ``good enough'' schedule such that the makespan can be upper bounded.

Unfortunately, Problem~(\ref{problem:makespan}) remains an NP-hard problem.
We state this formally in Theorem~\ref{thm:np}, which can be proved based on the reduction to the vertex coloring problem (VCP). 

\begin{thm}\label{thm:np}
Let $n_g=\max_j G_j$.
Solving Problem~\eqref{problem:makespan} to within an $O(\frac{\log n_g}{2^{\sqrt{\log\log n_g}}})$-approximate ratio is NP-hard even when the exact processing time of each job is available.
\end{thm}
%Due to space limitation, %we provide proof sketches for some results in this section.
%we relegate the proof to our online technical report~\cite{Yu22:SJF-BCO_report}.
%(see the proof in our online technical report \cite{??}).
\begin{proof}
Here, we consider the special case with all jobs having a unit processing time ($\rho(\y^k)=1$).
We first show that VCP can be reduced to the job scheduling problem in Problem~(\ref{problem:lp}) in polynomial time.
Given an instance $I$ of VCP, i.e., given a graph $G=(V, E)$ with bounded degree $n_g$, we can construct our job scheduling problem as follows: i) For each node $v\in V$, we create a job $j_v\in\mathcal{J}$, where it has only one schedule $y_{j_v} = \emptyset$;
% that no GPU is allocated yet; 
ii) For each edge $(u, v)\in E$,  we add a worker $w_{u,v}$ to $\mathcal{S}$. Also, update the scheduling as $y_{j_u}=y_{j_u} \cup \{w_{u,v}\}$ and $y_{j_v}=y_{j_v} \cup \{w_{u,v}\}$.
If the graph $G's$ maximum degree is no greater than $n_g$, then the maximum number of workers that can be allocated to each job is also $n_g$.

With this reduction, we next show the solution of VCP can be translated to the solution of Problem~(\ref{problem:lp}), and vice verse.
First, recall that each job has one unit processing time.
Thus, all jobs should be executed inside a unit time interval ($[0, 1), [1, 2), \hdots$).
If we have the solution to VCP, then we can schedule jobs with the same color in the same interval.
Also, if we have the solution to the job scheduling problem, then the jobs in the same interval can be marked as the same color.
Hence, finding an optimal solution of Problem~(\ref{problem:lp}) is equivalent to find an optimal solution of VCP.

Similarly, given an instance of job scheduling, we can construct an instance of VCP, where the makespan equals to the number of colors.
Therefore, if we have an $\alpha$-approximate solution to the job scheduling problem, we have an $\alpha$-approximate solution to VCP.
However, 
%it has known that finding a solution of $2^{O((\log K)^2)}$ colors for $K$-colorable graphs with degree at most $2^{2^{(\log K)^2}}$~\cite{Khot01:vertex-color} is NP-hard, i.e., 
with the graph of degree at most $n_g$, it is known that coloring a $2^{\sqrt{\log\log n_g}}$-colorable graph with $O(\log n_g)$ colors is NP-Hard.
This completes the proof.
%Thus it is NP-hard to find a solution that is $O(\frac{\log n_g}{2^{\sqrt{\log\log n_g}}})$-approximate.
\end{proof}
The hardness result in Theorem~\ref{thm:np} suggests that solving Problem~(\ref{problem:makespan}) necessitates the design of approximation algorithms, which is our goal in algorithm development next.

%\subsection{Converting to an Integer Linear Program}
\smallskip
{\bf 3) Identify a Scheduling with Bounded Makespan:}
We let $\mathcal{G}_j(\y^k)$ be the set of GPUs allocated for job $j$ when schedule $\y^k$ is used.
We use $W_{jg}^k=x_j^k\rho_j(\y^k)$ to denote the execution time added to GPU $g$ by job $j$ if job $j$ follows schedule $\y^k$. %with $g\in\mathcal{G}_j(\y^k)$.
Since each job $j$ only chooses one schedule, the total execution time of GPU $g$ can be computed as $W_g=\sum_j\sum_kW_{jg}^k$.
However, due to communication contention, the exact processing time $\rho_j(\y^k)$ is hard to evaluate in computing $W_{jg}^{k}$. %, and thus estimated value is given instead.
Fortunately, the estimated processing time $\hat{\rho}_j(\y^k)$ can be bounded as $\hat{\rho}_j(\y^k) \in [l\rho_j(\y^k), u\rho_j(\y^k)]$ for some $l\leq 1$ and $u\geq 1$, since $\tau_j[t]$ is bounded. 
Here, we use $\frac{\hat{\rho}_j(\y^k)}{u}\leq \rho_j(\y^k)$ to replace $\rho_j(\y^k)$ when computing $W_{jg}^{k}$.
%Then, the following ILP finds a lower bound of $W^\pi_{\max}$, which is also a lower bound of the optimal makespan.
Consider a search algorithm $\pi$ that solves the following ILP to choose one schedule from $\mathcal{Y}$:
\begin{align}
\label{problem:lp}&\min \  -1\\
\text{subject to. }
&\hat{W}_{jg}^k = x_j^k\frac{\hat{\rho}_j(\y^k)}{u}, \forall j\!\in\!\mathcal{J}, k\!\in\!\{1,\hdots,|\mathcal{Y}|\}, g\!\in\!\mathcal{N},\label{eqn:wk}\\
&\sum_{j\in\mathcal{J}}\sum_{k\in\{1,\hdots,|\mathcal{Y}|\}}\hat{W}_{jg}^k\leq \theta_u, \quad \forall g\in\mathcal{N},\label{eqn:gpu_lp}\\
\nonumber&\text{Constraints}~(\ref{eqn:all_placed})-(\ref{eqn:binary}).
\end{align}
Note that Problem~(\ref{problem:lp}) has no objective function to be optimized since we are only interested in whether a feasible solution no greater than a given maximum execution time limit $\theta_u$ exists ($\theta_u$ depends on parameter $u$).
Constraints~(\ref{eqn:wk})--(\ref{eqn:gpu_lp}) ensure that no GPU's execution time would exceed $\theta_u$.
Let $W^{\pi}_{\max}=\max_{g\in\mathcal{N}}W_g$ be the maximum execution time of all GPUs returned by algorithm $\pi$.
Due to the use of estimated $\frac{\hat{\rho}_j(\y^k)}{u}$, the solution of $\pi$ finds a lower bound of $W_{\max}^{\pi}$, which is also a lower bound of the makespan under $\pi$ (due to potential idling resulted from synchronization barrier). % in gang scheduling

Note that for any feasible scheduling with the upper bound $\theta_u$ for Problem~(\ref{problem:lp}), we can find a corresponding feasible solution for Problem~(\ref{problem:makespan}) by setting $x_j^k=1$ if job $j$ follows schedule $\y^k$; otherwise, set $x_j^k = 0$.
Thus, the challenge of solving Problem~(\ref{problem:makespan}) becomes finding a tightest execution time limit $\theta_u$ for Problem~(\ref{problem:lp}), which is relatively easy since there is no need to explore the exponential search space of schedules $\mathcal{Y}$.



It is insightful to understand the choice of $\theta_u$ in Problem~\eqref{problem:lp}.
On one hand, if $\theta_u$ is too small, Problem~(\ref{problem:lp}) could be infeasible, and no scheduling for Problem~(\ref{problem:makespan}) can be found.
On the other hand, when $\theta_u$ is too large, then all schedulings can be considered, and the gap between the optimal maximum execution time and the optimal makespan can be large, thus no meaningful lower bound of $W^\pi_{\max}$ can be found.
Fortunately, since determining an appropriate $\theta_{u}$ is a {\em univariate} search, we can simply use the bisection method to efficiently find the minimum $\theta_u$ feasible to Problem~(\ref{problem:lp}).



\smallskip
{\bf 4) Algorithm Description:}
We next present our scheduling algorithm based on bisection to search $\theta_u$ and the smallest job first strategy to solve Problem~\eqref{problem:lp} for a given $\theta_u$. %~\cite{Jeon2018:multi-tenant} to schedule the jobs, which is adopted in existing schedulers for deep learning execution times.
Note that if a job's ring of workers is scheduled over a large number of servers, it may potentially worsen communication contention with concurrent jobs and its communication overhead could be large.
%; while always addressing the consolidation of workers may lead to execution time unbalance and extensive communication contention.
Therefore, to control the number of active servers, we use a threshold parameter $\kappa \in[1, n_g]$  to control the number of maximum servers for scheduling jobs.
We summarize our scheduling approach in Algorithm~\ref{alg:place}.
The intuition behind Algorithm~\ref{alg:place} is that: 
1) When the job is small (i.e., $G_j \leq \kappa$), we prefer to pack the job into servers whose GPUs are already occupied by some other jobs rather than opening new server(s) to host its workers. 
Since the job is small, the induced contention is mild by using the shared servers. 
Further, by packing its workers to these servers, we can avoid fragmentation introduced by a small job and save space for larger jobs that will be scheduled next.
2) If $G_j > \kappa$, we prefer to allocate the job's workers to new server(s).
% to avoid potential large overhead. 
This is because shared servers may only have limited available GPU(s), and in order to gang-schedule a large job, a large number of shared servers may be used, which leads to a high communication overhead.
%Hence, we introduce $\kappa$ to balance between the communication contention and overhead.



 \begin{algorithm}[t!]
\SetAlgoLined
%\nonl\textbf{Input:} Set of jobs $\mathcal{J}$ and servers $\mathcal{S}$, remaining execution time of each worker $U_s^g$ and of each job $V_j$. The upper bound execution time threshold $\theta$ and a constant $\lambda\geq 1$\;
\textbf{Input:} $\mathcal{J}$, $U_s^g$, $\hat{\rho}_j(\y^k)$, $u$, $\lambda_j$\;
\textbf{Initialization:} Let $U_s^g\leftarrow0,\forall g, s$\;

Sort jobs by $G_j$ in non-decreasing order\label{line:sort-J}, and denote as $\mathcal{J}^{s}$\;
$m \leftarrow T$, $\y \leftarrow \emptyset$, $left\leftarrow 1$, $right\leftarrow T$\;
\While {$left <= right$\label{line:bs}}{
	$\theta_u\leftarrow (left+right)/2$, $m_{\theta}\leftarrow T$, $\y_\theta\leftarrow \emptyset$\;
	\For {$\kappa = 1,2,\hdots,\max_jG_j$\label{line:kappa}}{
		$\y_{\theta}^k\leftarrow\emptyset$, m$_{\theta}^k\leftarrow -1$\;
		\For {$j = 1,2,\hdots,|\mathcal{J}^s|$\label{line:iterate}}{
			\If{$G_j\leq \kappa$\label{line:<=}}{
			 Return $\y_j$, $T_j$ using Algorithm~\ref{alg:ff}\label{line:ff}\;
		}
			\Else{
				Return $\y_j$, $T_j$ using Algorithm~\ref{alg:ls}\label{line:ls}\;
		}
			\If{$\y_j==\emptyset$\label{line:infeasible}}{
				break\;
			}
			$\y_{\theta}^k\leftarrow \y_{\theta}^k\cup \{\y_j\}$, $m_{\theta}^k\leftarrow \max\{\text{m}_{\theta}^k, T_j\}\label{line:k-update}$\;
		}
%		Record makespan$_{\theta}^k$ and scheduling $\y_{\theta}^k$\;
		
		\If{$m_{\theta}^k < m_\theta$\label{line:local-compare}}{
			$m_\theta \leftarrow m_{\theta}^k$, $\y_\theta\leftarrow\y_\theta^k$\label{line:theta-update}\;
		}
	}
%	\If{$\y_\theta==\emptyset$}{
%		$left\leftarrow \theta_u + 1$\;
%	}
	\If{$m_\theta < m$\label{line:global-compare}}{
		$m\leftarrow m_\theta$, $\y\leftarrow\y_\theta$\label{line:global-update}\;
		$right\leftarrow \theta_u - 1$\label{line:right-move}\;
	}
	\Else{
		$left\leftarrow \theta_u + 1$\label{line:left-move}\;
	}
}
\Return m, $\y$\;


\caption{\underline{S}mallest \underline{J}ob \underline{F}irst with \underline{B}alanced \underline{C}ontention and \underline{O}verhead (SJF-BCO).}
 \label{alg:place}
\end{algorithm} 

\begin{algorithm}[t!]
\SetAlgoLined
\textbf{Input:} A given job $j$, $\mathcal{S}$, $U_s^g$, $\hat{\rho}_j(\y^k)$, $u$, $\theta_u$\;
	$\mathcal{G}^{\theta_u}_{idle}\leftarrow$ available GPUs with execution time not exceed $\theta_u$\label{line:add}\;
%		\For{$s\in\mathcal{S}\label{line:count_start}$}{
%				\For{each GPU $g$ in server $s$}{
%					\If{$U_s^g < \theta_u$}{
%					$\mathcal{G}^{\theta_u}_{idle}\leftarrow\mathcal{G}^{\theta_u}_{idle} \cup \{g\}$\label{line:count_end}\;
%					}
%				}
%		}
	     \If{$|\mathcal{G}^{\theta_u}_{idle}|\geq G_j\label{line:enough}$}{
	         Pick top-$G_j$ workers with least $U_s^g$ from $\mathcal{G}^{\theta_u}_{idle}$ as $\y_j$\label{line:LS}\;
%	         Record completion time $t_j$ based on $\y_j$\;
		$T_j\leftarrow\arg\max_t\{y_{js}[t] > 0 | y_{js}[t]\in\y_j, \forall s, t\}$\label{line:t}\;
	         $U_s^g \leftarrow U_s^g + \hat{\rho}_j(\y^k)/u, \forall (g,s)\in\y_j\label{line:update-U}$\;
	         \Return $\y_j, T_j$\;
	     }
%	      \Return $\emptyset$\label{line:empty_ff}\;
	   \If{there exists running jobs\label{line:if-ff}}{
	   	Waiting for some job to exit and then goes to Line~\ref{line:add}\label{line:repeat-ff}\;
	   }
	   \Return $\emptyset, T$\;

\caption{Fragment-Aware First Fit Packing (FA-FFP).}
 \label{alg:ff}
\end{algorithm} 

 \begin{algorithm}[t!]
\SetAlgoLined
%\nonl\textbf{Input:} Set of jobs $\mathcal{J}$ and servers $\mathcal{S}$, remaining execution time of each worker $U_s^g$ and of each job $V_j$. The upper bound execution time threshold $\theta$ and a constant $\lambda\geq 1$\;
\textbf{Input:} A given job $j$, $U_s^g$, $\hat{\rho}_j(\y^k)$, $u$, $\lambda_j$\;
%\textbf{Initialization:} Let $U_s^g\leftarrow0,\forall g, s$\;
	    Sort the server set $\mathcal{S}$ by $\sum_gU_s^g/O_s$ in non-decreasing order, and choose the top $m$-servers s.t. $\sum_{s=1}^{m}O_s \geq \lambda_jG_j$, and denote the selected server set as $\mathcal{S}_{selected}$\label{line:sort-S}\;
	    $\mathcal{G}^{\theta_u}_{idle}\leftarrow \emptyset$\;
	    \For{$s\in\mathcal{S}_{selected}\label{line:for}$}{
	        Sort GPUs whose $U_s^g+\hat{\rho}_j(\y^k)/u\leq\theta_u$ by execution time in non-decreasing order, then append them to $\mathcal{G}^{\theta_u}_{idle}$\label{line:sort-U}\;
	     }
	        	\If{$|\mathcal{G}^{\theta_u}_{idle}| \geq G_j\label{line:gpus}$}{
	        Pick top-$G_j$ workers with least $U_s^g$ as $\y_j$\label{line:pick}\;
	        $T_j\leftarrow\arg\max_t\{y_{js}[t] > 0 | y_{js}[t]\in\y_j, \forall s, t\}$\;
	        $U_s^g\leftarrow U_s^g + \hat{\rho}_j(\y^k)/u, \forall (g,s) \in \y_j$\label{line:update-U-2}\;
	        \Return $\y_j, T_j$\label{line:return}\;
	    	}
%	\Return $\emptyset$\label{line:empty_ls}\;
	      \If{there are running jobs\label{line:if-ls}}{
	      	Waiting for some job to exit and then goes to Line~\ref{line:sort-S}\label{line:repeat-ls}\;
	      }
	      \Return $\emptyset, T$\label{line:return-ls}\;
\caption{Least Busy Server-GPU First (LBSGF).}
 \label{alg:ls}
\end{algorithm} 

In Algorithm~\ref{alg:place}, $U_s^g$ denotes the accumulative execution time of worker $g$ on server $s$.
We first sort jobs in non-decreasing order of their sizes $G_j$ in Line~\ref{line:sort-J}.
We search $\theta_u$ using the bisection method in the range $[1, T]$, and use the pair $(\theta_u,\kappa)$ to perform scheduling (Lines~\ref{line:bs}-\ref{line:kappa}).
We then iterate through each job (Line~\ref{line:iterate}).
If its size is not greater than the threshold $\kappa$ (Line~\ref{line:<=}), Algorithm~\ref{alg:ff} will be used to do the scheduling (Line~\ref{line:ff}); otherwise, Algorithm~\ref{alg:ls} will be called (Line~\ref{line:ls}).
%The allocation scheme will be returned if the job is successfully scheduled; otherwise, we will wait for some job to finish (Line~\ref{line:idle}).
If no feasible scheduling of job $j$ is returned, then we quit the current loop and update $\kappa$ (Line~\ref{line:infeasible}); otherwise, we will update the scheduling and makespan given the current $(\theta_u, \kappa)$ (Line~\ref{line:k-update}).
Upon finishing scheduling all jobs, we will update the schedule and makespan for the given $\theta_u$ if it has a smaller makespan (Lines~\ref{line:local-compare}-\ref{line:theta-update}).
%After exhausting all values of $\kappa$ for a given $\theta_u$, we will update the scheduling and makespan for the $\theta_u$ if it has a smaller makespan (Lines~\ref{line:local-compare}-\ref{line:theta-update}).
After exhausting all values of $\kappa$ for a given $\theta_u$, we will update the global makespan and the schedule if the current input $\theta_u$ has a better performance (Lines~\ref{line:global-compare}-\ref{line:global-update}).
Also, it indicates that we can further decrease the value of $\theta_u$ to find a potentially better schedule.
Thus, we search for the left half space by moving the right pointer (Line~\ref{line:right-move}); otherwise, we should increase the value of $\theta_u$ by moving the left pointer (Line~\ref{line:left-move}).
By scheduling workers as described in Algorithm~\ref{alg:place}, no worker's execution time will exceed the given limit $\theta_u$.
%In other words, the returned scheduling will not violate Constraint~(\ref{eqn:gpu_lp}).
%Note that we binary search $\theta_u$ in the range $[1, T]$, and paired with each possible value of $\kappa\in[1, \max_j G_j]$.
We denote the tightest execution time limit returned as $\tilde{\theta}_u$.




Algorithm~\ref{alg:ff} is based on the idea of ``fragment-aware first fit packing,'' where we first add all available GPUs whose $U_s^g+\hat{\rho}_j(\y^k)/u \leq \theta_u$ (Line~\ref{line:add}).
If there are enough available GPUs to schedule for job $j$'s workers (Line~\ref{line:enough}), we choose top-$G_j$ GPUs with least execution time first (Line~\ref{line:LS}).
We then evaluate the completion time of job $j$ (Line~\ref{line:t}) and update the corresponding GPUs' execution time (Line~\ref{line:update-U}); otherwise, we wait for some job to finish (Lines~\ref{line:if-ff}-\ref{line:repeat-ff}).
%The allocation scheme will be returned if the job is scheduled; otherwise, empty set will be returned (Line~\ref{line:empty_ff}).



Algorithm~\ref{alg:ls} is based on the idea of ``least busy server-GPU first,'' where we sort the servers by its GPU's average accumulative execution time (Line~\ref{line:sort-S}) and add the available GPUs whose execution time does not exceed $\theta_u$ in a non-decreasing order (Lines~\ref{line:for}-\ref{line:sort-U}).
Here, we introduce $\lambda_j\geq 1$ as a tuning parameter.
The smaller the $\lambda_j$ is, the fewer number of servers can be used.
If enough idle workers can be found, we schedule the job, evaluate its completion time, update the execution time of the chosen GPUs, and return the schedule (Lines~\ref{line:gpus}-\ref{line:return}); otherwise, we wait for some job to finish (Lines~\ref{line:if-ls}-\ref{line:repeat-ls}).
If there is no running job left, then return schedule $\emptyset$ and timespan $T$ (as makespan) to indicate the scheduling is infeasible (Line~\ref{line:return-ls}).
%The allocation scheme will be returned if the job is successfully scheduled; otherwise, empty set will be returned (Line~\ref{line:empty_ls}).



%\subsection{Extensions to More Advanced Models}\label{sec:extension}
%
%\begin{figure}[t!]
%    \centering
%%    \includegraphics[width=0.45\textwidth]{Figures/fig_communication_task.eps}
%    \includegraphics[width=0.48\textwidth]{Figures/fig_models_example.eps}
%    \caption{A three-layer example of model comparison.}
%    \label{fig:comparison}
%\end{figure}
%
%%It is worth noting that our work focus on the ``sequential model", i.e., communication and computation are performed in order (See Fig.~\ref{fig:comparison}(a)).
%Recall that Eqn.~(\ref{contention_model}) is calculated based on ``sequential model''~\cite{Zhang17:Poseidon} (See Fig.~\ref{fig:comparison}(a)), where FP, BP, RAR are executed in order.
%Specifically, it starts from the last layer to the initial layer in the BP , followed by RAR at $i^{th}$ iteration, then conduct FP from the first layer to the last layer at $(i+1)^{th}$ iteration.
%We can see from the figure that there is no overlap between computation and communication.
%Then more advanced models, i.e., wait-free model~\cite{Zhang17:Poseidon} (Fig.~\ref{fig:comparison}(b)) and priority-based model~\cite{Jayarajan19:P3} (Fig.~\ref{fig:comparison}(c)) are proposed, where the training time could be further reduced brought by the overlap.
%
%In the wait-free model, where layer $l$ can immediately perform RAR once it finishes BP, contributing to the overlap between BP and RAR.
%However, this model does not consider when the data will be used at the next iteration, and as a result, no overlap between FP and RAR exists.
%Thus, in the priority-based model, it assigns the highest priority to the initial layer, and the lowest priority to the last layer since it can immediately start FP at $(i+1)^{th}$ as soon as it receives the gradients of the first layer at $i^{th}$ iteration.
%In addition, higher priority layers can preempt lower priority layers, which further enables overlap between FP and RAR.
%%However, it can be easily extended to more advanced models that considers overlapping between communication and computation (e.g., wait-free model in Fig.~\ref{fig:comparison}(b), where layer $l$ can immediately start communication when it finishes backward pass).
%%By overlapping communication and computation, the per-iteration training time can be further reduced.
%
%Following the similar method in~\cite{Yu21:INFOCOM}, we could derive a unified analytical model on per-iteration training time to characterize all these models.
%In other words, Eqn.~(\ref{contention_model}) can still be derived by introducing some coefficients that used to capture the overlap properties.
%Here, to make this paper self-contained, we give a simple derivation for a model with $L$ layers.
%We use the subscript $l$ to indicate the gradient/parameter size at layer $l$.
%%More details can be found in~\cite{Yu21:INFOCOM}.
%The per-iteration training time according to Eqn.~(\ref{contention_model}) is:
%
%\begin{align*}
%\tau &= \frac{\frac{m}{w}\cdot2(w-1)}{b/f(\boldsymbol{\alpha}, k)}+\frac{\frac{m}{w}\cdot(w-1)}{C}+\gamma(\y)+ t^fM +t^b\\
%&= \frac{\frac{\sum_{l=1}^Lm_l}{w}\cdot2(w\!-\!1)}{b/f(\boldsymbol{\alpha}, k)}+\frac{\frac{\sum_{l=1}^Lm_l}{w}\cdot(w\!-\!1)}{C}+\gamma(\y)+ \sum_{l=1}^L(t_l^f +t_l^b)\\
%&=\sum_{l=1}^L\bigg(\underbrace{t_l^f}_{\text{FP}} + \underbrace{t_l^b}_{\text{BP}} + \underbrace{\frac{m_l (w-1)}{w\cdot C} + \frac{2m_l(w-1)f(\boldsymbol{\alpha}, k)}{w\cdot b}}_{\text{RAR: $t_l^c$}}\bigg)+\gamma(\y)\\
%&= \eta_1t^f + \eta_2t^b+\eta_3\bigg(\frac{\frac{m}{w}\cdot(w-1)}{C} + \frac{\frac{m}{w}\cdot2(w-1)}{b/f(\boldsymbol{\alpha}, k)}\bigg)+ \gamma(\y),
%\end{align*}
%where $\eta_1, \eta_2, \eta_3 \in(0, 1]$, which are served as reduction coefficients from the benefit of overlap.
%More details can be found in~\cite{Yu21:INFOCOM}.



\section{Performance Analysis}\label{sec:Performance}
In this section, we analyze the theoretical performance of SJF-BCO.
%Due to space limitation, %we provide proof sketches for some results in this section.
%We refer readers to our online technical report~\cite{Yu22:SJF-BCO_report} for the missing proofs. %or other proof details.
%First, we show the NP-Hardness of Problem~(\ref{problem:lp}) in Theorem~\ref{thm:np} based on the reduction to the vertex coloring problem (VCP). 
%%(see the proof in our online technical report \cite{??}).
%\begin{thm}\label{thm:np}
%Solving Problem~(\ref{problem:lp}) to within an $O(\frac{\log n_g}{2^{\sqrt{\log\log n_g}}})$-approximate ratio is NP-hard even when the exact processing time of each job is available (i.e., $l=u=1$), where $n_g=\max_j G_j$.
%\end{thm}
%\begin{proof}
%Here, we consider the special case with all jobs having a unit processing time ($\rho(\y^k)=1$).
%We first show that VCP can be reduced to the job scheduling problem in Problem~(\ref{problem:lp}) in polynomial time.
%Given an instance $I$ of VCP, i.e., given a graph $G=(V, E)$ with bounded degree $n_g$, we can construct our job scheduling problem as follows: i) For each node $v\in V$, we create a job $j_v\in\mathcal{J}$, where it has only one schedule $y_{j_v} = \emptyset$;
%% that no GPU is allocated yet; 
%ii) For each edge $(u, v)\in E$,  we add a worker $w_{u,v}$ to $\mathcal{S}$. Also, update the scheduling as $y_{j_u}=y_{j_u} \cup \{w_{u,v}\}$ and $y_{j_v}=y_{j_v} \cup \{w_{u,v}\}$.
%If the graph $G's$ maximum degree is no greater than $n_g$, then the maximum number of workers that can be allocated to each job is also $n_g$.
%
%With this reduction, we next show the solution of VCP can be translated to the solution of Problem~(\ref{problem:lp}), and vice verse.
%First, recall that each job has one unit processing time.
%Thus, all jobs should be executed inside a unit time interval ($[0, 1), [1, 2), \hdots$).
%If we have the solution to VCP, then we can schedule jobs with the same color in the same interval.
%Also, if we have the solution to the job scheduling problem, then the jobs in the same interval can be marked as the same color.
%Hence, finding an optimal solution of Problem~(\ref{problem:lp}) is equivalent to find an optimal solution of VCP.
%
%Similarly, given an instance of job scheduling, we can construct an instance of VCP, where the makespan equals to the number of colors.
%Therefore, if we have an $\alpha$-approximate solution to the job scheduling problem, we have an $\alpha$-approximate solution to VCP.
%However, 
%%it has known that finding a solution of $2^{O((\log K)^2)}$ colors for $K$-colorable graphs with degree at most $2^{2^{(\log K)^2}}$~\cite{Khot01:vertex-color} is NP-hard, i.e., 
%with the graph of degree at most $n_g$, it is known that coloring a $2^{\sqrt{\log\log n_g}}$-colorable graph with $O(\log n_g)$ colors is NP-Hard.
%This completes the proof.
%%Thus it is NP-hard to find a solution that is $O(\frac{\log n_g}{2^{\sqrt{\log\log n_g}}})$-approximate.
%\end{proof}
Specifically, we will establish the approximation ratio guarantee of our proposed SJF-BCO algorithm as follows:
%For better readability, we provide a roadmap of our proof, which contains several key steps (will be stated as lemmas): 

\begin{list}{\labelitemi}{\leftmargin=1.2em \itemindent=-0.0em \itemsep=.2em}
\item[1)] We first show in Lemma~\ref{lem:execution time} that the maximum execution time (i.e., $\hat{W}_{\max}^{\mathrm{Alg1}}$) returned by our algorithm is equal to $\tilde{\theta}_u$.
%has a upper bound related to the execution time limit $\tilde{\theta}_u$ and the ratio of $u/l$ in Lemma~\ref{lem:execution time}; 

\item[2)] We then prove that the makespan is $O(\hat{W}_{\max}^{\mathrm{Alg1}})$ in Lemma~\ref{lem:makespan}. 

\item[3)]  We further show that the gap between $\tilde{\theta}_u$ and the tightest execution time limit $\theta_u^*$ returned by some offline optimal algorithm in the right-hand-side (RHS) of \eqref{eqn:gpu_lp} is bounded in Lemma~\ref{lem:wk_gap}. %Since we need to bound the gap between the optimal makespan and the makespan  We returned,
\end{list}
Finally, by putting all these lemmas together, we arrive at the approximation ratio result stated in Theorem~\ref{thm:ratio}.

\begin{lem}[Maximum Execution Time Upperbound]\label{lem:execution time}
Algorithm~\ref{alg:place} produces a schedule with the maximum execution time $\hat{W}_{\max}^{\mathrm{Alg1}} =\tilde{\theta}_u$.
\end{lem}

\begin{proof}%[Proof Sketch]
Note that in Algorithm~\ref{alg:place}, we can obtain a schedule such that the execution time of every worker will not exceed $\tilde{\theta}_u$,
%Note that $\tilde{\theta}_u$ is the tightest value found by Alg.~\ref{alg:place}, and it is equal to $\hat{W}_{\max}^{\mathrm{Alg1}}$ in the LHS of \eqref{eqn:gpu_lp}.
i.e., $\sum_j\sum_k x_j^k\frac{\hat{\rho}_j(\y^k)}{u}\leq \tilde{\theta}_u$, $\forall g$ (cf. Line~2 in Algorithm~\ref{alg:ff} and Line~5 in Algorithm~\ref{alg:ls}).
Note that $\tilde{\theta}_u$ is the tightest value found by Alg.~\ref{alg:place} since we will keep decreasing its value in the RHS of \eqref{eqn:gpu_lp} until it becomes equal to $\hat{W}_{\max}^{\mathrm{Alg1}}$ in the LHS of \eqref{eqn:gpu_lp}.
%That is, $\hat{W}_{\max}^{\mathrm{Alg 1}}= \tilde{\theta}_u$,
%which is equal to $\hat{W}_{\max}^{\mathrm{Alg1}}$.
It then follows that:
\begin{align*}
\hat{W}_{\max}^{\mathrm{Alg 1}} = \max_{g\in\mathcal{N}}\sum_{j\in\mathcal{J}}\sum_{k\in\{1,\hdots,|\mathcal{Y}|\}}x_j^k\frac{\hat{\rho}_j(\y^k)}{u} = \tilde{\theta}_u.
\end{align*}
%and the proof is complete.
Thus, we can have the maximum execution time $\hat{W}_{\max}^{\mathrm{Alg1}}$ is equal to $\tilde{\theta}_u$, and the proof is complete.
\end{proof}


%In the following analysis, we consider the case where $\kappa=n_g$, i.e., we schedule the jobs with the FA-FFP approach (Algorithm~\ref{alg:ff}).
%Recall that given $\theta_u$, SJF-BCO exhausts all values of $\kappa\in[1,n_g]$, and the best makespan found will be returned.
%Thus, the actual performance produced by SJF-BCO is at least as good as the following results stated in Lemmas~\ref{lem:makespan}--\ref{lem:wk_gap} and Theorem~\ref{thm:ratio}.

\begin{lem}[Makespan Upperbound]\label{lem:makespan}
Algorithm~\ref{alg:place} achieves a makespan at most $n_g\hat{W}^{\mathrm{Alg1}}_{\max}$, where $n_g$ is defined as in Theorem~\ref{thm:np}. %under the gang-scheduling discipline
\end{lem}

\begin{proof}%[Proof Sketch]
%We let $\mathcal{G}(\q_j^k)$ be the set of GPUs allocated when using scheduling $\q_j^k$.
To bound the makespan, we need to attain upper bounds of the total {\it busy} and {\it idle} time for each worker. %since the synchronous training can lead to worker idle status.
Recall that due to the synchronous gang scheduling for training, the worker may wait for other workers to finish executing other jobs before it could start processing the current job, which may result in idling.
First, we can have the total busy time $T_g^{\mathrm{busy}}\leq \hat{W}^{\mathrm{Alg1}}_{\max}\overset{\mathrm{Lem.}~\ref{lem:execution time}}{=}\tilde{\theta}_u$. 
Next, we work on bounding the total idle time $T_g^{\mathrm{idle}}$.

For any worker $g\in\mathcal{N}$, we use $g_j$ to denote the last job $j$ on $g$.
Suppose job $j$ follows schedule $\y^k$.
At any time slot $t$ before worker $g$ processes job $j$, there are two cases: i) worker $g$ is occupied by other jobs (i.e., $g$ is busy); ii) worker $g$ is idle, but at least one worker $g'\in\mathcal{G}_j(\y^k)$ is busy with executing other jobs.
Since we consider the gang-scheduling discipline, 
%where the job will be scheduled immediately once all its workers are available, 
the job cannot be delayed if there is a sufficient number of GPUs available as requested.
%it is impossible to have the case that all its required workers are available and yet the job is not started in time slot $t$.
%We observe that at any time $t$ that worker $g$ is idle (case ii), we must can find at least one busy worker $g'\in\mathcal{G}_j(\y^k)$.
%To calculate the idle time of worker $g$, we can calculate the busy time of worker $g'$ instead.
Thus we have:
\begin{align*}
T_g^{\mathrm{idle}} \overset{\mathrm{(a)}}{\leq}\!\!\!\!\sum_{g'\in\mathcal{G}_j(\y^k)|g'\neq g}\!\!\!\!T_{g'}^{\mathrm{busy}}\overset{}{\leq}\sum_{g'\in\mathcal{G}_j(\y^k)|g'\neq g}\!\!\!\!\hat{W}^{\mathrm{Alg 1}}_{\max}\overset{\mathrm{(b)}}{\leq}(G_j\!-\!1)\hat{W}^{\mathrm{Alg 1}}_{\max},
\end{align*}
where (a) follows from the fact that in any time slot $t$ that worker $g$ is idle (case ii), we must be able to find at least one busy worker $g'\in\mathcal{G}_j(\y^k)$.
To calculate the idle time of worker $g$, we can calculate the busy time of worker(s) $g'\in\mathcal{G}_j(\y^k)$ instead, and the limit of each worker's busy time is $\hat{W}_{\max}^{\mathrm{Alg1}}$.
%\textcolor{red}{Specifically, the max idle time of worker g is the summation of all the busy workers $g'\in\mathcal{G}_j(\y^k)$.}
%If multiple workers in $\mathcal{G}_j(\y^k)$ are busy, we can randomly pick one of them as $g'$.
Also, (b) follows from the fact that at most $G_j-1$ number of GPUs (except worker $g$)  are busy. %in time-slot $t$.
Then, we can upper bound the makespan $T^{\mathrm{total}}$ as:
\begin{align*}
T^{\mathrm{total}} &= \max_{g\in\mathcal{N}}(T_g^{\mathrm{busy}} + T_g^{\mathrm{idle}})\leq  \max_{j\in\mathcal{J}}\bigg(\hat{W}_{\max}^{\mathrm{Alg 1}} + (G_j-1)\hat{W}_{\max}^{\mathrm{Alg1}}\bigg)\\
&=\max_{j\in\mathcal{J}}G_j\hat{W}_{\max}^{\mathrm{Alg 1}}= n_g\hat{W}_{\max}^{\mathrm{Alg 1}},%\footnotemark.
\end{align*}
and the proof is complete.
%\footnotetext{It is worth noting that $W_{\max}$ is algorithm-dependent. In other words, the upper bound execution time varies with different algorithms.}
%Thus we conclude the proof.
\end{proof}

Next, we characterize the gap between the maximum execution time limit $\tilde{\theta}_u$ and the optimal execution time $\theta^*_u$ in the RHS of \eqref{eqn:gpu_lp}.

\begin{lem}\label{lem:wk_gap}
The maximum execution time $\tilde{\theta}_u$ returned by Algorithm~\ref{alg:place} satisfies $\tilde{\theta}_u\leq \varphi\frac{u}{l}\cdot\theta^*_u$, where $\varphi=\max_j\frac{\rho_j(\y^{k_1})}{\rho_j(\y^{k_2})}, \forall k_1, k_2$.
%, where $n_g$ is defined as in Theorem~\ref{thm:np} and $\varphi$ is defined in Section~\ref{sec:alg}.
\end{lem}

\begin{proof}%[Proof Sketch]
Let $k^*$ and $\tilde{k}$ be the schedule indices chosen by solving Problem~(\ref{problem:lp}) optimally and Algorithm~\ref{alg:place}, respectively.
Let $\mathcal{G}(\y^{k})$ be the set of selected GPUs if schedule $\y^k$ is used.
%Let $\tilde{\pi}$ and $\pi^*$ represent the offline optimal algorithm and algorithm SJF-BCO, respectively.
%Then we can bound $W_{\max}^{\tilde{\pi}}$ as follows:
%Note that the maximum execution time $\tilde{\theta}_u$ is the tightest value found by Algorithm~\ref{alg:place}, which is equal to $\hat{W}_{\max}^{\mathrm{Alg1}}$.
We have
\begin{align*}
\tilde{\theta}_u &\overset{\mathrm{Lem.~\ref{lem:execution time}}}{=} \max_{g\in\mathcal{G}(\y^{\tilde{k}})} \sum_{j\in\mathcal{J}}\frac{\hat{\rho}_j(\y^{\tilde{k}})}{u}\overset{\mathrm{(a)}}{\leq} \max_{g\in\mathcal{G}(\y^{\tilde{k}})} \sum_{j\in\mathcal{J}}\frac{\varphi\frac{u}{l}\hat{\rho}_j(\y^{k^*})}{u}\\
&\overset{\mathrm{(b)}}{\leq} \max_{g\in\mathcal{G}(\y^{k^*})} \sum_{j\in\mathcal{J}}\frac{\varphi\frac{u}{l}\hat{\rho}_j(\y^{k^*})}{u} \overset{\mathrm{Eq.}~\eqref{eqn:gpu_lp}}{\leq} \varphi\frac{u}{l}\theta^*_u.
%W_{\max}^{\tilde{\pi}} = \max_{g\in\mathcal{N}}\sum_{j\in\mathcal{J}} \hat{W}_{jg}^{\tilde{k}}=\max_{g\in\mathcal{N}} \sum_{j\in\mathcal{J}}\frac{\hat{\rho}_j(\q^{\tilde{k}})}{u}\leq \max_{g\in\mathcal{N}} \sum_{j\in\mathcal{J}}\frac{\hat{\rho}_j(\q^{k^*})}{u}
\end{align*}
To see why (a) holds, recall that for any schedule $\y^k$, we have $\hat{\rho}_j(\y^k)\in[l\rho_j(\y^k), u\rho_j(\y^k)]$.
Then, for any two different schedules $\y^{k_1}$ and $\y^{k_2}$, we can calculate the worst-case ratio as $\frac{\hat{\rho}_j(\y^{k_1})}{\hat{\rho}_j(\y^{k_2})}\leq \frac{u\rho_j(\y^{k_1})}{l\rho_j(\y^{k_2})}\leq\varphi\frac{u}{l}$.
%To prove the last equality, we first derive the $\tau_j[t]$
%We let $t^c_j$, $t^a_j$, $t^1_j$ and $t^2_j$ be the average per-iteration computation time, without overhead all-reduce time, contention and communication overhead of job $j$, respectively.
%Recall that we set $\kappa=n_g$, then for any job $j$, FA-FFP will be called to schedule its workers since Line~\ref{line:<=} in Algorithm~\ref{alg:place} is always satisfied.
%In FA-FFP, it will choose top-$G_j$ GPUs with least execution time first to schedule job $j$ server by server (Line~\ref{line:LS}).
%In other words, the maximum concurrent number of different jobs is two and the maximum number of servers used is $G_j$, i.e., $\frac{\hat{\rho}_j({\y^{k_1}})}{\hat{\rho}_j({\y^{k_2}})}\leq \frac{F_j(t^c_j + t^a_j + 2t^1_j+G_j\cdot t^2_j)}{F_j(t^c_j + t^a_j + t^1_j+t^2_j)}\leq n_g$, $\forall k_1, k_2$, based on the reasonable assumption that $n_g\geq 2$.
The inequality in (b) can be established as follows.
First, note that $\tilde{k}$ is chosen using the {\it least execution time first} scheduling strategy in Algorithm~\ref{alg:ff} (Line~\ref{line:LS}).
Then, we have $\max_{g\in\mathcal{G}(\y^{\tilde{k}})} \sum_{j\in\mathcal{J}}\frac{\hat{\rho}_j(\y^{\tilde{k}})}{u}\leq \max_{g\in\mathcal{G}(\y^{k})} \sum_{j\in\mathcal{J}}\frac{\hat{\rho}_j(\y^{k})}{u}$, $\forall k$, which can be proved by contradiction as follows.
Suppose there exists $g\in\mathcal{G}(\y^{k})\setminus \mathcal{G}(\y^{\tilde{k}})$ such that $\sum_{j\in\mathcal{J}}\frac{\hat{\rho}_j(\y^{k})}{u}\leq \sum_{j\in\mathcal{J}}\frac{\hat{\rho}_j(\y^{\tilde{k}})}{u}$, $\forall g'\in\mathcal{G}(\y^{\tilde{k}})$.
However, we know that $\tilde{k}$ chooses the GPUs with the least execution time first, i.e., $g$ should be in $\mathcal{G}(\y^{\tilde{k}})$, which contradicts our assumption.
This completes the proof.
\end{proof}

%Finally, by combining Lemmas~\ref{lem:execution time} and \ref{lem:makespan}, we have the following approximation ratio for Algorithm~\ref{alg:round}.
Finally, by putting everything together, we have the following approximation ratio for our proposed approach:
\begin{thm}[Approximation Ratio]\label{thm:ratio}
Alg.~\ref{alg:place} is $n_g\varphi\frac{u}{l}$-approximate.
%Our proposed algorithm is $n_g(1+2\lambda ln\frac{2N}{\delta})$-approximate.
%with probability at least $1-\delta$.
\end{thm} 
\begin{proof}
We use $T^*$ to denote the optimal makespan that produced by some offline optimal algorithm.
It then follows that
%\begin{align*}
%T^{total}&\overset{Lem.\ref{lem:makespan}}{\leq}n_gW_{\max}\overset{Lem.\ref{lem:execution time}}{\leq}n_g(1+2\lambda ln(\frac{2N}{\delta}))\theta^*\\
%&\overset{(d)}{\leq}n_g(1+2\lambda ln(\frac{2N}{\delta}))T^{total*},
%\end{align*}
\begin{align*}
T^{total}&\overset{\mathrm{Lem.}\ref{lem:makespan}}{\leq}n_g\hat{W}^{\mathrm{Alg1}}_{\max}\overset{\mathrm{Lem.}\ref{lem:execution time}}{=}n_g\tilde{\theta}_u\overset{\mathrm{Lem.}\ref{lem:wk_gap}}{\leq}n_g\varphi\frac{u}{l}\theta^*_u\overset{\mathrm{(a)}}{\leq}n_g\varphi\frac{u}{l}T^{*},
\end{align*}
where (a) is due to Problem~(\ref{problem:lp}) estimates the processing time as $\frac{\hat{\rho}_j(\y^k)}{u}$ without considering potential idling (caused by synchronization barrier), which implies $\theta^*_u\!\leq\!T^{*}$.
This completes the proof.
\end{proof}

\begin{remark}{\em
Note that the result in Theorem~\ref{thm:ratio} does not depend explicitly on the parameter $\kappa$ in SJF-BCO.
%This is because the maximum execution time limit $\tilde{\theta}_u$ (equivalent to maximum execution time $\hat{W}_{\max}^{\mathrm{Alg1}}$, see Lem.~\ref{lem:execution time}) is influenced by $\kappa$.
%Since we exhaust all possible $\kappa$-values (Line~\ref{line:kappa}),
%Even the approximation ratio has no $\kappa$ included, 
This is because Theorem~\ref{thm:ratio} is only a worst-case upper bound that depends on $\tilde{\theta}_u$, which in turn depends on $\kappa$.
Hence, $\kappa$ is implicitly captured in Theorem~\ref{thm:ratio}. 
%it is implicitly coupled in the ratio $u/l$ since we choose their values to cover all possible $\hat{W}_{\max}^{\mathrm{Alg1}}$, which is determined by $\kappa$.
%Note that the approximation ratio is related to the estimation error ratio $u/l$, and the range of per-iteration training time $\varphi$.
%Recall that in Algorithm~\ref{alg:place}, the maximum execution time limit $\tilde{\theta}_u$ that is equivalent to maximum execution time $\hat{W}_{\max}^{\mathrm{Alg1}}$ (see Lem.~\ref{lem:execution time}) is influenced by $\kappa$ since we exhaust all its possible values (Line~\ref{line:kappa}).
%Even the approximation ratio has no $\kappa$ included, it is implicitly coupled in the ratio $u/l$ since we choose their values to cover all possible $\hat{W}_{\max}^{\mathrm{Alg1}}$, which is determined by $\kappa$.
}
\end{remark}

\begin{thm}[Polynomial Running Time]\label{thm:time}
Time complexity of SJF-BCO is $O(n_g|\mathcal{J}|N\log N\log T)$, where $n_g$ is defined as in Thm.~\ref{thm:np}.
\end{thm}
\begin{proof}
The sorting operation plays a dominant role in the total running time in Algorithm~\ref{alg:place}.
For each job $j$, if $G_j\leq\kappa$, we need to sort all GPUs in the cluster, which takes $O(N\log N)$ time in order to choose top-$G_j$ workers with least execution time first in Algorithm~\ref{alg:ff} (Line~\ref{line:LS}).
Otherwise, we only need to sort servers, which takes $O(S\log S)$ time in order to choose top-$m$ servers as in Algorithm~\ref{alg:ls} (Line~\ref{line:sort-S}).
Thus, it takes $O(N\log N)$ time to schedule each job since $N > S$.
Then, for all the jobs to be scheduled given ($\theta_u, \kappa$), it has $O(|\mathcal{J}|N\log N)$ time complexity.
%Then it takes $O(|\mathcal{J}|N\log N)$ for all the jobs to be scheduled given ($\theta_u, \kappa$).
Recall that we use bisection to search $\theta_u$, where each iteration contains an inner loop indexed by $\kappa\!\in\![1, n_g]$.
This implies a total of $n_g\log T$ trials.
Thus, the overall time complexity is $O(n_g|\mathcal{J}|N\log N\log T)$.
\end{proof} 
 
 










==> MobiHoc'22_Communication_Contention_Tech_Report/Sec5_Algorithm/Sec5_Algorithm_backup.tex <==
% !TEX root = ../ML_Networking_INFOCOM'20.tex

\section{Solution Approach and Problem Reformulation} \label{sec:alg}
In this section, we describe the key components of our scheduling algorithm design for solving Problem~DDLJS, which is structured into tree steps from Sections...
We present the theoretical performance results in Section...

% \subsection{Handling Non-Deterministic Eqn.~(\ref{eqn:k_j})}
\subsection{Challenges in Solving Problem~DDLJS}
The first obstacle to solve Problem~DDLJS stems from the non-deterministic structure in constraint~(\ref{eqn:k_j}).
We let 
\begin{align}
\label{eqn:xjs2}x_{js}\!=\!\begin{cases}
\mathbbm{1}\{1\leq y_{js}\leq G_{j}-1\}, \forall s\!\in\!\mathcal{S}, j\!\in\!\mathcal{J}, &\hspace{-0.1in}\text{if }G_j\!>\!1,\\
0,&\hspace{-0.1in}\text{if }G_j\!=\!1.
\end{cases}
\end{align}
%$x_{js}\triangleq\mathbbm{1}\{1\leq y_{js}\leq G_{j}-1\}, \forall s\in\mathcal{S}, j\in\mathcal{J}$.
We observe that $k_j=0$ only if $y_{js}=G_j,\exists s\in\mathcal{S}$, which corresponds to intra-connect communication jobs (single-GPU job is the special case).
The maximum number of inter-connect communication jobs over all servers $p_j$ can be computed as $\max_{s\in\mathcal{S}}\sum_{j'\in\mathcal{J}} x_{j's}$. 
Notice that $x_{js}$ will be increased by one only if $y_{js}\in[1,G_{j}-1],\forall s\in\mathcal{S}, j\in\mathcal{J}$ and $G_j\neq 1$.
With the linear proportional assumption, we can have the following equivalent formulation for constraint~(\ref{eqn:k_j}):
\begin{align*}
    k_j=\begin{cases}
    0, \quad \text{if } y_{js}=G_j, \exists s\in\mathcal{S},\\
    \alpha \max_{s\in\mathcal{S}}\sum_{j'\in\mathcal{J}}x_{j's}, \quad \text{o.w.}
    \end{cases}
\end{align*}
We can see that $k_j=0$ implies $x_{js}=0$ since $y_{js}=G_j, \exists s\in\mathcal{S}$. 
%and for the special case when $G_j=1$, $x_{js}=0$ still holds.
Since $x_{js}\geq 0$ and $\alpha\in(0,1)$, we can further simplify $k_j$ as follows:
\begin{align*}
    k_j=\alpha\max_{s\in\mathcal{S}}\sum_{j'\in\mathcal{J}}x_{j's}.
\end{align*}
% We can see from the above equation that $k_j$ with initial value $0$ will only be increased by one when some server $s$ is scheduled to place GPUs from job $j$ but it does not contain all its GPUs.
We can see from the above equation that $k_j$ involves the "max`` structure, which can be removed  by the following equivalent transformation:
\begin{align}
    \label{eqn:k_j_reformulate}&k_j\geq \alpha\sum_{j'\in\mathcal{J}}x_{j's}, \quad \forall s\in\mathcal{S}, j\in\mathcal{J}.
    % &k_j\geq 0,\quad \forall j\in\mathcal{J}\nonumber.
\end{align}

% \subsection{Handling Indicator Functions in Eqns.~(\ref{eqn:k_j})(\ref{eqn:chi_s})}
After solving the non-deterministic structure in Eqn.~(\ref{eqn:k_j}), it still remains difficult to directly solve Problem~DDLJS due to the indicator functions in Eqns.~(\ref{eqn:k_j})(\ref{eqn:chi_s}).
In the literature, a commonly used technique is to use big-$M$ to reformulate indicator function to a series of linear constraints, and solve it using LP solver.
However, it is well-known that indicator constraints present the drawback of having a weak continuous relaxation, and might lead to numerical issues \cite{Belotti16:indicatorfunction}.
In order to circumvent the limitations, we observe that the original problem~(\ref{Problem:primal}) can be converted into the following equivalent formulation, where we interpret it from the perspective of GPU instead of job placement.

\subsection{Problem Reformulation}
We use $\mathcal{G}_j$ to denote the set of GPUs that required by user $j$.
Recall that $|\mathcal{G}_j|=G_j$.
We let $z_{jgs}, \forall g\in\mathcal{G}_j,s\in\mathcal{S}, j\in\mathcal{J}$ encode the placement scheme of job $j$, where $z_{jgs}=1$ if server $s$ is selected to host GPU $g$ of job $j$; otherwise it is $0$.
We first simply the objective function as follows:
%We further can simply the objective function as follows:
\begin{align*}
&c\sum_{j\in\mathcal{J}}F_jt_j+\mu\sum_{s\in\mathcal{S}}(N_s\chi_s-\sum_{j\in\mathcal{J}}\sum_{g\in\mathcal{G}_j}z_{jgs})\\
&=c\sum_{j\in\mathcal{J}}F_j(d_j+h_jk_j)+\mu\sum_{s\in\mathcal{S}}N_s\chi_s-\mu\sum_{s\in\mathcal{S}}\sum_{j\in\mathcal{J}}\sum_{g\in\mathcal{G}_j}z_{jgs}\\
&=c\sum_{j\in\mathcal{J}}F_jd_j+c\sum_{j\in\mathcal{J}}F_jh_jk_j-\mu\sum_{j\in\mathcal{J}}G_j+\mu\sum_{s\in\mathcal{S}}N_s\chi_s
\end{align*}

We use $\gamma_{js}$ to denote whether any GPU of job $j$ is allocated to server $s$ ($\gamma_{js}=1$) or not ($\gamma_{js}=0$).
Then our original problem can be reformulated as the following equivalent problem:
\begin{align}
   \underset{\mathbf{z,x,k,\chi}} {\text{Minimize }} &c\sum_{j\in\mathcal{J}}F_jh_jk_j+\mu\sum_{s\in\mathcal{S}}N_s\chi_s\label{Problem:primal}\\
    \text{subject to }
    &\sum_{s\in\mathcal{S}}z_{jgs}=1, \quad\forall j\in\mathcal{J}, g\in\mathcal{G}_j,\label{eqn:gpu2}\\
    &\sum_{j\in\mathcal{J}}\sum_{g\in\mathcal{G}_j}z_{jgs}\leq N_s,\quad\forall s\in\mathcal{S},\label{eqn:cap2}\\
%    &\chi_{s}\geq z_{jgs}, \quad\forall j\in\mathcal{J}, g\in\mathcal{G}_j, s\in\mathcal{S},\label{eqn:chi_s2}\\    
    &\gamma_{js}\geq z_{jgs}, \quad \forall  j\in\mathcal{J}, g\in\mathcal{G}_j, s\in\mathcal{S},\label{eqn:gamma}\\
    &\chi_{s}\geq \gamma_{js}, \quad\forall j\in\mathcal{J}, s\in\mathcal{S},\label{eqn:chi_s2}\\
    &x_{js}\geq \gamma_{js}-z_{jgs}, \quad \forall j\in\mathcal{J}, g \in\mathcal{G}_j, s\in\mathcal{S},\label{eqn:xjs}\\
%    &x_{js}\geq z_{jgs}\!-\!z_{jg's}, \forall j\in\mathcal{J}, g,g'\!\in\!\mathcal{G}_j, s\!\in\!\mathcal{S},\label{eqn:xjs}\\
    &z_{jgs}, x_{js},\chi_s,\gamma_{js}\in\{0,1\}, k_j\geq 0,\nonumber\\
    &\hspace{1.2in}\forall j\in\mathcal{J}, g\in\mathcal{G}_j, s\in\mathcal{S},\label{eqn:int2}\\
    &\text{Constraint}~(\ref{eqn:k_j_reformulate})\nonumber.
\end{align}

Note that in the objective, we further omit the constants terms, which does not affect the optimal solutions derived by solving the above problem.
Constraint~(\ref{eqn:gpu2}) ensures that each job's GPU is placed to exactly one server, which guarantees exactly $G_j$ workers will be scheduled to job $j$.
Constraint~(\ref{eqn:cap2}) ensures that the total number of GPUs scheduled over all jobs to server $s$ should not exceed its capacity.
Constraint~(\ref{eqn:gamma}) indicates whether any GPU of job $j$ is placed to server $s$.
Constraint~(\ref{eqn:chi_s2}) indicates the server $s$ is chosen (i.e., $\chi_s=1$) as long as some job places its GPU to it, implying $\sum_{j\in\mathcal{J}}y_{js}\geq 1$.
Constraint~(\ref{eqn:xjs}) is equivalent to Eqn.~(\ref{eqn:xjs2}) (refer to Lemma~\ref{lem:equivalence}).


\begin{lem}\label{lem:equivalence}
Problem~DDLJS and Problem~(\ref{Problem:primal}) are equivalent, i.e., a feasible solution to the former has a corresponding same feasible solution to the latter, and vice verse.
\end{lem}
\begin{proof}
First, it is obvious that Constraints~(\ref{eqn:gpu2}) and (\ref{eqn:cap2}) are equivalent to Constraints~(\ref{eqn:gpu}) and (\ref{eqn:cap}), respectively.

Next, we show the equivalence between Constraints~(\ref{eqn:gamma})(\ref{eqn:chi_s2}) and (\ref{eqn:chi_s}). 
We can know that $\chi_s\geq \gamma_{js}\geq z_{jgs}$, thus we only need to show it is equivalent to Eqn.~(\ref{eqn:chi_s}). 
On one hand, we know that as long as there exists some job $j$ that places its GPU to the server $s$, i.e., $z_{jgs}=1$, then $\sum_jy_{js}\geq 1$ since $y_{js}\geq1$.
On the other hand, from Constraint~(\ref{eqn:chi_s}), we know that as long as server $s$ is chosen to schedule GPUs,
i.e., $\sum_jy_{js}\geq 1$, then there must exist some job $j$ that schedules its GPU $g$ to the server $s$, implying $z_{jgs}=1$.
Thus, the equivalence between these two constraints are proved.

Lastly, we show that Constraint~(\ref{eqn:xjs}) is the same as Eqn.~(\ref{eqn:xjs2}).
We consider the following three cases for job $j$:

%{\em 1) }The job only requires one GPU (i.e., $G_j=1$), then $z_{jg's}=z_{jgs}$, which implies that $x_{js}\geq 0$ based on Constraint~(\ref{eqn:xjs}), meaning $x_{js}$ can be $0$ or $1$.
%However, In order to minimize the objective value, the system tends to minimize $k_j$ that decreases as $x_{js}$ decreases, and as a result, $x_{js}$ will be set to $0$.
%% which comply with $\mathbbm{1}\{1\leq y_{js}\leq G_j-1\}$.
%
%{\em 2) }There exists some server $s$ that host all its workers (i.e., $y_{js}=G_j$ and $G_j>1$), then $z_{jgs}=1, \forall g\in\mathcal{G}_j$, which implies that $x_{js}\geq 0$. 
%%based on Constraint~(\ref{eqn:xjs}), meaning $x_{js}$ can be $0$ or $1$.
%And with the same reason in case {\em 1)}, $x_{js}$ will be set to $0$.
%
%{\em 3) }There exists at lease two servers to host its workers (i.e., $1\leq y_{js}\leq G_j-1, \forall s\in\mathcal{S}_j$ and $G_j>1$), then $z_{jgs}-z_{jg's}=1, \exists g,g'\in\mathcal{G}_j, s\in\mathcal{S}_j$, implying $x_{js}\geq 1$, and as a result, $x_{js}$ will be set to $1$.

{\em 1) }The job only requires one GPU (i.e., $G_j=1$), then $\gamma_{js}=1$ and $\gamma_{js}-z_{jgs}=0$, which implies that $x_{js}\geq 0$ based on Constraint~(\ref{eqn:xjs}), meaning $x_{js}$ can be $0$ or $1$.
However, In order to minimize the objective value, the system tends to minimize $k_j$ that decreases as $x_{js}$ decreases, and as a result, $x_{js}$ will be set to $0$.
% which comply with $\mathbbm{1}\{1\leq y_{js}\leq G_j-1\}$.

{\em 2) }There exists some server $s$ that host all its workers (i.e., $y_{js}=G_j$ and $G_j>1$), then $z_{jgs}=1, \forall g\in\mathcal{G}_j$, which implies that $x_{js}\geq 0$. 
%based on Constraint~(\ref{eqn:xjs}), meaning $x_{js}$ can be $0$ or $1$.
And with the same reason in case {\em 1)}, $x_{js}$ will be set to $0$.

{\em 3) }There exists at lease two servers to host its workers (i.e., $1\leq y_{js}\leq G_j-1, \forall s\in\mathcal{S}_j$ and $G_j>1$), then $\gamma_{js}-z_{jgs}=1, \exists g\in\mathcal{G}_j, s\in\mathcal{S}_j$, implying $x_{js}\geq 1$, and as a result, $x_{js}$ will be set to $1$.


We can see from all the cases above that $x_{js}$ in Constraint~(\ref{eqn:xjs}) is $1$ if and only if $x_{js}$ in Eqn.~(\ref{eqn:xjs2}) is $1$, and vice verse, and the proof is complete.
\end{proof}
% Several remarks for Lemma~\ref{lem:equivalence} are in order:
Notice that the first two cases correspond to jobs that use intra-connect communication, which will not introduce resource contention between servers; while the last case involves inter-connect communication, which needs to be counted to the concurrent number of communication tasks.







% Recall that $x_{j's}$ is $0$ only when $y_{j's}=0$ or $y_{j's}=G_{j'}$; otherwise it is $1$.
% We let $l_{js}\triangleq\{y_{js}\geq 1\}$, and let $u_{js}\triangleq\{y_{js}\leq G_j-1\}$.
% We first convert the indicator function as follows:
% \begin{align}
%     &y_{js}\geq 1+G_j(l_{js}-1), \forall s\in\mathcal{S}, j\in\mathcal{J},\label{eqn:y1}\\
%     &y_{js}\leq G_j-1+G_j(1-u_{js}),\forall s\in\mathcal{S}, j\in\mathcal{J},\label{eqn:y2}\\
%     &x_{js}\leq l_{js},\forall s\in\mathcal{S}, j\in\mathcal{J},\label{eqn:x1}\\
%     &x_{js}\leq u_{js}, \forall s\in\mathcal{S}, j\in\mathcal{J}\label{eqn:x2},\\
%     &l_{js},u_{js}, x_{js}\in\{0,1\},\forall s\in\mathcal{S}, j\in\mathcal{J}\label{eqn:lux}.
% \end{align}
% From Eqn.~(\ref{eqn:y1}), we have $l_{js}=0$ when $z_{js}=0$; similarly, from Eqn.~(\ref{eqn:y2}), we have $u_{js}=0$ when $z'_{js}=G_j$.
% And Eqns.~(\ref{eqn:x1})(\ref{eqn:x2}) imply that $x_{js}=\min\{l_{js},u_{js}\}$.
% In other words, $x_{js}=0$ only if both $l_{js}=0$ (corresponds to the case that no job $j$'s GPUs are placed to the server $s$) and $u_{js}=0$ (corresponds to the case that all job $j$'s GPUs are placed to the server $s$), which comply with the calculation of $k_j$ since no resource contention is introduced under these two cases.
% Notice that single-GPU jobs will never compete for the bandwidth with other jobs, meaning $x_{js}$ should be $0$ for the server $s$ where its GPU is scheduled.
% Under this case, $x_{js}=\mathbbm{1}\{1\leq y_{js}\leq 0\}$, which is impossible to be satisfied, implying $x_{js}=0$.
% Thus, it is still valid even with special case that jobs only require one GPU.
% % In addition, we can infer from Eqns.~(\ref{eqn:x1}) and (\ref{eqn:x2}) that

% % \begin{align}
% %     &k_j\leq \alpha\sum_{j'\in\mathcal{J}}l_{j's},\forall j\in\mathcal{J},\label{eqn:k_j_up1}\\
% %     &k_j\leq \alpha\sum_{j'\in\mathcal{J}}u_{j's},\forall j\in\mathcal{J}\label{eqn:k_j_up2},
% % \end{align}
% % which we obtain the upper bound of $k_j$, and as a result, the objective value will still be bounded.

% We notice that  $\sum_{j\in\mathcal{J}}y_{js}\geq 1$ as long as the server $s$ is chosen by some job $j$, which is associated with $x_{js}$.
% However, $x_{js}=0$ when $y_{js}=G_j$, which shows that we need to have this special case included.
% Here, we introduce the equation $z_{js}=\mathbbm{1}\{y_{js}\geq G_j\}$ to include the border case, where $y_{js}=G_j$, then $z_{js}=1$.
% Analogously, 
% % we let $z_{js}=\mathbbm{1}\{y_{js}\geq 1\}, \forall s\in\mathcal{S}, j\in\mathcal{J}$.
% % , and let $G\triangleq\max_{j\in\mathcal{J}}G_j$.
% we can transform the indicator function in Eqn.~(\ref{eqn:chi_s}) to a set of following linear equations:
% \begin{align}
%     &y_{js}\geq G_j+G_j(z_{js}-1), \forall s\in\mathcal{S},\label{eqn:sum_y}\\
%   &\chi_s\geq z_{js}, \forall s\in\mathcal{S},j\in\mathcal{J}, \label{eqn:chi_s_2}\\
%     &\chi_s\geq x_{js}, \forall s\in\mathcal{S},j\in\mathcal{J},\label{eqn:chi_s_3}\\
%     &\chi_s, z_{js}\in\{0,1\}, \forall s\in\mathcal{S},j\in\mathcal{J} \label{eqn:zs}.
% \end{align}
% % \begin{align}
% %     \label{eqn:sum_y}&\sum_{j\in\mathcal{J}}y_{js}\geq 1+G(z_s-1), \forall s\in\mathcal{S},\\
% %     \label{eqn:chi_s_2}&\chi_s=z_s, \forall s\in\mathcal{S},\\
% %     &z_s\in\{0,1\}, \forall s\in\mathcal{S}, \label{eqn:zs}.
% % \end{align}

% Combine Eqns.~(\ref{eqn:sum_y})-(\ref{eqn:chi_s_3}), we can have that $\chi_s=1$ when $1\leq y_{js}\leq G_j, \forall s\in\mathcal{S}, \exists j\in\mathcal{J}$.
% However, it is not guaranteed from Eqns.~(\ref{eqn:y1})(\ref{eqn:y2}) that $l_{js}=1$ when $y_{js}=0$, and $u_{js}=1$ when $y_{js}\leq G_j-1$ since they are still valid with $l_{js}=0$ and $u_{js}=0$.
% % Also from Eqn.~(\ref{eqn:sum_y}), $z_s$ is not guaranteed to have value $1$ when $\sum_{j\in\mathcal{J}}y_{js}\geq 1$.
% Thus, we add a dummy term $-\frac{\mu}{J}\sum_{j\in\mathcal{J}}\sum_{s\in\mathcal{S}}x_{js}$ to the objective function, which will enforce the system to set $l_{js}$ and  $u_{js}$ to $1$ due to the minimization objective function.
% Also, $z_{js}$ can be either $0$ or $1$ when $y_{js}= G_j$.
% Similarly, we add another dummy term $-\frac{\mu}{J}\sum_{j\in\mathcal{J}}\sum_{s\in\mathcal{S}}z_{js}$ to force the system to set $z_{js}$ to $1$ when $y_{js}=G_j$ since it can reduce the objective value.

% \subsection{Problem Reformulation}
% After we handle with the non-amenable constraints


\section{An Offline Fractional Algorithm}\label{sec:frac}
\begin{figure}[t]
    \centering
    \includegraphics[width=0.45\textwidth]{Figures/fig_relaxation.eps}
    \caption{Example of too loose relaxation bound.}\label{fig:relaxation}
%        \vspace{-.1in}
\end{figure}

It is clearly that Problem~(\ref{Problem:primal}) is a Mixed integer linear program (MILP), which is NP-hard in general.
We first relax the integer constraints to continuous values to obtain the fractional solution, which serves as a lower bound to the discrete solution.
However, when we relax the binary variables to continuous values between 0 and 1, the system tend to assign same fractional value for all GPUs to make $x_{js}$ to 0, which also could make $\chi_s$ small, even they distribute across servers and may introduce resource contention.
In other words, Eqns.~(\ref{eqn:gamma})-(\ref{eqn:xjs}) are too loose to capture the inter-connect communication case, and thus lead to very small $k_j$ and $\chi_s$.
And as a result, the gap between the fractional solution and integer solution can be large.

Consider one scenario as indicated in Fig.~\ref{fig:relaxation} to show that the relaxed linear program solution can be a very loose bound.
In order to distinguish jobs' GPUs, we index them as  1 and 2.
%If only integer number of workers are allowed to be scheduled to each server, one placement scheme is shown in Fig.~\ref{fig:placement}(a), where both jobs use the external communication to perform the training.
Suppose the integer placement scheme is shown as in Fig.~\ref{fig:relaxation}(a), i.e., server 1 and 2 host one GPU from both jobs.
Then $x_{js}=1, j=1,2, s=1,2$, and  $k_1=k_2=2\alpha$.
However, if we relax the integer constraints and the fractional number of workers is allowed to be scheduled to each server, one placement scheme is shown in Fig.~\ref{fig:relaxation}(b).
We can see from the figure that each worker of the job is split into halves and is placed to server 1 and 2 (i.e., $z_{jgs}=0.5, j=1,2, g=1,2, s=1,2$).
According to Eqn.~(\ref{eqn:xjs}), $x_{js}=0, j=1,2, s=1,2$ and $k_1=k_2=0$, which is equivalent to the intra-connect communication case.
However, if we do not distinguish between GPUs of each job and merge two half GPUs of the same job in the same server into one complete GPU, the fractional placement scheme actually corresponds to the inter-connect communication case, and is equivalent to the integer placement scheme.
%In other words, $x_{11}$, $x_{12}$, $x_{23}$ and $x_{24}$ should not be $0$.
Therefore, the fractional solution is a very loose bound to its corresponding integer solution.



\subsection{Improvement of Relaxation Bound}
In order to strengthen the relaxation, we add the following constraints to Problem~(\ref{Problem:primal}):

\begin{align}
%    &\sum_{s'\in\mathcal{S}\setminus\{s\}}z_{jgs'}\geq 1-z_{jgs}, \quad\forall j\in\mathcal{J}, g\in\mathcal{G}_j,s \in\mathcal{S},\label{eqn:add1}\\
    &\sum_{g\in\mathcal{G}_j}z_{jgs}\geq G_j(1-x'_{js}),  \quad\forall j\in\mathcal{J}, s \in\mathcal{S},\label{eqn:add2}\\
%    &x_{js}\geq z_{jgs}\cdot x'_{js},  \quad\forall j\in\mathcal{J}, g\in\mathcal{G}_j,s \in\mathcal{S},\label{eqn:add3}\\
%    &x_{js}\geq (1-\frac{\sum_{g\in\mathcal{G}_j}z_{jgs}}{G_j})z_{jgs}, \quad\forall j\in\mathcal{J}, g\in\mathcal{G}_j,s \in\mathcal{S}\label{eqn:add2},\\
%    &x_{js}\geq (1-\sum_{s'\in\mathcal{S}\setminus\{s\}}z_{jgs'}) x'_{js}, \forall j\in\mathcal{J}, g\in\mathcal{G}_j,s \in\mathcal{S},\label{eqn:add4}\\
%    &\chi_s\geq \sum_{s'\in\mathcal{S}\setminus\{s\}}z_{jgs'}, \quad\forall j\in\mathcal{J}, g\in\mathcal{G}_j,s \in\mathcal{S},\label{eqn:add5}\\
    &\chi_s\geq 1-\sum_{s'\in\mathcal{S}\setminus\{s\}}z_{jgs'}, \quad\forall j\in\mathcal{J}, g\in\mathcal{G}_j,s \in\mathcal{S},\label{eqn:add5}\\
% &\chi_s\geq 1-\gamma_{js}, \quad\forall j\in\mathcal{J}, s \in\mathcal{S},\label{eqn:add5}\\
    &x_{js}\geq \chi_sx'_{js},\quad\forall j\in\mathcal{J}, s \in\mathcal{S},\label{eqn:add6}\\
%    &x_{js}\geq \chi_sx'_{js},\quad\forall j\in\mathcal{J}, s \in\mathcal{S},\label{eqn:add6}\\
    &x'_{js}\in\{0,1\}, \quad\forall j\in\mathcal{J}, s \in\mathcal{S}\label{eqn:add7}.
\end{align}
%where $H_j=\min\{N_s,G_j\}$.
%Recall that $\sum_{g\in\mathcal{G}_j}z_{jgs}\leq H_j$.
 From Constraint~(\ref{eqn:gpu2}), we know that $\sum_{s'\in\mathcal{S}\setminus\{s\}}z_{jgs'}=0$ implies  $z_{jgs}=1$ (i.e., server $s$ is selected to host job $j$'s GPU $g$), and $\sum_{s'\in\mathcal{S}\setminus\{s\}}z_{jgs'}=1$ implies  $z_{jgs}=0$ (i.e., server $s$ is not selected to host job $j$'s GPU $g$).
% ; otherwise $z_{jgs}=0$ (i.e., server $s$ is not chosen to schedule job $j$'s GPU $g$).
 From Constraint~(\ref{eqn:add2}), we know that if $\sum_{g\in\mathcal{G}_j}z_{jgs}=G_j$ (i.e., jobs using intra-connect communication), then $x'_{js}$ could be either 0 or 1.
  However, in order to minimize $x_{js}$ (Eqn.~(\ref{eqn:add6})) to minimize $k_j$,  $x'_{js}$ will be set to 0.
 If $1\leq \sum_{g\in\mathcal{G}_j}z_{jgs}\leq G_j-1$ (i.e., jobs using inter-connect communication), then $x'_{js}=1$.
 And if $\sum_{g\in\mathcal{G}_j}z_{jgs}=0$ (i.e., server $s$ is not chosen to host job $j$'s GPUs), then $x'_{js}=1$.
 
% First, we check the correctness of Constraint~(\ref{eqn:add3}).
% Note that $x_{js}$ is determined by the product of $z_{jgs}$ and $x'_{js}$, and based on the above discussion, we have: 1) $x_{js}\geq 0$ if server $s$ is not selected to schedule job $j$'s GPU $g$ ($z_{jgs}=0$) or intra-connect communication is used ($x'_{js}=0$); 2) $x_{js}\geq 1$ if server $s$ is chosen to schedule job $j$'s GPU $g$ ($z_{jgs}=1$) and inter-connect communication is used ($x'_{js}=1$), this shows its correctness.
% 
% Second, we check the correctness of Constraint~(\ref{eqn:add4}).
% Analogously, $x_{js}$ is determined by the produce of $1-\sum_{s'\in\mathcal{S}\setminus\{s\}}z_{jgs'}$ and $x'_{js}$.
% We have: 1) $x_{js}\geq 0$ if server $s$ is not selected to schedule job $j$'s GPU $g$ ($1-\sum_{s'\in\mathcal{S}\setminus\{s\}}z_{jgs'}=0$) or intra-connect communication is used ($x'_{js}=0$); 2) $x_{js}\geq 1$ if server $s$ is chosen to schedule job $j$'s GPU $g$ ($1-\sum_{s'\in\mathcal{S}\setminus\{s\}}z_{jgs'}=1$) and inter-connect communication is used ($x'_{js}=1$), thus shows its correctness.
 
First, we check the correctness of Constraint~(\ref{eqn:add5}).
%Recall that $\chi_s$ is the binary variable to indicate whether server $s$ is selected to schedule jobs or not.
If server $s$ is chosen, i.e., $\sum_{s'\in\mathcal{S}\setminus\{s\}}z_{jgs'}=0$, implying $\chi_s\geq 1$; otherwise, $\sum_{s'\in\mathcal{S}\setminus\{s\}}z_{jgs'}=1$, then $\chi_s\geq 0$, which is conformal to the definition of $\chi_s$.

Next, we check the correctness of Constraint~(\ref{eqn:add6}).
Note that $x_{js}$ is determined by the produce of $\chi_s$ and $x'_{js}$.
 We have: 1) $x_{js}\geq 0$ if server $s$ is not selected to schedule job $j$'s GPU $g$ ($\chi_s=0$) or intra-connect communication is used ($x'_{js}=0$); 2) $x_{js}\geq 1$ if server $s$ is chosen to schedule job $j$'s GPU $g$ ($\chi_s=1$) and inter-connect communication is used ($x'_{js}=1$), thus shows its correctness.
 
 
 After adding these constraints, we next show that they could strengthen the relaxation bound, basically, we need to show that the bound of $x_{js}$ and $\chi_s$ are larger compared to those in the original Problem~(\ref{Problem:primal}).
We observe that either $z_{jgs}$ or $1-\sum_{s'\in\mathcal{S}\setminus\{s\}}z_{jgs'}$ should be larger than 0.5 since we have $z_{jgs}+\sum_{s'\in\mathcal{S}\setminus\{s\}}z_{jgs'}=1$.
In other words, $\chi_s\geq 0.5$, which is tightened from 0.
Also, based on Eqn.~(\ref{eqn:add2}), when server $s$ is chosen to schedule GPU $g$ from job $j$ using inter-connect communication, then $x'_{js}\geq 1-\sum_{g\in\mathcal{G}_j}z_{jgs}/G_j$.
As a result, $x_{js}\geq 0.5\times (1-\sum_{g\in\mathcal{G}_j}z_{jgs}/G_j)$, which is tightened from 0.
%In addition, $\chi_s\geq 0.5$ according to Eqns.~(\ref{eqn:chi_s2})(\ref{eqn:add5}), thus it also gets larger compared to 0.
Therefore, the fractional solution bound is improved.

\subsection{Solving Bilinear Constraints}
 
% 
% \subsection{Strengthen Technique One}
%
%In order to strength the relaxation, we introduce the following bilinear constraint to Problem~(\ref{Problem:primal}):
%
%\begin{align*}
%    x_{js}\geq (1-z_{jgs})\chi_s, \quad\forall j\in\mathcal{J}, g\in\mathcal{G}_j,s\in\mathcal{S}.
%\end{align*}
%The rational behind is that for the selected servers, we add some virtual worker represented by 1, and as long as $z_{jgs}\neq 1, \forall g\in\mathcal{G}_j$ (i.e., not use internal communication), it will add the non-zero value to $x_{js}$, which can improve the relaxation bound. 
%We take Fig.~\ref{fig:placement}(b) as an example, the shaded workers are the added virtual workers to each selected server (server 1 and 2 in this example).
%Then $1-z_{jgs}=0, j=1,2, g=1,2, s=1,2$, and $\chi_s>0$ for the selected servers, thus we have $x_{js}>0,j=1,2,s=1,2$ instead of $x_{js}=0, j=1,2,s=1,2$.
%And as a result, the fractional solution bound is improved.
%In order to solve such bilinear constraint, we let $z'_{js}=z_{jgs}\chi_s$.
%Traditionally, in order to solve the bilinear constraint, the McCormick inequalities\cite{McCormick76:McCormick} will be leveraged to convert $z'_{js}$ into a set of following linear constraints:
%
%\begin{align}
%    &z'_{js}\geq z_{jgs}+\chi_s-1,\quad\forall j\in\mathcal{J}, g\in\mathcal{G}_j,s\in\mathcal{S},\label{eqn:bilinear1}\\
%    &z'_{js}\leq z_{jgs},\quad\forall j\in\mathcal{J}, g\in\mathcal{G}_j,s\in\mathcal{S},\\
%       &z'_{js}\leq \chi_s,\quad\forall j\in\mathcal{J}, g\in\mathcal{G}_j,s\in\mathcal{S},\\
%    &z'_{js}\geq 0,\quad\forall j\in\mathcal{J}, g\in\mathcal{G}_j,s\in\mathcal{S}\label{eqn:bilinear2}.
%%    &x_{js}\geq \chi_s-z'_{js},\quad\forall j\in\mathcal{J}, g\in\mathcal{G}_j,s\in\mathcal{S}.
%\end{align}
%The strongest possible relaxation of the non-convex domain of the bilinear constraint is its convex hull, and has been shown to be a polyhedron\cite{Rikun97:convex-envelope}.
% In general, the McCormick relaxation may strictly contain the convex hull, leading to weaker relaxation bounds.
% However, when the bounds on the variables are all between 0 and 1, then the McCormick relaxation is equivalent to the convex hull\cite{Ryoo01:boundsformultilinear}, thus the convex envelop for the bilinear constraint domain in our case is the convex hull.
% 
% Therefore, we can obtain the following linear program after we strength the relaxation:
% \begin{align}
% \text{Minimize } &c\sum_{j\in\mathcal{J}}F_je_jk_j+\mu\sum_{s\in\mathcal{S}}N_s\chi_s\label{Problem:relax}\\
%    \text{subject to }
%    &x_{js}\geq \chi_s-z'_{js},\\
%    &z_{jgs},x_{js},\chi_s\in[0,1], k_j\geq 0, \forall j\in\mathcal{J}, g\in\mathcal{G}_j, s\in\mathcal{S},\nonumber\\
%    &\text{Constraints}~(\ref{eqn:t_j})(\ref{eqn:k_j_reformulate})(\ref{eqn:cap2})-(\ref{eqn:xjs})(\ref{eqn:bilinear1})-(\ref{eqn:bilinear2})\nonumber.
% \end{align}
% 
% Note that as long as $z_{jgs}\neq 1, \forall g\in\mathcal{G}_j$ (corresponds to internal communication case), $x_{js}>0$, which implies that the added bilinear constraint makes the bound tighter.


%\begin{align*}
%    &z'_{js}\geq 2z_{jgs}-1,\quad\forall j\in\mathcal{J}, g\in\mathcal{G}_j,s\in\mathcal{S},\\
%    &z'_{js}\leq z_{jgs},\quad\forall j\in\mathcal{J}, g\in\mathcal{G}_j,s\in\mathcal{S},\\
%    &z'_{js}\geq 0,\quad\forall j\in\mathcal{J}, g\in\mathcal{G}_j,s\in\mathcal{S},\\
%    &x_{js}\geq 4z_{jgs}-4z'_{js},\quad\forall j\in\mathcal{J}, g\in\mathcal{G}_j,s\in\mathcal{S}.
%\end{align*}

%{\color{red} The bound is still loose since the fractional values of $x_{js}$ can be arbitrary small, which makes the performance ratio less interesting.
%This issue I think is caused by the indicator function, which has the weak continuous relaxation problem in essence.}
%Here, we consider bilinear functions of the form\cite{Luedtke12:multilinear}:
%
%\begin{align*}
%f(q)=\sum_{\{i,j\}\in E}q_iq_j,
%\end{align*}
%for $q_i,q_j\in[0,1]$, where $E$ is a subset of unordered pairs of distinct indices in $N=\{1,\hdots,n\}$.
%We let $u_{ij}\triangleq q_iq_j, \forall \{i,j\}\in E$.
%Traditionally, in order to solve such bilinear function $u_{ij}$, the McCormick inequalities\cite{McCormick76:McCormick} will be leveraged to bound each term $q_iq_j$:
%\begin{align*}
%&u_{ij}\geq q_i+q_j-1,\quad\forall \{i,j\}\in E,\\
%&u_{ij}\leq q_i, \quad\forall \{i,j\}\in E,\\
%&u_{ij}\leq q_j, \quad\forall \{i,j\}\in E,\\
%&u_{ij}\geq 0,\quad\forall \{i,j\}\in E.
%\end{align*}

%We point out here that the strongest possible relaxation of the non-convex domain of the bilinear constraint is its convex hull, and has been shown to be a polyhedron\cite{Rikun97:convex-envelope}.
%In general, the McCormick relaxation may strictly contain the convex hull, leading to weaker relaxation bounds.
%However, when the bounds on the variables are all between 0 and 1, then the McCormick relaxation is equivalent to the convex hull\cite{Ryoo01:boundsformultilinear}, thus the convex envelop for the bilinear constraint domain in our case is the convex hull.
%After adding extra Constraints~(\ref{eqn:add1})-(\ref{eqn:add6}), we can see that Problem~(\ref{Problem:primal}) is a non-convex optimization problem involving bilinear functions \cite{Luedtke12:multilinear}, which is defined as $f: [l,u]\rightarrow \mathbb{R}$, where
%\begin{align*}
%f(x)=\sum_{i\in\mathcal{I}}a_i\prod_{k\in\mathcal{K}_i}q_j,
%\end{align*}
%and $[l,u]=\{q\in\mathbb{R}^n|l\leq q\leq u\}$ as well as $|\mathcal{K}_i|\leq 2,\forall i\in\mathcal{I}$.
%
%The first challenge stems from the non-linear constraint~(\ref{eqn:add3}).
%We let $z'_{js}=z_{jgs}\cdot x'_{js}$, which is a bilinear function with single term (i.e., $|\mathcal{I}|=1$).
%%In order to solve such bilinear constraint, we let $z'_{js}=z_{jgs}\cdot x'_{js}$.
%Traditionally, in order to solve such bilinear function, the McCormick inequalities\cite{McCormick76:McCormick} will be leveraged to convert $z'_{js}$ into a set of following linear constraints:

After adding extra Constraints~(\ref{eqn:add2})-(\ref{eqn:add7}), we can see that Problem~(\ref{Problem:primal}) is a non-convex optimization problem involving bilinear functions that has the above form.
We let $z'_{js}=\chi_sx'_{js}$.
Traditionally, in order to solve such bilinear function $u_{ij}$, the McCormick inequalities\cite{McCormick76:McCormick} will be leveraged to bound $z'_{js}$.
%and let $\zeta_{js'}=z_{jgs'}x'_{js}$.
%We thus can obtain the following McCormick inequalities by specializing the above formulation:

%\begin{align}
%    &z'_{js}\geq z_{jgs}+x'_{js}-1,\quad\forall j\in\mathcal{J}, g\in\mathcal{G}_j,s\in\mathcal{S},\label{eqn:bilinear1}\\
%    &z'_{js}\leq z_{jgs},\quad\forall j\in\mathcal{J}, g\in\mathcal{G}_j,s\in\mathcal{S},\\
%       &z'_{js}\leq x'_{js},\quad\forall j\in\mathcal{J}, g\in\mathcal{G}_j,s\in\mathcal{S},\\
%    &z'_{js}\geq 0,\quad\forall j\in\mathcal{J}, g\in\mathcal{G}_j,s\in\mathcal{S}\label{eqn:bilinear2}.
%%    &x_{js}\geq \chi_s-z'_{js},\quad\forall j\in\mathcal{J}, g\in\mathcal{G}_j,s\in\mathcal{S}.
%\end{align}
%We next deal with constraint~(\ref{eqn:add4}), which involves the general bilinear function.
%We let $z''_{js}=\sum_{s'\in\mathcal{S}\setminus\{s\}}z_{jgs}x'_{js}$.
We thus can replace Eqn.~(\ref{eqn:add6}) with following McCormick inequalities:
\begin{align}
&x_{js}\geq z'_{js}, \quad \forall j\in\mathcal{J}, s\in\mathcal{S},\\
&z'_{js}\geq \chi_s+x'_{js}-1,\quad\forall j\in\mathcal{J}, s\in\mathcal{S},\label{eqn:bilinear1}\\
&z'_{js}\leq \chi_s,\quad\forall j\in\mathcal{J}, s\in\mathcal{S},\label{eqn:bilinear2}\\
&z'_{js}\leq x'_{js},\quad\forall j\in\mathcal{J}, s\in\mathcal{S},\label{eqn:bilinear3}\\
&z'_{js}\geq 0,\quad\forall j\in\mathcal{J}, s\in\mathcal{S}\label{eqn:bilinear4}.
\end{align}

%{\em 2) } Similarly, we replace Egn.~(\ref{eqn:add4}) with following equations:
%\begin{align}
%&x_{js}\geq x'_{js}-\sum_{s'\in\mathcal{S}\setminus\{s\}}\zeta_{js'}, \quad \forall j\in\mathcal{J}, s\in\mathcal{S},\\
%&\zeta_{js'}\geq z_{jgs'}+x'_{js}\!-\!1,\forall j\!\in\!\mathcal{J}, g\!\in\!\mathcal{G}_j,s\!\in\!\mathcal{S},s'\!\in\!\mathcal{S}\!\setminus\!\{s\},\label{eqn:bilinear3}\\
%&\zeta_{js'}\leq z_{jgs'},\quad\forall j\in\mathcal{J}, g\in\mathcal{G}_j,s'\in\mathcal{S}\setminus\{s\},\\
%&\zeta_{js'}\leq x'_{js},\quad\forall j\in\mathcal{J},s\in\mathcal{S}, s'\in\mathcal{S}\setminus\{s\},\\
%&\zeta_{js'}\geq 0,\quad\forall j\in\mathcal{J},s'\in\mathcal{S}\setminus\{s\}\label{eqn:bilinear4}.
%\end{align}

Several important remarks are in order:

{\em 1): } If server $s$ is not selected ($x'_{js}=1$ and $\chi_s=0$), then $z'_{js}\geq \chi_s+x'_{js}-1=0$, implying $x_{js}\geq z'_{js}=0$, thus $x_{js}=0$.

{\em 2): } If server $s$ is selected and intra-connect communication is performed ($x'_{js}=0$ and $\chi_s=1$), then $z'_{js}\geq \chi_s+x'_{js}-1= 0$, implying $x_{js}\geq z'_{js}=0$, thus $x_{js}=0$.

{\em 3): } If server $s$ is selected and inter-connect communication is performed ($x'_{js}>0$ and $\chi_s>0$), then $z'_{js}\geq \chi_s+x'_{js}-1\geq 0.5+1-\sum_{g\in\mathcal{G}_j}z_{jgs}/G_j-1\geq 0.5-\sum_{g\in\mathcal{G}_j}z_{jgs}/G_j$, implying $x_{js}\leq 0.5$.
% implying $x_{js}\geq z'_{js}$, which implies $x_{js}\leq 0.5$. {\color{red}The convex hull operation actually worsen the bound of $x_{js}$.}
It shows that the McCormick relaxation technique actually worsen the bound of $x_{js}$, but $\chi_s$ is not influenced.


We point out here that the strongest possible relaxation of the non-convex domain of the bilinear constraint is its convex hull, and has been shown to be a polyhedron\cite{Rikun97:convex-envelope}.
In general, the McCormick relaxation may strictly contain the convex hull, leading to weaker relaxation bounds.
However, when the bounds on the variables are all between 0 and 1, then the McCormick relaxation is equivalent to the convex hull\cite{Ryoo01:boundsformultilinear}, thus the convex envelop for the bilinear constraint domain in our case is the convex hull.

After the McCormick transformation and continuous relaxation, Problem~(\ref{Problem:primal}) becomes a linear program, which can be solved efficiently by LP solvers (e.g., Gurobi) to obtain the fractional solution.
 

 \section{Dependent Rounding Scheme}\label{sec:rounding}
 
The fractional solution returned by solving Problem~(\ref{Problem:primal}) is for the relaxed program.
The number of GPUs of each job should take non-negative integer values in each server.
% It is highly challenging to round Problem~(\ref{problem:pt}) due to its complicated packing and cover constraints as well as equality constraint~(\ref{ctr:gpu}) involved, making it impossible to round to integers efficiently.
% Therefore, we relax the equality constraint~(\ref{ctr:gpu}), i.e., $\sum_{s\in\mathcal{S}}y_s^j[t]\leq G^j$, to do the rounding.
% However, we will show later that the summation of rounded integers is at least $G^j-1$.
% In other words, from the cloud provider's perspective, the efficient training achieved at the cost of at most one extra GPU needs to be added to the submitted job.
We need to round the fractional solution $z_{jgs}$, $\forall j\in\mathcal{J},g\in\mathcal{G}_j, s\in\mathcal{S}$ into integer solution while not to violate Constraints~(\ref{eqn:gpu2})(\ref{eqn:cap2}).
In addition, we need to take the $\chi_s$ and $k_j$ into consideration to minimize the gap between the fractional solution and the integer solution after rounding to offer a better performance ratio.
Note that the variables are dependent on each other due to those coupling constraints.
The traditional independent rounding scheme where each variable is rounded up or down independently may well lead to constraint violation.
Hence we design a novel dependent rounding scheme by exploring the inherent dependence among variables.
 
 \begin{figure}[t]
    \centering
    \includegraphics[width=0.48\textwidth]{Figures/fig_round.eps}
    \caption{Example on fraction merge before rounding.}\label{fig:round}
%        \vspace{-.1in}
\end{figure}
 
 
 Recall that after the continuous relaxation, the system tends to break down each GPU into similar fractional values in order to minimize $x_{js}$ based on Eqn.~(\ref{eqn:xjs}).
 In other words, each GPU of the job may distribute its partial values over multiple servers, and the server may contain its each GPU's partial value. 
 As an example illustrated in Fig.~\ref{fig:round}(a), where job 1 requires three GPUs and job 2 requires two GPUs.
 In order to distinguish GPUs, we index them as $1, 2,\hdots, n$.
 Before we rounding the fractional solution, we first merge these partial values of the same job to maintain the capacity constraint of each server.
 As we can see from Fig.~\ref{fig:round}(b), after we perform the value fusion, in each server, at most one partial value for each job will occur.
 

 We let $\hat{y}_{js}\triangleq\lfloor\sum_{g\in\mathcal{G}_j}z_{jgs}\rfloor, \forall j\in\mathcal{J}, s\in\mathcal{S}$.
 Let $\hat{z}_{js}\triangleq \sum_{g\in\mathcal{G}_j}z_{jgs}-\hat{y}_{js}, \forall j\in\mathcal{J}, s\in\mathcal{S}$ , i.e., the remaining fractional value after the merge operation of job $j$ in server $s$.
 Let $\hat{N}_s\triangleq \max\{1,N_s-\sum_{j\in\mathcal{J}}\hat{y}_{js}\}, \forall s\in\mathcal{S}$, i.e., the remaining capacity of server $s$ (if the remaining capacity is less than 1, then round it up to 1).
 Let $L_j=\sum_{s\in\mathcal{S}}\hat{z}_{js}$ be the number of tasks (GPUs) associated with job $j$, then the total number of tasks to be scheduled is $L=\sum_{j\in\mathcal{J}}L_j$.
 We use $\mathcal{L}=\{\mathcal{L}_1,\hdots,\mathcal{L}_J\}$ to denote the ordered set of tasks to be rounded, where $\mathcal{L}_j$ is the set of tasks related to job $j$.
% We reduce the problem to Generalized Assignment Problem (GAP), where the number of jobs is $L=\sum_{j\in\mathcal{J}}\sum_{s\in\mathcal{S}}\hat{z}_{js}$.
We reduce the problem to Generalized Assignment Problem (GAP), where the number of tasks to be scheduled is $L$ and the number of machines is $S$.
% and use $\mathcal{H}, H$ to denote the set and number of machines to be scheduled, respectively i.e., servers that has fractional placement.
% We use $N_h$ to denote the remaining capacity of machine $h$, i.e., $N_h=N_s, \forall s\in\mathcal{H}$.
 We use $C_{ls}$ to denote the cost of assigning task $l$ to server $s$,  and we let $C_{ls}=G_j-\hat{y}_{js}$.
 The rational behind is in order to minimize $k_j$, intra-connect communication should be preferred, i.e., servers that already host most GPUs should have preference to schedule the rest fractional GPUs.
 We also use binary variable $\zeta_{ls}$ to indicate whether task $l$ is placed to server $s$ ($\zeta_{ls}=1$) or not ($\zeta_{ls}=0$).
 Then, the GAP problem we consider is as follows:
 \begin{align}
\underset{\zeta}{\textbf{GAP: }\text{Minimize  }}&\sum_{s\in\mathcal{S}}\sum_{l\in\mathcal{L}}C_{ls}\zeta_{ls}\leq \beta\nonumber\\
 \text{subject to }&\sum_{s\in\mathcal{S}}\zeta_{ls}=1, \quad \forall l\in\mathcal{L},\label{eqn:assignment}\\
 &\sum_{l\in\mathcal{L}}\zeta_{ls}\leq \hat{N}_s, \quad \forall s\in\mathcal{S},\label{eqn:capacity}\\
 &\zeta_{ls}\geq 0, \quad \forall l\in\mathcal{L}, s\in\mathcal{S}\nonumber.
%&\zeta_{ls}=0, \quad \text{if } 1> \hat{N}_s, \forall l\in\mathcal{L}, s\in\mathcal{S}\nonumber.
 \end{align}
 We next leverage ST rounding\cite{Shmoys93:GAP} to obtain the integral solution from the fractional solution.
 We first construct a weighted bipartite graph $G=\langle \mathcal{L}, \mathcal{S}, E\rangle$ based on $\zeta_{ls}$ as follows:
 
 {\em Step 1: } One side of the bipartite graph consists of task nodes: $\mathcal{L}=\{u_l | l=1,\hdots,L\}$, and the other side of the contains server nodes: $\mathcal{S}=\{v_{s\gamma} | s=1,\hdots, S, \gamma=1,\hdots,\Gamma_s\}$, where $\Gamma_s=\lceil \sum_{l\in\mathcal{L}}\zeta_{ls}\rceil$.
 Basically, we assign $\Gamma_s$ task nodes to server $s$.
 
 {\em Step 2: } For each server $s$, we can view server nodes $v_{s\gamma}$ as unit capacity bins, and view $\zeta_{ls}, \forall l\in\mathcal{L}$ as pieces of tasks scheduled to these bins.
 We keep placing pieces into bin node $v_{s1}$ one by one until placing piece $l$ exceed the unit capacity, then partial of $l$ will be placed to $v_{s1}$ to reach its capacity, and the remaining fraction will be placed to next bin $v_{s2}$.
 The process is continued until all pieces are scheduled to bins.
 
 {\em Step 3: } We add edge $(u_l,v_{s\gamma})$ to $E$ if a fraction of task $l$ is placed to bin $v_{s\gamma}$.
 We use $y'(u_l,v_{s\gamma})$ to denote the fraction of task $l$ places to bin $v_{s\gamma}$, and set the cost of this edge to $C_{ls}$.
 
 Note that the vector $y'$ is a fractional matching in bipartite graph $G$ that exactly matches all task nodes.
 There exists an integral matching with objective value at most $\beta$ according to matching theory\cite{Lovasz09:matchingtheory}, which also exactly matches all task nodes.
 We summarize the rounding procedure in Algorithm~\ref{alg:round}:
 \begin{algorithm}
\SetAlgoLined
\nonl\textbf{Input:} $\zeta_{ls},\forall l,s$\;
\nonl\textbf{Initialization:} $\bar{\zeta}_{ls}=0,\forall l,s$\;
Build a bipartite graph $G=\langle \mathcal{L}, \mathcal{S}, E\rangle$ based on $\zeta_{ls}$ as illustrated above\;
Find an integer matching that exactly matches all job nodes in $G$ with the minimum GAP objective value\;
If task $l$ is mapped to server $s$, then update $\bar{\zeta}_{ls}=1$\;
\Return $\bar{\zeta}_{ls},\forall l,s$\;
\caption{Rounding Algorithm.}
 \label{alg:round}
\end{algorithm} 

After the rounding, we update the integral solution $y_{js}=\hat{y}_{js}+\sum_{l\in\mathcal{L}_j}\bar{\zeta}_{ls},\forall j,s$.
Then we can obtain the integral $k_j, \forall j$ and $\chi_s,\forall s$ based on $y_{js},\forall j,s$.

 
 Next, we provide the theoretical analysis with respect to our algorithms.
 
 {\em 1) Feasibility Discussion:}
 
 \begin{thm}\label{thm:feasibility}
 The integral solution returned by Algorithm~\ref{alg:round} guarantees Constraint~(\ref{eqn:assignment}) to be satisfied, and the violation of the capacity constraint~(\ref{eqn:capacity}) is at most twice of $\hat{N}_s$, i.e., $\sum_{l\in\mathcal{L}}\bar{\zeta}_{ls}\leq 2\hat{N}_s, \forall s\in\mathcal{S}$.
 \end{thm}
 \begin{proof}
 Recall that Algorithm~\ref{alg:round} generates an integral matching that exactly matches all task nodes, thus Constraint~(\ref{eqn:assignment}) is satisfied.
 In order to show the violation of capacity constraint~(\ref{eqn:capacity}) is at most twice of $\hat{N}_s$.
 Note that the total GPU resource consumption of tasks scheduled to server $s$ by any integral matching in $G$ is no greater than $\sum_{\gamma=1}^{\Gamma_s}1$.
% We consider the following two cases:
% 
% {\em i): } $\hat{N}_s<1$, then $\Gamma_s=\lceil \sum_{l\in\mathcal{L}}\zeta_{ls} \rceil=1$.
% 
% Clearly, $\sum_{\gamma=1}^{\Gamma_s}1\leq 1$.
% 
% {\em ii): } 
And it is clear that $1\leq \hat{N}_s$, then we have:
 \begin{align*}
 \sum_{\gamma=2}^{\Gamma_s}1&=\sum_{\gamma=1}^{\Gamma_s-1}1= \sum_{\gamma=1}^{\Gamma_s-1}\sum_{l:(u_l,v_{s\gamma})\in E}y'(u_l,v_{s\gamma})\\
 &\leq \sum_{\gamma=1}^{\Gamma_s}\sum_{l:(u_l,v_{s\gamma})\in E}y'(u_l,v_{s\gamma})=\sum_{l\in\mathcal{L}}\zeta_{lh}\leq \hat{N}_s.
 \end{align*}
 Hence we have $\sum_{\gamma=1}^{\Gamma_s}1=1+\sum_{\gamma=2}^{\Gamma_s}1\leq 2\hat{N}_s$, and the proof is complete.
 \end{proof}

 
 {\em 2) Time Complexity:}
 
 \begin{thm}\label{thm:time}
 The time complexity of our algorithm is $O(S^3+SJ^2\log J)$, which is polynomial.
 \end{thm}
 \begin{proof}
 Our algorithm consists of three main steps: i) Solving the LP relaxation of Problem~(\ref{Problem:primal}) can be approximately bounded by $O(S^3)$ if we use a polynomial time LP solver (e.g., Vaidya's algorithm\cite{Vaidya87:LP}); 
% ii) Constructing GAP problem based on the returned fractional solution takes $O(\sum_{j\in\mathcal{J}}G_j)=O(J)$; 
 ii) The ST rounding in Algorithm~\ref{alg:round} takes $O(SJ^2\log J)$\cite{Shmoys93:GAP};
 iii) Update the integral solution $y_{js}$ and obtain the integral $k_j$ and $\chi_s$ takes $O(SJ)$.
 Therefore, the time complexity of our algorithm is $O(S^3+SJ^2\log J)$, which is polynomial.
 \end{proof}
 
 
 \begin{lem}
\label{lem:relation} Let  $A(\mathbf{x})\!=\!\frac{\sum_{k=1}^nf(k,\mathbf{x})}{\sum_{k=1}^ng(k,\mathbf{x})}$, and $B(\mathbf{x})\!=\!\sum_{k=1}^n\frac{f(k,\mathbf{x})}{g(k,\mathbf{x})}$.
If both $f(\cdot)$ and $g(\cdot)$ are non-negativity, then we have $A(\mathbf{x})\leq B(\mathbf{x})$.
\end{lem}

\begin{proof}
$\frac{f(k,\mathbf{x})}{\sum_{k=1}^ng(k,\mathbf{x})}\leq\frac{f(k,\mathbf{x})}{g(k,\mathbf{x})}$, since $g(k,\mathbf{x})\leq\sum_{k=1}^ng(k,\mathbf{x})$.
Thus $A(\mathbf{x})=\frac{\sum_{k=1}^nf(k,\mathbf{x})}{\sum_{k=1}^ng(k,\mathbf{x})}=\sum_{k=1}^n\frac{f(k,\mathbf{x})}{\sum_{k=1}^ng(k,\mathbf{x})}\leq\sum_{k=1}^n\frac{f(k,\mathbf{x})}{g(k,\mathbf{x})}=B(\mathbf{x})$.
\end{proof}
 
 
 {\em 3) Approximation Ratio:}  The approximation is the worst-case ratio between the objective value achieved by our algorithm and the objective ratio achieved by some off-line optimal algorithm.
 
 
 \begin{thm}\label{thm:ratio}
Our algorithm is $N^{\max}/N^{\min}+2$-approximation, where $ N^{\max}=\max_{j,s}\{N_s,G_j\}$ and $N^{\min}=\min_j\{1-\sum_gz_{jgs}/G_j)\}$.
 \end{thm}
 
 \begin{proof}
 We let $\bar{k}_j, \bar{\chi}_s$ and $\bar{k}_j^*, \bar{\chi}_s^*$ be the integral solution returned by our solution and the optimal integral solution obtained by some offline algorithm.
 Let $\hat{k}_j, \hat{\chi}_s$ be the fractional solution by solving Problem~(\ref{Problem:primal}) after continuous relaxation without McCormick inequality operation.
 Note that $\bar{k}_j\leq\alpha N^{\max}$, where $ N^{\max}=\max_{j,s}\{N_s,G_j\}$ since the largest number of concurrent running jobs is bounded by both the server's capacity and the number of GPUs required, and $\bar{\chi}_s\leq 1$.
 Note that if $\hat{k}_j=0$, then we have $\bar{k}_j=0$, thus we consider the inter-connect communication jobs, i.e., $\hat{k}_j>0$. 
And we have $\hat{k}_j\geq \alpha \sum_{j'}x_{j's}\geq \alpha\sum_{j'}(1-\sum_gz_{jgs}/G_j)=\alpha N^{\min}$, where $N^{\min}\!=\!\min_j\{1-\sum_gz_{jgs}/G_j\}$, and $\hat{\chi}_s\geq 1/2$.
 With Lemma~\ref{lem:relation}, the approximation ratio can be computed as:
 \begin{align*}
 &\frac{c\sum_{j\in\mathcal{J}}F_je_j\bar{k}_j+\mu\sum_{s\in\mathcal{S}}N_s\bar{\chi}_s}{c\sum_{j\in\mathcal{J}}F_je_j\bar{k}_j^*+\mu\sum_{s\in\mathcal{S}}N_s\bar{\chi}_s^*}\\
 &\leq \frac{c\sum_{j\in\mathcal{J}}F_je_j\bar{k}_j}{c\sum_{j\in\mathcal{J}}F_je_j\bar{k}_j^*}+\frac{\mu\sum_{s\in\mathcal{S}}N_s\bar{\chi}_s}{\mu\sum_{s\in\mathcal{S}}N_s\bar{\chi}_s^*}\\
 &\leq \frac{c\sum_{j\in\mathcal{J}}F_je_j\bar{k}_j}{c\sum_{j\in\mathcal{J}}F_je_j\hat{k}_j}+\frac{\mu\sum_{s\in\mathcal{S}}N_s\bar{\chi}_s}{\mu\sum_{s\in\mathcal{S}}N_s\hat{\chi}_s}\\
 &\leq \frac{N^{\max}}{N^{\min}}+2.
 \end{align*}
 \end{proof}
 
 
 
 










==> MobiHoc'22_Communication_Contention_Tech_Report/Sec6_Numerical/Sec6_Numerical.tex <==
% !TEX root = ../Communication_Contention_MobiHoc22.tex


\begin{figure*}[t!]
   % \hspace{0.005\linewidth}
       \begin{minipage}[t]{0.24\linewidth}
        \centering
        \includegraphics[width=1.05\textwidth]{Figures/baseline.eps}
        %\captionsetup{width=0.75\textwidth}       
        \caption{Makespan comparison under different policies.}\label{fig:baseline} 
        % with unit resource (cpu:3400,gpu:600,memory:1400GB,storage:1200GB)
    \end{minipage}%
    \hspace{0.006\linewidth}
    \begin{minipage}[t]{0.24\linewidth}
        \centering
        \includegraphics[width=1.04\textwidth]{Figures/kappa.eps}      
        \caption{Impact of value of $\kappa$ on makespan.} \label{fig:kappa}
    \end{minipage}%  
      \hspace{0.01\textwidth}
         \begin{minipage}[t]{0.24\linewidth}
        \centering
        \includegraphics[width=1.04\textwidth]{Figures/servers.eps}
        \caption{Makespan as the number of servers increases.} \label{fig:contention}
    \end{minipage}%
           \hspace{0.007\textwidth}
    \begin{minipage}[t]{0.24\linewidth}
        \centering
        \includegraphics[width=1.01\textwidth]{Figures/lambda.eps}
        \caption{Impact of the value of $\lambda$ on makespan.}\label{fig:lambda}
    \end{minipage}%
\vspace{-.1in}
\end{figure*}


\section{Numerical Results}
\label{sec:numerical}

In this section, we conduct simulation studies to evaluate the performance of our proposed SJF-BCO algorithm.

%\subsection{Simulation Setup}
\smallskip
\textbf{1) Experiment Settings:} 
Similar to the setting in~\cite{Wang20:contention}, the workload is generated  based on the Microsoft job trace~\cite{Jeon19:microsofttrace}.
%We generate 160 DDL jobs from~\cite{Jeon19:microsofttrace} following the job-type distribution, where there are 80 single-GPU jobs, 14 2-GPU jobs, 26 4-GPU jobs, 30 8-GPU jobs, 8 16-GPU jobs, and 2 32-GPU jobs.
We generate 160 DDL jobs by scaling down the original job trace~\cite{Jeon19:microsofttrace} following the job-type distribution, where there are 80 single-GPU jobs, 14 2-GPU jobs, 26 4-GPU jobs, 30 8-GPU jobs, 8 16-GPU jobs, and 2 32-GPU jobs.
We set $F_j\in[1000,6000]$.
The extra time cost brought by communication contention and overhead is within 15\% of the total actual execution time.
We let $\xi_1 = \xi_2$ (cf. Sec.~\ref{subsec:sys_model}) to make communication contention and overhead cost comparable.
We set $\tau_j[t]\in[0.01, 0.05]$~\cite{Yu21:PD-ORS}, and $\lambda_j = 1, \forall j$.
We set the estimated execution time $\hat{\rho}(\y^k)\in[50, 300]$ (evaluated from the product of $\tau_j[t]$ and $F_j$).
The GPU cluster has 20 servers.
The number of GPUs on each server is chosen from $\{4, 8, 16, 32\}$ uniformly at random.

\smallskip
\textbf{2) Baselines for Comparison:} We compare our algorithm with three representative job scheduling algorithms: First-Fit (FF)~\cite{Stavrinides11:FF-LS}, List-Scheduling (LS)~\cite{Stavrinides11:FF-LS}, and Random (RAND)~\cite{Wang20:contention}.
%1) RAND: randomly schedule jobs to servers if the servers' capacity is not violated;
Here, we define $\theta_u^{f}$ as the maximum execution time limit returned by the scheduling policy $f$. %, which could be found using bisection search.
Given a job $j$,
FF picks the first $G_j$ available GPUs such that their accumulative execution time does not exceed the limit $\theta_u^{FF}$, from server to server.
This policy tends to pack different jobs into the fewest number of servers to avoid fragmentation introduced by small jobs, which can save space for large jobs to be scheduled next.
LS selects top-$G_j$ GPUs with least execution time first, so that the accumulative execution time does not exceed the limit $\theta_u^{LS}$.
Note that this policy may introduce high communication overhead since it may choose GPUs from a large number of servers.
Further, LS tries to balance the execution time between GPUs by always selecting the one with the least execution time.
RAND randomly chooses servers and GPUs to schedule jobs.
In this policy, we allocate GPUs to a job as long as it does not exceed $T$, i.e., we set $\theta_u^{RAND} = T$, to avoid the long running time in order to find a feasible schedule.

\smallskip
\textbf{3) Experiment Results:}
First, we compare the makespan performance achieved by our SJF-BCO algorithm with those of the baseline  policies.
We set $T=1200$.
As shown in Fig.~\ref{fig:baseline}, SJF-BCO outperforms other scheduling policies both in terms of makespan and average job completion times, implying that SJF-BCO is also superior in terms of total job completion time.
Note that SJF-BCO tends to open new server(s) for large jobs to avoid the large communication overhead and use shared servers for small jobs to avoid the fragmentation, thus achieving better average completion time and makespan than FF and RAND.
%Surprisingly, RAND has better average completion time than FF.
%The possible reason is that FF suffers from execution time imbalance, i.e., certain worker's accumulative execution time may be large. % yielding worse overall job completion time.
%Further, since FF always co-locate different jobs to the same server, its performance may also be compromised due to the extensive communication contention.
%%The possible reason is that FF has a high possibility that different jobs will use the same server, leading to higher communication contention.
%%Also, FF will have potential serious execution time imbalance issue.
%However, as the number of servers increases, the probability of selecting large number of servers in RAND becomes higher, i.e., communication overhead may become dominant, then FF could have better average performance.
Note that SJF-BCO has more prominent advantages over these baselines when the cluster has limited GPU resources.
%since SJF-BCO will strive for a balance between communication contention and overhead.
%Theoretically, SJF-BCO tries to strive for a balance between communication contention and overhead, it will have more superior performance when the cluster has limited GPU resources .

Then, we examine the impact of $\kappa$ on the makespan in our proposed SJF-BCO algorithm.
We set $T=1200$, and select $\kappa$ from 1 to 32.
As indicated in Fig.~\ref{fig:kappa}, as the value of $\kappa$ increases, the makespan first drops and then increases and then drops again.
Recall that in Algorithm~\ref{alg:place}, FA-FFP is used when the number of requested GPUs $G_j\leq\kappa$; otherwise LBSGF is used.
Note that before Turning point 1 in Fig.~\ref{fig:kappa}, as $\kappa$ increases, the makespan drops since more small jobs are packed into the fewest number of shared servers, resulting in decrement of communication contention and overhead introduced by larger jobs to be scheduled later.
% the decrement of communication contention is more significant compared to the increase of the communication overhead since more jobs use FA-FFP to schedule.
However, as $\kappa$ continues to grow, communication contention becomes more noticeable since more large jobs are scheduled to the shared servers, leading to the increase of makespan.
Finally, as $\kappa$ becomes sufficiently large, then the majority or even all jobs use shared servers to schedule their workers, which can slightly decrease the communication overhead due to the smaller resultant ring-span (see Turning point 2 in Fig.~\ref{fig:kappa}).


%Thus, $\kappa$ serves as a control parameter to balance between contention and overhead.
%In other words, as the ratio increases, more jobs will be scheduled based on LS policy, i.e., workload is more likely to be evenly distributed across servers, leading to less contention and better performance.

Next, we investigate the influence of communication contention by reducing the number of servers.
We set $T=1500$.
Intuitively, the larger number of servers, the less communication contention.
As we can see from Fig.~\ref{fig:contention}, as we increase the number of servers from 10 to 20, the makespan of FF, LS and SJF-BCO decrease due to the degradation of contention level.
Note that, if enough resources are available in the cluster, then each job will have a separate set of servers using SJF-BCO, i.e.,  its performance will become better as number of GPUs increases.
In this case, no communication contention will be introduced using SJF-BCO.
%, {\color{red}implying it is one of the optimal scheduling policies}.
The intuition that FF has the largest makespan reduction is that the average idle time for workers drops dramatically since a smaller execution time limit could be set as the number of servers increases.

Lastly, we inspect the influence of $\lambda$ on the makespan for SJF-BCO with $\lambda \in\{1, 2, 4, 8\}$ and $\kappa=1$.
As we can see from Fig.~\ref{fig:lambda}, the makespan monotonically decreases as the $\lambda$ increases.
Recall that a larger $\lambda$-value implies a larger number of servers could be selected.
Then, the job has a higher chance to open new servers to schedule its workers, resulting in less communication contention and a smaller communication overhead.
Interestingly, $\lambda$ plays a similar role as $\kappa$, with the aim to balance communication overhead and contention.
Specifically, $\kappa$ affects the overall balance between all jobs since it determines the portion of jobs to use either FA-FFP or LBSGF, while $\lambda$ focuses more on the balance between communication contention and overhead for a specific job that uses LBSGF to schedule.




















==> MobiHoc'22_Communication_Contention_Tech_Report/Sec7_Conclusion/Sec7_Conclusion.tex <==
% !TEX root = ../Communication_Contention_MobiHoc22.tex

\section{Conclusion}
\label{sec:conclusion}

In this paper, we studied resource scheduling for DDL jobs in a multi-tenant GPU cluster, where we considered the communication contention and overhead determined by the distribution of workers.
We showed that this problem can be formulated as a highly non-trivial non-linear integer program with nonconvex and mixed packing-covering constraints.
We then converted the problem into a tractable integer linear program, which enables the design of approximation algorithms.
Specifically, we developed a new analytical model that jointly considers the placements and starting times of the workers of each DDL job.
Through careful reformulation, we then transformed the problem into an integer linear program with a more tractable structure, and proposed an approximation algorithm with an approximation ratio performance guarantee.
We provided rigorous theoretical analysis and conducted experiments to demonstrate the efficacy of our algorithms.
Collectively, our results contribute to a fundamental understanding on resource scheduling for DDL jobs in multi-tenant GPU clusters.


\section{Acknowledgements} \label{sec:ack}
J. Liu’s work has been supported in part by NSF grants CAREER CNS-2110259, CNS-2112471, CNS-2102233, CCF-2110252, and a Cisco Systems Research Grant GR127298.
B. Ji’s work has been supported in part by NSF CNS-2112694.
H. Rajan's work has been supported in part by NSF 21-20448 and NSF 19-34884.

==> MobiHoc'22_Communication_Contention_Tech_Report/Supporting_Preambles/jackmac.tex <==
%>From snoeyink%cs.ubc.ca@cs.Technion.AC.IL Wed Nov  3 08:18:27 1993
%Received: from csmail.cs.technion.ac.il by math.tau.ac.il (5.67/math.tau-930921)
	%id AA17625; Wed, 3 Nov 93 08:18:23 +0200
%Received: from csc (csc.cs.technion.ac.il) by csmail.cs.Technion.AC.IL (4.1/3.14)
	%id AA14244; Wed, 3 Nov 93 01:19:10 IST
%Received: from csa by csc (4.1/3.14)
	%id AA24688; Wed, 3 Nov 93 01:19:48 IST
%Received: from grolsch.cs.ubc.ca by csa (4.1/3.14)
	%id AA20525; Wed, 3 Nov 93 01:11:28 IST
%Return-Path: <snoeyink@cs.ubc.ca>
%Received: from cascade.cs.ubc.ca by grolsch.cs.ubc.ca with SMTP id AA13516
  %(5.65c/IDA-1.3.5 for alon@cs.Technion.AC.IL); Tue, 2 Nov 1993 13:56:34 -0800
%Date: Tue, 2 Nov 1993 13:56:34 -0800
%From: Jack Snoeyink <snoeyink%cs.ubc.ca@cs.Technion.AC.IL>
%Message-Id: <199311022156.AA13516@grolsch.cs.ubc.ca>
%Received: by cascade.cs.ubc.ca (4.1/SMI-4.1)
	%id AA21873; Tue, 2 Nov 93 13:56:33 PST
%To: alon@cs.Technion.AC.IL
%In-Reply-To: Alon Efrat's message of Sun, 31 Oct 93 23:38:48 IST <9310312138.AA19880@csc>
%Subject: LaTex Macros
%Status: RO
%Content-Length: 19065
%X-Lines: 638
%
%
%I'm in oberwolfach w/ micha, so I';ll just send you this and answer
%your questions on it when I get back to vancouver next week...
%
    %o                                    Jack
  %_/\_.
%(')>-(`)                          snoeyink@cs.ubc.ca
%----figbox.tex----

% 12 Oct 90 LaTeX figure boxing macros  by Jack Snoeyink
%					w/ ideas from John Hershberger
%					and code from Tom Rokicki
%%%%%%%%%%%%%%%%%
% 
% This file contains two classes of macros for dealing with figures in
% Latex documents:  
%  \figbox (and its relatives) take a box containing a figure or table
%    or whatever, caption it, and either place it on the page and wrap the
%    text around it or let it float (as usual).
%  \boxeps and \boxps take encasulated or plain postscript from a file
%    and put it in a box for use by \figbox
%
%%%%%%%%%%%%%%%%
%
% The most important macro for dealing with boxes is:
%
% \figbox: caption a box as a figure or table and place it in the margin
% 	(a marginal box) or float it (a floating box).
% 	Wide marginal boxes are promoted to one column floats; wide one
% 	column floats are promoted to two column floats.
%
% Usage: \figbox [*htblr] {box} {style} {label} {caption}
%
% The optional argument default is [htb].  Other choices
%   * two column (must come first),
%   h here, t top, b bottom (as in latex),
%   l left, r right (marginal boxes that do not float)
%
% NB: Left and right marginal boxes will not overlap in height.
%
% Two column figures default to htb unless some other 
%   	options follow the *.
%   They can also be specified by style {figure*} or {table*}.
%
% box is a box containing a figure or table.
% style is the caption style {figure}, {figure*}, {table}, or {table*}.  
% label is the label assigned.
%	if empty, the figure will not be labeled.
% caption is of the form {}, {Caption} or {[short caption] Long caption},
%       where the short caption goes into the list of figures/tables.
%	if empty, the figure will not be captioned or labeled.
% 
% The lower level macro \captionbox, described much later, can be used
% to combine two or more captioned figures into a single marginal or
% floating box.
%
%%%%%%%%%%%%%%%%
%
% options defined by macros are: \captionstyle \boxcaptionstyle
% \maxfigfraction \figboxhang \figboxmargin 
%
% \captionstyle is executed for all floating box captions
% \boxcaptionstyle is executed for all marginal box captions.
%	Default \raggedright
% \maxfigfraction is the maximum fraction of a column that can be taken up
% 	by a marginal box before it gets converted to a float.
% 	Default .6
% dimen \figboxhang is the distance a marginal box hangs into the margin.
%	Default 0pt
% dimen \figboxmargin is the width of space between the text and a
% 	marginal box. 
%	Default .15in
%
%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%
%
% The most important macros for turning postscript into boxes are:
% 
% \boxeps: Form a box containing encapsulated postscript from a file at a
%	given scale.
% \boxps: Form a box containing postscript from a file at a given scale, 
% 	width, and height.
% 
%
% Usage: \boxeps[local commands] {file} {scale}
%	 \boxps[local commands] {file} {scale} {width} {height}
%
% The optional local commands are executed after scaling. As described
% 	below, they are useful for setting origins, non-uniform scaling, etc?
% file is the filename in the \figuredirectory and without the .ps
% 	extension.
% scale is a real number: 1 to use the drawn size.  0.9 to use 90% of
% 	drawn size.  Can be changed by local commands. (see below)
% width and height are dimensions of the box produced by \boxps.
%
%%%%%%%%%%%%%%%%
%
% options: \DVIscaling \figuredirectory \missingfigure \boxer
% local commands: \horizscale \vertscale
%
% \DVIscaling is the number the dvi to ps converter considers a unit
% 	scaling transformation.  Default: 1 for dvi2ps  --- 100 for
% 	some of Rokicki's versions of dvips.
%
% \globalscaling is the scaling applied to every picture --- useful
% 	for making double size figures for journals.  Default: 1
%
% \figuredirectory is the pathname where figure postscript files are kept.
%	Default: ./figure
%
% \missingfigure{file} is executed when the file is not found.
%	Default: \def\missingfigure#1{\hbox{Missing figure #1.ps}}
%
% \boxer is the command used by \boxps to make a box of the desired size
% 	containing the figure.  Possible commands depend on the origin of
% 	the figure, and include \llboxer \lcboxer \ulboxer and \ccboxer.
% 	(ll = lower left, ul = upper left, cc = dead center, etc.)
%	\boxer can be defined in the local commands or globally.
%
% Local commands \horizscale, and \vertscale can scale the picture
% 	horizontally and vertically by different factors.  \scale
% 	scales the picture uniformly.  Scales accumulate.
%
%%%%%%%%%%%%%%%%



%%%%%%%%%%%%%%%%
%
% Default options
%

\def\captionstyle{}
\def\boxcaptionstyle{\raggedright}

\def\maxfigfraction{.6}% 	--- max frac of column for marg figure

\newdimen\figboxmargin%		--- margin between text and picture
\figboxmargin = .15in

\newdimen\figboxhang%		--- amount to hang picture into margin
\figboxhang = 0pt

\def\DVIscaling{1}%		--- for dvi2ps
\def\globalscaling{1}%		--- for scaling everything
\def\figuredirectory{./figures}%--- where to find the .ps files 
\let\boxer=\llboxer%		--- default origin in lower left for non-
%				      encapsulated postscript figures

\def\missingfigure#1{\hbox{Missing figure #1.ps}}


%%%%%%%%%%%%%%%%
%
% Use latex internals
%
\catcode `\@=11
\special{! /@scaleunit 1 def }

\newbox\figurebox

\def\figbox{%	[place] box style label caption
\@ifnextchar[{\figboxaux}{\figboxaux[htb]}}

%
% Parse position parameters and try appropriate placement
%
\long\def\figboxaux[#1#2]#3#4#5#6{%	--- want left margin figure?
\writepict{{#3}{#4}{#5}{#6}}%		--- save figure if journalpicts
\setbox\figurebox\hbox{#3}%
\if l#1\tryleftbox{#4}{#5}{#6}%
\else%					--- want right margin figure?
\if r#1\tryrightbox{#4}{#5}{#6}%
\else%					--- want one or two column figure?
\if *#1\checktwocoloptions#2]{\box\figurebox}{#4*}{#5}{#6}%
\else\tryonecol[#1#2]{#4}{#5}{#6}%
\fi
\fi
\fi\ignorespaces}

%
% Try a placement; promote if too wide
%

\long\def\tryleftbox#1#2#3{%		--- does left margin figure fit?
\ifdim\wd\figurebox>\maxfigfraction\columnwidth \tryonecol[htb]{#1}{#2}{#3}%
\else\leftbox{\captionbox{\box\figurebox}{#1}{#2}{#3}}\fi}

\long\def\tryrightbox#1#2#3{%	--- does right margin figure fit?
\ifdim\wd\figurebox>\maxfigfraction\columnwidth \tryonecol[htb]{#1}{#2}{#3}%
\else\rightbox{\captionbox{\box\figurebox}{#1}{#2}{#3}}\fi}

\def\checktwocoloptions{%	--- make sure twocol has htb or p
\@ifnextchar]{\floatbox[htb}{\floatbox[}}

\long\def\tryonecol[#1]#2#3#4{%	--- does one column figure fit?
\ifdim\wd\figurebox>\columnwidth \floatbox[#1]{\box\figurebox}{#2*}{#3}{#4}%
\else\floatbox[#1]{\box\figurebox}{#2}{#3}{#4}\fi}

%
% Do the work for a floating box.
%
% \floatbox[place]{box} {style} {label} {caption}
%

\long\def\floatbox[#1]#2#3#4#5{%
\begin{#3}[#1]
\hbox to \hsize{\hfil#2\hfil}
\captionandlabel{#3}{#4}{#5}
\end{#3}
}


%
% Make a caption the width of the box with given style. 
%
%\captionbox {box} {style} {label} {[optshortcap] caption}
%
% options: \boxcaptionstyle 
%
%%%%%%%%%%%%%%%%
%
% This can be used with box commands (\hbox, \vbox, \mbox, and the like),
% along with \figbox with an empty caption, to place two or more captioned
% boxes in a single marginal or floating box.   
%
% e.g. \figbox{\hbox{
%		     \captionbox{ \boxeps{fig1}1} {figure} {f1} {a figure}
%		     \hskip 1in
%		     \captionbox{ \boxeps{tab1}1} {table} {t1} {a table}
%		    }} {figure} {ignored-label} {}
%

\long\def\captionbox#1#2#3#4{% box style label {[optshortcap] caption}
\setbox\figurebox\hbox{#1}%
\parbox[t]{\wd\figurebox}{%
\bigskip\box\figurebox
\let\captionstyle=\boxcaptionstyle
\captionandlabel{#2}{#3}{#4}
\bigskip
}}

%				--- caption and label if label is nonempty
\def\captionandlabel#1#2#3{% 	--- {style} {label} {caption}
\def\testit{#3}%
\ifx\testit\empty\else%		--- if non empty caption
\writecapt{{#1}{#2}{#3}}%	--- save for journal figs
\captypeunstarred#1*.%		--- remove optional stars
\getcaption#3\endc@ption%       --- parse the caption
\def\testit{#2}%		--- check for empty label
\ifx\testit\empty\else\label{#2}\fi
\fi}

\def\captypeunstarred#1*#2.{%	--- remove two-column star from style
\def\@captype{#1}}

%
% Parse the caption of the form {caption} or {[short] long caption} 
%

\def\getcaption{\@ifnextchar[{\getcaptwo}{\getcapone}}
\long\def\getcapone#1\endc@ption{\caption[#1]%
{\def\baselinestretch{1}\Large\normalsize\captionstyle\ignorespaces #1}}
\long\def\getcaptwo[#1]#2\endc@ption{\caption[#1]%
{\def\baselinestretch{1}\Large\normalsize\captionstyle\ignorespaces #2}}

%
% Do the right thing with an already captioned marginal box
%
% \leftbox{box}
% \rightbox{box}
%
% options: \figboxmargin \figboxhang \figuredirectory

\newdimen\figboxht
\newcount\figboxn


\newcount\figboxlines%		--- picture height in number of lines
\newdimen\figboxwid%		--- picture width

\newif\ifisleftbox

\long\def\leftbox#1{%
\setbox\figurebox\hbox{#1}\global\isleftboxtrue
\startmarginbox
\vadjust{\smash{\rlap{\hskip\hsize\hskip\figboxhang
\llap{\raise.7\baselineskip\box\figurebox\hskip\rightskip}}}}%
\endmarginbox%
}

\long\def\rightbox#1{%
\setbox\figurebox\hbox{#1}\global\isleftboxfalse
\startmarginbox
\smash{\llap{\raise.7\baselineskip\box\figurebox\hskip\figboxmargin}}%
\endmarginbox%
}

\def\startmarginbox{%
\ifvmode\passpict\let\endmarginbox=\indent
\else\message{WARNING: marginbox in not in vmode}\hfilneg\ \passpict
\let\endmarginbox=\relax\fi
%
\figboxht=\dp\figurebox%	 actual height
\advance\figboxht by 1.3\baselineskip% round up
\vskip\figboxht\penalty-300\vskip-\figboxht% filbreak trick
\divide\figboxht by\baselineskip%      how many lines?
\global\figboxlines=\figboxht
%
\global\figboxwid=\wd\figurebox
\global\advance\figboxwid by \figboxmargin
\global\advance\figboxwid by -\figboxhang
\setmypar\noindent}
%

%
% Useful macros
%
% for lengthening (and shortening) picture space
%
\def\addlines#1{\global\advance\figboxlines by #1\myparshape}
\def\zerolines{\origpar\global\figboxlines=0\myparshape}

%
% for passing any marginal figures
%
\def\passpict{\par\ifnum\figboxlines>1\vskip\figboxlines\baselineskip
\zerolines\fi}

\def\emptybox#1#2{\hbox to #1{\vbox to #2{\vss}\hss}}

%%%%%%%%%%%%%%%%%%%%%
%\par hacking  
% We define our own version of Tex's \par and tell Latex it is the original

\global\let\origpar=\@@par%	--- Latex's saved version of Tex's \par
\global\let\dopar=\origpar
\global\def\@@par{\dopar}
\@setpar{\dopar}

\def\setmypar{\global\let\dopar=\mypar
\global\prevgraf=0\myparshape}

\def\mypar{\origpar\global\advance\figboxlines by -\prevgraf%
\global\prevgraf=0\myparshape}

\def\myparshape{\relax%
\ifnum\figboxlines>1\theparshape \else
\global\hangindent=0pt\global\hangafter=1%  these sometimes get restored...
\global\let\dopar=\origpar\fi}

\def\theparshape{%
\ifisleftbox\global\hangindent=-\figboxwid 
\else\global\hangindent=\figboxwid \fi
\global\hangafter=-\figboxlines \global\advance\hangafter by 1%
}


%%%%%%%%%%%%%%%%
%
%  Macros to make the list of figures and captions used by journals
%
%  To use, execute \journalpicts{scalefactor} at the beginning of the
%  file.  All figbox figures and tables will be written to a .pic file
%  and all captions to a .cap file.  On \enddocument, these files are
%  read in and the lists of figures and captions are produced.
%  
%  For non-english versions, or to add other types of floats, the
%  macro \definefnum should be changed.
%

\def\definefnum#1{%		--- ugly latex hacking to get the
%		 			right figure/table name 
\def\fnum@figure{Figure \ref{#1}}%
\def\fnum@table{Table \ref{#1}}%
\def\fnum@code{Algorithm \ref{#1}}%
}

\def\writepict#1{}
\def\writecapt#1{}

%%%%%%%%%%%%%%%%
% \journalpicts{globalscalefactor} writes all pictures and captions to
% 	files and modifies \enddocument to read these files and
% 	produce lists of enlarged figures and of captions
% 

\def\journalpicts#1{% 		global scale factor
\newwrite\pictfile
\newwrite\captfile
%
\openout\pictfile\jobname.pic
\openout\captfile\jobname.cap
%
\gdef\writepict##1{\unexpandedwrite\pictfile{\doit##1}}%
\gdef\writecapt##1{\unexpandedwrite\captfile{\doit##1}}%
%
\global\let\ENDdocument=\enddocument
\gdef\enddocument{\DOjournalpicts{#1}\ENDdocument}
}

%
%	generate enlarged figures 1 per page and list captions
%
\def\DOjournalpicts#1{{%
\def\writepict##1{}\closeout\pictfile
\def\writecapt##1{}\closeout\captfile
\@fileswfalse%			--- turn off toc, lof, and so on.
%
\onecolumn
\def\globalscaling{#1}
\def\doit##1##2##3##4{%		--- print a picture on blank page
%					{box}{style}{label}{caption}
\figboxaux[t]{\hss##1\hss}{##2}{}{}%
\vspace*{1in}
\definefnum{##3}%		--- use Figure \ref{label} or Table \ref{label}
\captionandlabel{##2}{}{##4}
\clearpage}%
%
\input\jobname.pic
%
\def\doit##1##2##3{%		--- print caption
%					{style}{label}{caption}
\definefnum{##2}%		--- use Figure \ref{label} or Table \ref{label}
\captionandlabel{##1}{}{##3}}%
%
\raggedright\let\captionstyle=\raggedright
\def\@makecaption##1##2{##1: ##2\par}%  --- Be sure captions aren't centered
%
\input\jobname.cap
}}%				--- to be followed by \enddocument



%%%%%%%%%%%%%%%%
%
%  Box macros
%
%%%%%%%%%%%%%%%%
%
% \boxeps[local commands] {file} {scale}
%
% options \DVIscaling \figuredirectory \scale \horizscale \vertscale
% \missingfigure \globalscaling
%
% \boxps[local commands] {file} {scale} {width} {height}
%
% \scale \horizscale \vertscale 

%
%  Various `boxers' --- which one is used depends on where the origin
%  of the picture is.  If you are using the bounding boxes of
%  encapsulated postscript, just use the default \llboxer.  Otherwise,
%  you have to figure out where the origin is and set \boxer appropriately.
%

\def\llboxer#1{\vbox to \figboxht{\vfil\hbox to \figboxwid{#1\hfill}}}
\def\lcboxer#1{\vbox to \figboxht{\vfil\hbox to \figboxwid{\hfill#1\hfill}}}
\def\oldboxer#1{\vbox to \figboxht{\vfil
		      \hbox to \figboxwid{\hfill\llap{#1\hskip4.25in}\hfill}}}
\def\ulboxer#1{\vbox to \figboxht{\hbox to \figboxwid{#1\hfill}\vfil}}
\def\ccboxer#1{\vbox to \figboxht{\vfil
			\hbox to \figboxwid{\hfill#1\hfill}\vfil}}

% a macro to strip the pt off a dimension
%
{\catcode`\p=12\catcode`\t=12
\gdef\removedimen#1pt{#1}}

\def\defscaled#1#2{#2=\DVIscaling#2%
\xdef#1{\expandafter\removedimen\the#2}}

\def\DVIspace{ }
\newdimen\hscalefactor
\newdimen\vscalefactor

\def\scale#1{\horizscale{#1}\vertscale{#1}}
\def\horizscale#1{\hscalefactor=#1\hscalefactor\figboxht=#1\figboxht}
\def\vertscale#1{\vscalefactor=#1\vscalefactor\figboxwid=#1\figboxwid}

%%%%%%%%%%%%%%%%
%

\def\boxps{%
\@ifnextchar[{\boxpsaux}{\boxpsaux[\relax]}}

\def\boxpsaux[#1]#2#3#4#5{%
{\figboxwid#4\figboxht#5\hscalefactor=1pt\vscalefactor=1pt%
\scale{#3}%
\scale{\globalscaling}%
#1%
\defscaled\DVIhscale\hscalefactor
\defscaled\DVIvscale\vscalefactor
\boxer{\special{psfile=\figuredirectory/#2.ps \DVIspace
		hscale=\DVIhscale\DVIspace 
		vscale=\DVIvscale}}}%
}


%%%%%%%%%%%%%%%%
% The following is from tex/inputs/epsf.tex by Tom Rokicki
% with slight modifications by Jack Snoeyink.
%
%   Written by Tomas Rokicki of Radical Eye Software, 29 Mar 1989.
%
%   Include an ecapsulated postscript graphic.
%   Works by finding the bounding box comment.
%
\newread\Epsffilein
\newif\ifEpsffileok
\newif\ifEpsfbbfound

\newdimen\pspoints
\pspoints=1in
\divide\pspoints by 72


\def\boxeps{%
\@ifnextchar[{\boxepsaux}{\boxepsaux[\relax]}}
\def\boxepsaux[#1]#2#3{%
%
%   The first thing we need to do is to open the
%   PostScript file, if possible.
%
\openin\Epsffilein=\figuredirectory/#2.ps 
\ifeof\Epsffilein\message{I couldn't open \figuredirectory/#2.ps }%
\missingfigure{#2}
\else
%
%   Okay, we got it.  Now we scan lines until we find one
%   that doesn't start with a percentage sign.  We're
%   looking for the bounding box comment.
%
   {\Epsffileoktrue\Epsfbbfoundfalse
    \catcode`\%=11 \catcode`\\=11
    \catcode`\{=11 \catcode`\}=11
    \catcode`\$=11 \catcode`\^=11
    \catcode`\&=11 \catcode`\#=11
    \catcode`\~=11 \catcode`\_=11
    \loop
       \read\Epsffilein to \Epsffileline
       \ifeof\Epsffilein\Epsffileokfalse\else
%
%   Now we check to make sure the first character is a % sign,
%   and that the rest are `%BoundingBox:' if necessary.
%
          \expandafter\Epsfaux\Epsffileline . .\\%
       \fi
   \ifEpsffileok\repeat
   \ifEpsfbbfound
	\figboxht=\Epsfury\pspoints
	\advance\figboxht by-\Epsflly\pspoints
	\figboxwid=\Epsfurx\pspoints
	\advance\figboxwid by-\Epsfllx\pspoints
   \else
	\message{No bounding box comment in \figuredirectory/#2.ps }%
	\figboxwid=2in\figboxht=1in%
   \fi%
   \immediate\closein\Epsffilein
   \hscalefactor=1pt\vscalefactor=1pt%
   \scale{#3}%
   \scale{\globalscaling}%
   #1%
%
   \defscaled\DVIhscale\hscalefactor
   \defscaled\DVIvscale\vscalefactor
%
   \hscalefactor=-\Epsfllx\hscalefactor
   \hscalefactor=1.00375\hscalefactor%	--- 72.27/72 = TeXpoints/PSpoints
   \defscaled\DVIhoffset\hscalefactor
%
   \vscalefactor=-\Epsflly\vscalefactor
   \vscalefactor=1.00375\vscalefactor%	--- 72.27/72 = TeXpoints/PSpoints
   \defscaled\DVIvoffset\vscalefactor
%
   \llboxer{\special{psfile=\figuredirectory/#2.ps \DVIspace
		hoffset=\DVIhoffset\DVIspace
		voffset=\DVIvoffset\DVIspace
                hscale=\DVIhscale\DVIspace 
                vscale=\DVIvscale}} }%
\fi
}%
%
%   We need these for comparison purposes.
%
{\catcode`\%=11 \global\let\Epsfpar=\par
\global\let\Epsfpercent=%\global\def\Epsfbblit{%BoundingBox:}}%
%
%   This is our function that checks for `%BoundingBox:' and grabs the
%   values if they are found.
%
\long\def\Epsfaux#1#2 #3\\{\relax\ifx#1\Epsfpercent
   \def\testit{#2}\ifx\testit\Epsfbblit
      \Epsfsize #3 . . . .\\%
      \global\Epsffileokfalse
      \global\Epsfbbfoundtrue
   \fi\else\ifx#1\Epsfpar\else\global\Epsffileokfalse\fi\fi}%
%
%   Here we grab the values and stuff them in the appropriate definitions.
%
\def\Epsfsize#1 #2 #3 #4 #5\\{\global\def\Epsfllx{#1}\global\def\Epsflly{#2}%
   \global\def\Epsfurx{#3}\global\def\Epsfury{#4}}%




\catcode`\@=12 			% done with with internals

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% For backward compatability
%
% \pic file; height in inches; width in inches; caption\par
% \picsc file; ht (in); wid (in); scale; caption\par
%
% \mpic file; height in inches; width in inches; caption\par
% \mpicsc file; ht (in); wid (in); scale; caption\par
%
%%%%%%%%%%%%%%%%

\def\pic#1;#2;#3;#4\par{\picsc#1;#2;#3;1;#4\par}% file; wd; ht; caption 

\def\picsc#1;#2;#3;#4;#5\par{% file; wd; ht; scale; caption
\figbox[htb]{\boxeps{#1}{#4}%{#2in}{#3in}%
}{figure}{#1}{%
% (#1: #2x#3 sc #4) % 			Uncomment for debugging
#5}}


\def\mpic#1;#2;#3;#4\par{\mpicsc#1;#2;#3;1;#4\par}% file; wd; ht; caption 

\def\mpicsc#1;#2;#3;#4;#5\par{% file; wd; ht; scale; caption
\figbox[l]{\boxeps{#1}{#4}%{#2in}{#3in}%
}{figure}{#1}{%
% (#1: #2x#3 sc #4) % 			Uncomment for debugging
#5}}





==> MobiHoc'22_Communication_Contention_Tech_Report/Supporting_Preambles/symbols_commands.tex <==
% !TEX root = ../Multi_Momentum_INFOCOM.tex

%\renewcommand{\thesection}{\Roman{section}}
%\renewcommand{\thesubsection}{\Roman{section}-\Alph{subsection}}
%\renewcommand{\thesubsubsection}{\Alph{subsection}.\arabic{subsubsection}}

\newcommand{\A}{\mathbf{A}}
\renewcommand{\a}{\mathbf{a}}
\newcommand{\B}{\mathbf{B}}
\newcommand{\Bt}{\mathbf{B}}
\renewcommand{\b}{\mathbf{b}}
\newcommand{\bt}{\mathbf{b}}
\renewcommand{\c}{\mathbf{c}}
\newcommand{\ct}{\widetilde{\mathbf{c}}}
%\newcommand{\C}{\mathbf{C}}
\newcommand{\Ch}{\widehat{\mathbf{C}}}
\newcommand{\D}{\mathbf{D}}
\newcommand{\Dh}{\widehat{\mathbf{D}}}
\renewcommand{\d}{\mathbf{d}}
\newcommand{\E}{\mathbf{E}}
\newcommand{\e}{\mathbf{e}}
\newcommand{\et}{\widetilde{\mathbf{e}}}
\newcommand{\f}{\mathbf{f}}
\newcommand{\F}{\mathbf{F}}
%\newcommand{\G}{\mathbf{G}}
\newcommand{\g}{\mathbf{g}}
\newcommand{\I}{\mathbf{I}}
\newcommand{\J}{\mathbf{J}}
\newcommand{\K}{\mathbf{K}}
\newcommand{\M}{\mathbf{M}}
\newcommand{\m}{\mathbf{m}}
\newcommand{\mh}{\widehat{\mathbf{m}}}
\newcommand{\Mh}{\widehat{\mathbf{M}}}
\newcommand{\Mt}{\widetilde{\mathbf{M}}}
\newcommand{\Mb}{\overline{\mathbf{M}}}
\newcommand{\N}{\mathbf{N}}
\newcommand{\n}{\mathbf{n}}
\newcommand{\p}{\mathbf{p}}
\renewcommand{\P}{\mathbf{P}}
\newcommand{\Q}{\mathbf{Q}}
\newcommand{\q}{\mathbf{q}}
\newcommand{\R}{\mathbf{R}}
\renewcommand{\r}{\mathbf{r}}
\renewcommand{\S}{\mathbf{S}}
\newcommand{\Sh}{\widehat{\mathbf{S}}}
\newcommand{\s}{\mathbf{s}}
\renewcommand{\t}{\mathbf{t}}
\newcommand{\T}{\mathbf{T}}
\newcommand{\Th}{\widehat{\mathbf{T}}}
%\newcommand{\U}{\mathbf{U}}
\renewcommand{\u}{\mathbf{u}}
\newcommand{\V}{\mathbf{V}}
\renewcommand{\v}{\mathbf{v}}
\newcommand{\W}{\mathbf{W}}
\newcommand{\w}{\mathbf{w}}
\newcommand{\wt}{\widetilde{\mathbf{w}}}
\newcommand{\wts}{\widetilde{w}}
\newcommand{\X}{\mathbf{X}}
\newcommand{\Xh}{\widehat{\mathbf{X}}}
\newcommand{\x}{\mathbf{x}}
\newcommand{\xt}{\widetilde{\mathbf{x}}}
\newcommand{\xh}{\widehat{\mathbf{x}}}
\newcommand{\Y}{\mathbf{Y}}
\newcommand{\y}{\mathbf{y}}
\newcommand{\z}{\mathbf{z}}
\newcommand{\Z}{\mathbf{Z}}
\newcommand{\yt}{\widetilde{\mathbf{y}}}
\newcommand{\rb}{\mathbf{b}}
\newcommand{\rvec}{\mathbf{r}}
\newcommand{\0}{\mathbf{0}}
\newcommand{\1}{\mathbf{1}}
\newcommand{\Hc}{\mathbf{H}}
\newcommand{\tHc}{\widetilde{\mathbf{H}}}
\newcommand{\hHc}{\overline{\mathbf{H}}}
\newcommand{\DL}{\mathbf{DL}}
\newcommand{\mLambda}{\mathbf{\Lambda}}
\newcommand{\vlambda}{\boldsymbol{\lambda}}
\newcommand{\mOmega}{\mathbf{\Omega}}
\newcommand{\mOmegab}{\overline{\mathbf{\Omega}}}
\newcommand{\mGamma}{\mathbf{\Gamma}}
\newcommand{\mPi}{\mathbf{\Pi}}
\newcommand{\mPsi}{\mathbf{\Psi}}
\newcommand{\mPsib}{\overline{\mathbf{\Psi}}}
\newcommand{\valpha}{\mathbf{\alpha}}
\newcommand{\vpi}{\boldsymbol \pi}
\newcommand{\Sone}{\mathcal{S}}
\newcommand{\tr}{\mathrm{Tr}}
\newcommand{\new}{\mathrm{new}}
\newcommand{\net}{\mathrm{net}}
\newcommand{\link}{\mathrm{link-phy}}
\newcommand{\LL}{\mathbf{L}}
\newcommand{\Out}[1]{\mathcal{O}\left( #1 \right)}
\newcommand{\In}[1]{\mathcal{I}\left( #1 \right)}
\newcommand{\Int}[1]{\mathcal{F}\left( #1 \right)}
\newcommand{\sInt}[1]{\hat{\mathcal{F}}\left( #1 \right)}
\renewcommand{\Re}[1]{\mbox{$\mathfrak{Re} \left( #1 \right)$}}
\renewcommand{\Im}[1]{\mbox{$\mathfrak{Im} \left( #1 \right)$}}
\newcommand{\Resq}[1]{\mbox{$\mathfrak{Re}^{2} \left( #1 \right)$}}
\newcommand{\Imsq}[1]{\mbox{$\mathfrak{Im}^{2} \left( #1 \right)$}}
\newcommand{\LTM}{\langle L \rangle}
\newcommand{\con}[1]{\overline{#1}}
\newcommand{\abs}[1]{\mbox{$\lvert #1 \rvert$}}
\newcommand{\norm}[1]{\mbox{$\left\lVert #1 \right\rVert$}}
\newcommand{\dual}{$\mathbf{D}^{\mathrm{CRPBA}}$}
\newcommand{\dnet}{$\mathbf{D}^{\mathrm{CRPBA}}_{\net}$}
\newcommand{\dlink}{$\mathbf{D}^{\mathrm{CRPBA}}_{\link}$}
\newcommand{\Pwrcon}{\Omega_{+}(n)}
\newcommand{\src}[1]{\mathrm{Src}(#1)}
\newcommand{\dst}[1]{\mathrm{Dst}(#1)}
\newcommand{\rx}[1]{\mathrm{Rx}(#1)}
\newcommand{\tx}[1]{\mathrm{Tx}(#1)}
\newcommand{\Dy}{\Delta \y}
\newcommand{\Dyt}{\Delta \widetilde{\y}}
%\newcommand*\circled[1]{\tikz[baseline=(char.base)]{
%            \node[shape=circle,draw,inner sep=2pt] (char) {#1};}}
%\newcommand{\seq}[1]{\mbox{$\{ #1 \} $}}
%\newcommand{\myref}[1]{(\ref{#1})}
%\newcommand{\sd}{\mbox{$\stackrel{\Delta}{=}$}}
%\newcommand{\sci}[2]{\mbox{$#1 \times 10^{- #2}$}}
%%\newtheorem{thm}{Theorem}

\newtheorem{thm}{Theorem}
\newtheorem{cor}[thm]{Corollary}
\newtheorem{lem}[thm]{Lemma}
\newtheorem{claim}{Claim}
\newtheorem{prop}[thm]{Proposition}
\newtheorem{ex}{Example}[section]
%\theoremstyle{definition}
\newtheorem{defn}[thm]{Definition}
%\theoremstyle{remark}
\newtheorem{finalremark}[thm]{Final Remark}
\newtheorem{rem}{Remark}
\newtheorem{sol}{Solution}
\newtheorem{fact}{Fact}
%\numberwithin{equation}[section]

\newcommand{\po}{\mbox{$ \mbox{P}_{\rm out}$}}
\newcommand{\ga}{\bar{\gamma}}
\newcommand{\mtrx}[1]{\mbox{$\left[\begin{array} #1 \end{array}\right]$}}
\newcommand{\mtrxt}[1]{\mbox{$\begin{array} #1 \end{array}$}}
\newcommand{\diag}[1]{\mathrm{Diag}\left\{ #1 \right\}}
\newcommand{\diaginv}[1]{\mathrm{Diag}^{-1}\left\{ #1 \right\}}
\newcommand{\diagtran}[1]{\mathrm{Diag}^{T}\left\{ #1 \right\}}
\newcommand{\diagv}[1]{\mathrm{diag}\left\{ #1 \right\}}
\newcommand{\etal}{{\em et al. }}
\newcommand{\ind}{\mathbbm{1}}
\newcommand{\vbeta}{\boldsymbol \beta}

%\renewcommand{\algorithmicrequire}{\textbf{Input:}}
%\renewcommand{\algorithmicensure}{\textbf{Output:}}
%\algtext*{EndWhile}% Remove "end while" text
%\algtext*{EndIf}% Remove "end if" text
%\algtext*{EndFor}% Remove "end while" text
%\algtext*{EndFunction}% Remove "end if" text
%\algtext*{EndProcedure}% Remove "end while" text
%%\algtext*{EndIf}% Remove "end if" text

%\newcommand{\algorithmicinitialize}{\textbf{Initialization:}}
%\newcommand{\algorithmicmainiterate}{\textbf{Main Iteration:}}
%\newcommand{\algorithmicprimal}{\textbf{Primal Newton Direction:}}
%\newcommand{\algorithmicdual}{\textbf{Dual Variables Update:}}


==> Sec4_Model/Sec4_Model_backup.tex <==
% !TEX root = ../ML_Networking_INFOCOM'20.tex


\section{System Model and Problem Formulation} \label{sec:model_formulation}

In this section, we first introduce our system model, then present our general problem formulation for DDL training on shared, multi-tenant GPU clusters.
\subsection{System Model}
We consider a GPU cluster consists of servers that has limited network resources and takes the communication contention into consideration for job scheduling.
% connected with a network switch of sufficiently large bandwidth.
We let $\mathcal{S}$ represent the set of servers in the GPU cluster.
Each server $s\in\mathcal{S}$ has configured with various number of GPU capacity.
Assume that GPUs are homogeneous and synchronized.
The network performance of each server is modelled by Eqn.~(\ref{contention_reduce}) and shared among different jobs.
The GPU cluster accepts DL job requests from users, and rent GPU resource from the cluster for running the jobs.
We assume that the jobs are processed periodically and 
we use $\mathcal{J}$ to represent the set of {\em active} jobs to be trained in the current scheduling interval. 
% and let $d_j$ denote the submission time-slot of job $j\in\mathcal{J}$.
% The jobs are executed over a large time span $T$ in a time-slotted system where the scheduling time-horizon is denoted as $\mathcal{T}$. 
% The length of a time slot is potentially much larger than the duration of a training epoch, for the repeated training of the input dataset in each time slot.
% We assume the  at least one jobs is being executed at each scheduling time slot.
% There is no available information about the future upcoming jobs.
The number of GPUs of each job is specified by the user upon its submission. 
%and remains unchanged throughout the entire training process.
% We use $\mathcal{G}_j$ and $G^j$ be the set of GPUs and the number of GPUs required by job $j\in\mathcal{J}$, respectively.
% We use $G_j$ to denote the number of GPUs required by job $j\in\mathcal{J}$.
The set of GPUs can be allocated within the same server or across different servers, and will remain unchanged throughout the entire training process.
We also assume each GPU can only be occupied by one worker at any time.
% The jobs may complete at certain time slot, and we employ the dynamic scheduling.
% The job scheduling is in an online fashion, and the scheduling problem is solved at each time slot.
% Moreover, no preemption is allowed in the system, i.e., once the jobs gets started, it can not be interrupted.
% We assume that the system should be able to reassign the resources freed from the terminated jobs efficiently.
% Also, when a job runs to completion, the running jobs either can continue their training with the same number of GPUs on the same or different servers.
% Since the GPU resource is very expensive as well as avoid fragmentation, which is reserved for jobs require larger number of GPUs, the cloud is potentially assign ``just enough" servers to process the submitted jobs.

% We do not consider overall GPU resource capacity constraint in the cluster, as a cloud typically provides sufficient resources for serving a large number of customers.

% \section{Problem Formulation}

% \begin{align}
%     \text{Minimize } &c\sum_jF_jt_j\!+\!\mu\big[\sum_h(N_h\chi_h\!-\!\sum_jy_h^j)\!+\!\sum_k(N_k\chi_k\!-\!\sum_jz_k^j)\big]\\
%     \text{subject to }
%     &\sum_jy_h^j\leq N_h, \forall h\in\mathcal{H},\\
%     &\sum_jz_k^j\leq N_k, \forall k\in\mathcal{K},\\
%     &\sum_hy_h^j+\sum_kz_k^j=G_j, \forall j\in\mathcal{J},\\
%     &\sum_hy_h^j\big /\sum_kz_k^j=\gamma_j, \forall j\in\mathcal{J},\\
%     \label{eqn:k}&k=\alpha\max\{\max_h\sum_jy_h^j,\max_k\sum_jz_k^j\},\\
%     &t_j=a_j+kb_jM_j+(k-1)\eta_jM_j,\forall j\in\mathcal{J},\\
%     \label{eqn:chi_h}&\chi_h\geq \mathbbm{1}\{y_h^j\geq 1\}, \forall h\in\mathcal{H}, j\in\mathcal{J},\\
%     \label{eqn:chi_k}&\chi_k\geq \mathbbm{1}\{z_h^j\geq 1\}, \forall k\in\mathcal{K}, j\in\mathcal{J},\\
%     &\chi_h,\chi_k\in\{0,1\}, y_h^j,z_k^j\in\mathbb{Z}^+.
% \end{align}

% {\em 1)} Transformation of Eqn.~(\ref{eqn:k})

% \begin{align*}
%     k&\geq \alpha\sum_jy_h^j, \forall h\in\mathcal{H},\\
%     k&\geq \alpha\sum_jz_k^j, \forall k\in\mathcal{K}.
% \end{align*}

% {\em 2) } Transformation of Eqns.~(\ref{eqn:chi_h}) and (\ref{eqn:chi_k})

% \begin{align*}
%     y_h^j&\geq 1+ G_j(x_h^j-1), \forall h\in\mathcal{H}, j\in\mathcal{J},\\
%     z_k^j&\geq 1+ G_j(x_k^j-1), \forall k\in\mathcal{K}, j\in\mathcal{J},\\
%     x_h^j&\geq \frac{y_h^j}{G_j}, \forall h\in\mathcal{H}, j\in\mathcal{J},\\
%     x_k^j&\geq \frac{z_k^j}{G_j}, \forall k\in\mathcal{K}, j\in\mathcal{J},\\
%     \chi_h&\geq x_h^j, \forall h\in\mathcal{H}, j\in\mathcal{J},\\
%     \chi_k&\geq x_k^j, \forall k\in\mathcal{K}, j\in\mathcal{J}.
% \end{align*}



\subsection{Problem Formulation}

\begin{figure}[t]
    \centering
    \includegraphics[width=0.45\textwidth]{Figures/fig_placement.eps}
    \caption{Scenarios on different placement schemes.}\label{fig:placement}
%        \vspace{-.1in}
\end{figure}

{\bf 1) Learning Job Modeling:} 
% We use a binary variable $x_j$ to indicate whether job $j$ is executed ($x_j=1$) or not ($x_j=0$).
We use $y_{js}$ to denote the number of GPUs scheduled to server $s\in\mathcal{S}$ of job $j$.
We also use $\mathcal{S}_j$ to denote the set of servers that are used to place GPUs of job $j$.
We let $G_j$ be the number of GPUs required by job $j$.
Let $k_j$ be the maximum number of concurrent running communication tasks over all servers that associated with job $j$.
Here, we assume that $k_j$ is proportional to the max number of inter-connect communication jobs over all servers, which can be viewed as the expectation result.
%including sending or receiving gradients.
The intuition is that as the number of jobs increases, the number of concurrent running communication tasks should also be increased.
We use $\alpha$ to denote such linear coefficient.
In order to calculate $k_j$, we need to consider following two cases: 1) When all job $j$'s GPUs are placed to the same server, where its workers using intra-connect communication to training the job; 2) At least two servers are scheduled to place job $j$'s servers,  where its workers utilizing inter-connect communication.
Then the server that becomes the  bottleneck (i.e., has maximum number of scheduled jobs) needs to be found.
Take Fig.~\ref{fig:placement} as an example, Job 1 requires two GPU, which uses intra-connect communication ($|\mathcal{S}_1|=1$), and no resource contention is introduced.
Job 3 places each of its GPU into two servers (server 1 and 2), and it uses inter-connect communication.
However, no other inter-connect communication jobs are placed to server 1 and 2, thus no resource contention occurs.
With respect to job 2 and 4, their GPUs are placed to both server 3 and 4, and as a result,  the resource contention happens between these two jobs.
We can see from the figure that both server 3 and 4 has two different jobs (job 2 and 4), thus the bottleneck server in this case lies in both servers.


Based on the above discussion, we can compute $k_j$ as follows:
\begin{align}
    \label{eqn:k_j}k_j\!=\!\begin{cases}
    0, \quad\text{if }|\mathcal{S}_j|=1,\\
%    \alpha \max_{s\in\mathcal{S}_j}\sum_{j'\in\mathcal{J}}\mathbbm{1}\{y_{j's}\geq 1\},  \quad\text{if } |\mathcal{S}_j|>1.
	\alpha p_j,  \quad\text{if } |\mathcal{S}_j|>1,
    \end{cases}
\end{align}
%The first case corresponds to workers of job $j$ using internal communication since there exists some server that is scheduled to place all its GPUs.
%And the second case corresponds to workers of job $j$ using external communication since at lease two servers are arranged to host its $G_j$ workers.

% We Let $M_j$ to denote the mini-batch size of job $j$.
% Let $m^j$ denote the model size for the DNN training job $j$.
% Let $k[t]$ be the maximum number of concurrent running jobs over all the servers in time slot $t$, which can be computed as $k[t]=\max_{s\in\mathcal{S}}\{\sum_{j\in\mathcal{J}}y_s^j[t]>0\},\forall t\in\mathcal{T}$.
% We use $p_j$ to denote the computation time for each minibatch of job $j$.
where $p_j\triangleq \max_{s\in\mathcal{S}_j}\sum_{j'\in\mathcal{J}}\mathbbm{1}\{y_{j's}\geq 1\}$, i.e., the maximum number of inter-connect communication jobs over all servers associated with job $j$.

Next we can derive the per-iteration time of job $j$ by following the performance modeling Eqn~(\ref{contention_model}).
Note that the message size  $m_j$ (i.e., the size of gradients) is related to mini-batch size and the DNN model characteristics (e.g., number of layers, number of neurons at each layer).
%Here, we assume the gradient size $m_j$ is linear proportional to mini-batch size $M_j$, i.e., $m_j=\beta_jM_j$.
And we can obtain the following per-iteration time of job $j$:
\begin{align}
    \label{eqn:t_j}t_j=d_j+h_jk_j, \quad\forall j\in\mathcal{J},
\end{align}
%where $d_j\!\triangleq\! a_j+(\tau_j\beta_j+t_j^f-\eta_j\beta_j)M_j+t_j^b$ and $e_j\!\triangleq\! \beta_j(b_j+\eta_j)$.
where $d_j\triangleq a_j-\eta_jm_j+t_j^fM_j+t_j^b$ and $h_j\triangleq (e_j-\eta_j)m_j$.

% Let $\mathcal{T}_j$ be the set of time slots that job $j$ is executing.
% We use $\hat{t}_j$ to denote the completion time slot for job $j$.
% Note that if $y_s^j[t]>0$ over some server $s$ in time slot $t$, then job $j$ is being processed, thus we can use $\mathbbm{1}\{y_s^j[t]>0\}$ as the decision variable to indicate whether the job is running or not.
To ensure that there are exactly $G_j$ number of GPUs scheduled to job $j$ during its training time,
% and the allocated GPUs can be migrated throughout the entire training process,
we have:

\begin{align}
    %  \label{eqn:gpu}&\sum_{s\in\mathcal{S}}\sum_{g\in\mathcal{G}_j}y_{gs}^j[t] = G^j\cdot x_j, \quad\forall d_j \leq t\leq \hat{t}_j,j\in\mathcal{J}, \\
    \label{eqn:gpu}&\sum_{s\in\mathcal{S}}y_{js} = G_j, \quad \forall j\in\mathcal{J}.
    %  \label{eqn:gang}&y_{gs}^j[t]=y_{gs}^j[t+1], \quad \forall d_j\leq t<\hat{t}_j, g\in\mathcal{G}_j, s\in\mathcal{S},  j\in\mathcal{J}.
\end{align}
% We use $F_j\triangleq E_jG_jM_j$ to denote the total number of mini-batch training iterations for job $j$. 
% % which is specified by the user on submission.\footnote{In practice, to prevent spending excessively long time to wait the DNN training process to converge, a maximum number of iterations is usually set by the user.}
% In the DDL training setting, each worker (GPU) then needs to train $E^j\triangleq F^j/G_j$ if $G^j$ number of workers are scheduled for job $j$.
% Here we estimate the training iterations with the possible maximum number of GPUs can be deployed (we will show later that at least $G^j-1$ GPUs will be scheduled for each job).
% Since in practice, the model usually converges when only around 40\% of specified training iterations are conducted\cite{cite}.
% In other words, even with at most one fewer worker actually placed, the model typically can have good enough performance with the fewer number of training iterations.
% To make sure the total number of iterations trained for job $j$ over the entire training horizon does not exceed the specified number of iterations, which indicates that there is no extra utility to train more than $E^j$ iterations, we have:
% \begin{align}
%     \label{eqn:iter}&\sum_{t\in\mathcal{T}}e^j[t]\leq E^j,\quad\forall j\in\mathcal{J}.
%     % \label{eqn:iter}&\sum_{t\in\mathcal{T}}\frac{1}{t_f^jb^j\!+\!t_b^j\!+\!a^j\!+\!k[t]b^jm^j\!+\!(k[t]\!-\!1)\eta^j m^j}\!\geq\!E^jx_j,\quad\forall j\in\mathcal{J}.    
% \end{align}

{\bf 2) Chosen Server  Modeling: }
We use a binary variable $\chi_s$ to indicate whether server $s$ is chosen to schedule GPUs in the current interval.
Note that as long as some GPU is placed to server $s$, then $\chi_s=1$, thus we can have the following equation:
\begin{align}
    &\label{eqn:chi_s}\chi_s=\mathbbm{1}\{\sum_{j\in\mathcal{J}}y_{js}\geq 1\},\quad \forall s\in\mathcal{S}.
\end{align}

{\bf 3) Resource Constraint Modeling:} We use $N_s$ to denote the maximum number of GPUs can be scheduled to server $s\in\mathcal{S}$.
To ensure that the allocated GPUs do not exceed each server's capacity, we have:
\begin{align}
    \label{eqn:cap}&\sum_{j\in\mathcal{J}}y_{js}\leq N_s, \quad\forall s\in\mathcal{S}.
\end{align}

Finally, to define the decision variables domain, we have:

\begin{align}
    \label{eqn:int}&y_{js}, \in\mathbb{Z}^+, k_j, t_j\geq 0, \chi_s\in\{0,1\},
    \forall s\in\mathcal{S}, j\in\mathcal{J}.
\end{align}
% Note that for job $j$, its completion time $\hat{t}_j$ corresponds to the latest time-slot where there remain some active workers allocated for it.
% Therefore, we have:
% \begin{align}
%     \label{eqn:t}&\hat{t}_j = \arg\max_{t\in\mathcal{T}}\{\sum_{s\in\mathcal{S}}\sum_{g\in\mathcal{G}_j}y_{gs}^j[t]>0\},\quad\forall j\in\mathcal{J}.
% \end{align}

% Lastly, to ensure that there is no workers allocated before $j$'s arrival, we have:
% \begin{align}
%   \label{eqn:pri_arr}&y_{s}^j[t]=0,\quad\forall t<d_j, s\in\mathcal{S},j\in\mathcal{J}.
%   \label{eqn:pri_arr}&y_{s}^j[t]\in \mathbb{Z}^+,\quad\forall t\in\mathcal{T}, s\in\mathcal{S},j\in\mathcal{J}.
%   &y_{s}^j[t]\in \mathbb{Z}^+\text{ and }  \label{eqn:pri_arr}y_{s}^j[t]\leq G^j ,\quad\forall t\in\mathcal{T}, s\in\mathcal{S},j\in\mathcal{J}.
% \end{align}

{\bf 3) Objective Function and Problem Statement: } 
% We use the function  $f_j(\sum_{t\in\mathcal{T}}e^j[t])$ to denote the concave utility function for job $j$, which can deliver the results with respect to partial training iterations $\sum_{t\in\mathcal{T}}e^j[t]$.
In this paper, our goal is to minimize the overall operations cost, including the execution cost and the fragmentation cost, for all jobs from the system's perspective.
% We let $c_1$ be the time unit price paid by users, and let $c_2$ be the time unit operations cost.
We let $c$ be the time unit execution cost for running the GPUs in the cluster.
Let $E_j$ be the number of epochs to be trained of job $j$, and then  $F_j=E_jG_jM_j$ is the number of mini-batch iterations to be trained of job $j$.
The term $\sum_{j\in\mathcal{J}}cF_jt_j$ corresponds to the overall execution cost associated with each job, which is proportional to the training time.
% Thus $c\sum_{j\in\mathcal{J}}F_jt_j$ will be the total benefit by running GPUs, where $c\triangleq c_1-c_2$.
Also the term $\mu\sum_{s\in\mathcal{S}}(N_s\chi_s-\sum_{j\in\mathcal{J}}y_{js})$ is the fragmentation cost, which is measured by the difference between the number of allocated GPUs and the number of available GPUs from each selected server $s$, and $\mu$ is a penalty coefficient for unused GPUs.
On one hand, the system tends to avoid the resource contention to minimize the overall execution cost, i.e., spreading jobs over all servers.
On the other hand, the system also tends to pack jobs into servers to reduce the fragmentation cost.
Hence, to minimize the operations cost of the objective function, the system tends to find a balance between spread jobs over servers and exploit all available GPU resources for each selected server.
% In other words, the system tries to avoid too much server fragmentation, which can save internal communication for coming jobs that require larger number of GPUs.
Putting all constraints and the objective function together, the offline distributed DDL job scheduling problem~DDLJS can be formulated as:
\begin{align*}
{\bf DDLJS: } \underset{\mathbf{y,k,t,\chi}}{\text{ Minimize }} &c\sum_{j\in\mathcal{J}}F_jt_j+\mu\sum_{s\in\mathcal{S}}(N_s\chi_s-\sum_{j\in\mathcal{J}}y_{js})\\
    \text{subject to } 
    &\text{Constraints}  (\ref{eqn:k_j})-(\ref{eqn:int}).  
\end{align*}
It can be seen that Problem~DDLJS is a mixed integer nonlinear program (MINLP), which is NP-hard in general.
It involves a non-deterministic constraint~(\ref{eqn:k_j}), and two indicator functions in constraints~(\ref{eqn:k_j})(\ref{eqn:chi_s}), which are not amenable for conventional optimization techniques.
Overcoming these challenges constitutes the main subjects in the next section.
To conclude this section, we summarize the key notation used in this paper in Table~\ref{table:notation} for easy reference.

\begin{table}[t!]
\centering
\caption{Notation.}
\label{table:notation}
\begin{tabular}{|c|l|}\hline
$\mathcal{J}$ & The set of active jobs in the current scheduling interval \\ \hline
% $\tilde{t}_{j}$ & Completion time of job $j$ \\ \hline
$t_j^f$ &Average FP time to train a sample for job $j$ \\ \hline
$t_j^b$ &Average BP time to train a mini-batch for job $j$ \\ \hline
%$f_j(\cdot)$ & Job $j$'$s$ utility function \\ \hline
$M_j$ & Mini-batch size for job $j$ \\ \hline
$m_j$ & Gradient size at each mini-batch iteration for job $j$ \\ \hline
$\mathcal{S}$ & Set of servers in the GPU cluster\\ \hline 
$\chi_s$ & Binary variable to indicate whether server $s$ is chosen or not \\ \hline
$E_{j}$ & Number of training epochs for job $j$ \\ \hline
%$M_{i}$ & Number of mini-batches in a data chunk for job $i$ \\ \hline
$N_s$ & Capacity of GPUs resource on server $s$ \\ \hline
$\mathcal{G}_j$ &Set of GPUs requested by job $j$ \\ \hline
$G_j$ &Number of GPUs requested by job $j$ \\ \hline
$F_j$ &Number of mini-batch iterations to be trained of job $j$ \\ \hline
$\mathcal{S}_j$ &Set of servers used to place GPUs job $j$ \\ \hline
$y_{js}$ &Number of GPUs scheduled to server $s$ of job $j$ \\ \hline
$x_{js}$ &\begin{tabular}[c]{@{}l@{}}Binary variable to indicate whether job $j$ introduces external\\ communication in server $s$ \end{tabular}\\ \hline
$z_{jgs}$ & \begin{tabular}[c]{@{}l@{}} Binary variable to indicate whether server $s$ is selected\\ to schedule GPU $g$ for job $j$ or not\end{tabular}\\ \hline
$k_j$ &\begin{tabular}[c]{@{}l@{}}The maximum number of concurrent running jobs over all \\servers associated with job $j$\end{tabular} \\ \hline
$p_j$ &\begin{tabular}[c]{@{}l@{}}The maximum number of inter-connect communication jobs \\over all servers associated with job $j$\end{tabular}\\ \hline
%$\alpha$ &\begin{tabular}[c]{@{}l@{}}The coefficient to characterize the number of concurrent \\running communication tasks from number of concurrent \\inter-connect communication running jobs\end{tabular}\\ \hline
%$b_j$ &Transmission time per byte of job $j$\\\hline
%$\tau_j$ &Computation time per byte of job $j$\\\hline
%$a_j$ &\begin{tabular}[c]{@{}l@{}}The latency time caused by communication overhead \\(e.g., ACK time for message transmission) of job $j$\end{tabular}\\\hline
%$d_j$ & Constant defined as $a_j+(\tau_j-\eta_j)m_j++t_j^fM_j+t_j^b$ \\\hline
%$e_j$ &Constant defined as $(b_j+\eta_j)m_j$\\\hline
%$t_j$ &Per-worker-per-iteration time of job $j$\\\hline
%$\mu$ &Penalty coefficient for unused GPUs for the selected sever\\\hline
\end{tabular}
\vspace{-.2in}
\end{table}



==> Sec4_Model/Sec4_Model_backup2.tex <==
% !TEX root = ../ML_Networking_INFOCOM'20.tex


\section{System Model and Problem Formulation} \label{sec:model_formulation}

In this section, we first introduce our system model, then present our general problem formulation for DDL training on shared, multi-tenant GPU clusters.
\subsection{System Model}
We consider a GPU cluster consists of servers that has limited network resources and takes the communication contention into consideration for job scheduling.
% connected with a network switch of sufficiently large bandwidth.
We let $\mathcal{S}$ represent the set of servers in the GPU cluster.
Each server $s\in\mathcal{S}$ has configured with various number of GPU capacity.
Assume that GPUs are homogeneous and synchronized.
The network performance of each server is modelled by Eqn.~(\ref{contention_reduce}) and shared among different jobs.
The GPU cluster accepts DL job requests from users, and allocates GPU resource from the cluster for running the jobs.
We assume that the jobs are processed periodically and 
we use $\mathcal{J}$ to represent the set of {\em active} jobs to be trained in the current scheduling interval. 
% and let $d_j$ denote the submission time-slot for job $j\in\mathcal{J}$.
% The jobs are executed over a large time span $T$ in a time-slotted system where the scheduling time-horizon is denoted as $\mathcal{T}$. 
% The length of a time slot is potentially much larger than the duration of a training epoch, for the repeated training of the input dataset in each time slot.
% We assume the  at least one jobs is being executed at each scheduling time slot.
% There is no available information about the future upcoming jobs.
The number of GPUs of each job is requested by the user upon its submission. 
%and remains unchanged throughout the entire training process.
% We use $\mathcal{G}_j$ and $G^j$ be the set of GPUs and the number of GPUs required by job $j\in\mathcal{J}$, respectively.
% We use $G_j$ to denote the number of GPUs required by job $j\in\mathcal{J}$.
The set of GPUs can be allocated within the same server or across different servers, and will remain unchanged throughout the entire training process.
We also assume each GPU can only be occupied by one worker at any time.
% The jobs may complete at certain time slot, and we employ the dynamic scheduling.
% The job scheduling is in an online fashion, and the scheduling problem is solved at each time slot.
% Moreover, no preemption is allowed in the system, i.e., once the jobs gets started, it can not be interrupted.
% We assume that the system should be able to reassign the resources freed from the terminated jobs efficiently.
% Also, when a job runs to completion, the running jobs either can continue their training with the same number of GPUs on the same or different servers.
% Since the GPU resource is very expensive as well as avoid fragmentation, which is reserved for jobs require larger number of GPUs, the cloud is potentially assign ``just enough" servers to process the submitted jobs.

% We do not consider overall GPU resource capacity constraint in the cluster, as a cloud typically provides sufficient resources for serving a large number of customers.

% \section{Problem Formulation}

% \begin{align}
%     \text{Minimize } &c\sum_jF_jt_j\!+\!\mu\big[\sum_h(N_h\chi_h\!-\!\sum_jy_h^j)\!+\!\sum_k(N_k\chi_k\!-\!\sum_jz_k^j)\big]\\
%     \text{subject to }
%     &\sum_jy_h^j\leq N_h, \forall h\in\mathcal{H},\\
%     &\sum_jz_k^j\leq N_k, \forall k\in\mathcal{K},\\
%     &\sum_hy_h^j+\sum_kz_k^j=G_j, \forall j\in\mathcal{J},\\
%     &\sum_hy_h^j\big /\sum_kz_k^j=\gamma_j, \forall j\in\mathcal{J},\\
%     \label{eqn:k}&k=\alpha\max\{\max_h\sum_jy_h^j,\max_k\sum_jz_k^j\},\\
%     &t_j=a_j+kb_jM_j+(k-1)\eta_jM_j,\forall j\in\mathcal{J},\\
%     \label{eqn:chi_h}&\chi_h\geq \mathbbm{1}\{y_h^j\geq 1\}, \forall h\in\mathcal{H}, j\in\mathcal{J},\\
%     \label{eqn:chi_k}&\chi_k\geq \mathbbm{1}\{z_h^j\geq 1\}, \forall k\in\mathcal{K}, j\in\mathcal{J},\\
%     &\chi_h,\chi_k\in\{0,1\}, y_h^j,z_k^j\in\mathbb{Z}^+.
% \end{align}

% {\em 1)} Transformation of Eqn.~(\ref{eqn:k})

% \begin{align*}
%     k&\geq \alpha\sum_jy_h^j, \forall h\in\mathcal{H},\\
%     k&\geq \alpha\sum_jz_k^j, \forall k\in\mathcal{K}.
% \end{align*}

% {\em 2) } Transformation of Eqns.~(\ref{eqn:chi_h}) and (\ref{eqn:chi_k})

% \begin{align*}
%     y_h^j&\geq 1+ G_j(x_h^j-1), \forall h\in\mathcal{H}, j\in\mathcal{J},\\
%     z_k^j&\geq 1+ G_j(x_k^j-1), \forall k\in\mathcal{K}, j\in\mathcal{J},\\
%     x_h^j&\geq \frac{y_h^j}{G_j}, \forall h\in\mathcal{H}, j\in\mathcal{J},\\
%     x_k^j&\geq \frac{z_k^j}{G_j}, \forall k\in\mathcal{K}, j\in\mathcal{J},\\
%     \chi_h&\geq x_h^j, \forall h\in\mathcal{H}, j\in\mathcal{J},\\
%     \chi_k&\geq x_k^j, \forall k\in\mathcal{K}, j\in\mathcal{J}.
% \end{align*}



\subsection{Problem Formulation}

\begin{figure}[t]
    \centering
    \includegraphics[width=0.45\textwidth]{Figures/fig_placement.eps}
    \caption{Scenarios on different placement schemes.}\label{fig:placement}
%        \vspace{-.1in}
\end{figure}

{\bf 1) Learning Job Modeling:} 
% We use a binary variable $x_j$ to indicate whether job $j$ is executed ($x_j=1$) or not ($x_j=0$).
We use $y_{js}[t]$ to denote the number of GPUs scheduled on server $s\in\mathcal{S}$ in time slot $t$ for job $j$.
We also use $\mathcal{S}_j[t]$ to denote the set of servers that are used to place GPUs in time slot $t$ for job $j$.
We let $G_j$ be the number of GPUs requested by job $j$.
Let $k_j[t]$ be the maximum number of concurrent running communication tasks over all servers that associated with job $j$ in time slot $t$.
Here, we assume that $k_j[t]$ is proportional to the maximum number of inter-connect communication jobs over all servers.
%, which can be viewed as the expectation result.
%including sending or receiving gradients.
The intuition is that as the number for jobs increases, the number of concurrent running communication tasks should also be increased.
We use $\alpha$ to denote such linear coefficient.
In order to calculate $k_j[t]$, we need to consider following three cases:  1) When job $j$ finishes after $T_j$, then $k_j[t]=0$;
2) When all job $j$'s GPUs are placed to the same server in time slot $t$, where its workers using intra-connect communication to training the job; 3) At least two servers are scheduled to place job $j$'s servers in time slot $t$,  where its workers utilizing inter-connect communication.
Then the server that becomes the  bottleneck (i.e., has maximum number of scheduled jobs) needs to be found.
Take Fig.~\ref{fig:placement} as an example, Job 1 requires two GPU, which uses intra-connect communication ($|\mathcal{S}_1|=1$), and no resource contention is introduced.
Job 3 places each of its GPU into two servers (server 1 and 2), and it uses inter-connect communication.
However, no other inter-connect communication jobs are placed to server 1 and 2, thus no resource contention occurs.
With respect to job 2 and 4, their GPUs are placed to both server 3 and 4, and as a result,  the resource contention happens between these two jobs.
We can see from the figure that both server 3 and 4 has two different jobs (job 2 and 4), thus the bottleneck server in this case lies in both servers.


Based on the above discussion, we can compute $k_j[t]$ as follows:
\begin{align}
    \label{eqn:k_j}k_j{\color{red}[t]}=\begin{cases}
    0, \quad\text{if } t>{T}_j,\\
    0, \quad\text{if }|\mathcal{S}_j{\color{red}[t]}|=1, {\color{red}\forall t\leq T_j},\\
%    \alpha \max_{s\in\mathcal{S}_j}\sum_{j'\in\mathcal{J}}\mathbbm{1}\{y_{j's}\geq 1\},  \quad\text{if } |\mathcal{S}_j|>1.
	\alpha p_j{\color{red}[t]},  \quad\text{if } |\mathcal{S}_j{\color{red}[t]}|>1, {\color{red}\forall t\leq T_j},
    \end{cases}
\end{align}
%The first case corresponds to workers for job $j$ using internal communication since there exists some server that is scheduled to place all its GPUs.
%And the second case corresponds to workers for job $j$ using external communication since at lease two servers are arranged to host its $G_j$ workers.

% We Let $M_j$ to denote the mini-batch size for job $j$.
% Let $m^j$ denote the model size for the DNN training job $j$.
% Let $k[t]$ be the maximum number of concurrent running jobs over all the servers in time slot $t$, which can be computed as $k[t]=\max_{s\in\mathcal{S}}\{\sum_{j\in\mathcal{J}}y_s^j[t]>0\},\forall t\in\mathcal{T}$.
% We use $p_j$ to denote the computation time for each minibatch for job $j$.
where $p_j[t]\triangleq \max_{s\in\mathcal{S}_j[t]}\sum_{j'\in\mathcal{J}}\mathbbm{1}\{y_{j's}[t]\geq 1\}$, i.e., the maximum number of inter-connect communication jobs over all servers associated with job $j$ in time slot $t$.

Next we can derive the per-iteration time for job $j$ by following the performance modeling Eqn~(\ref{contention_model}).
Note that the message size  $m_j$ (i.e., the size of gradients) is related to mini-batch size and the DNN model characteristics (e.g., number of layers, number of neurons at each layer).
%Here, we assume the gradient size $m_j$ is linear proportional to mini-batch size $M_j$, i.e., $m_j=\beta_jM_j$.
And we can obtain the following per-iteration time for job $j$:
\begin{align}
	t_j[t]=\begin{cases}
	0, \quad\forall j\in\mathcal{J}, t>{T}_j,\\
	 \label{eqn:t_j}d_j+h_jk_j{\color{red}[t]}, \quad\forall j\in\mathcal{J}, {\color{red}t\leq T_j},
	\end{cases}
   \end{align}
%where $d_j\!\triangleq\! a_j+(\tau_j\beta_j+t_j^f-\eta_j\beta_j)M_j+t_j^b$ and $e_j\!\triangleq\! \beta_j(b_j+\eta_j)$.
where $d_j\triangleq a_j-\eta_jm_j+t_j^fM_j+t_j^b$ and $h_j\triangleq (e_j-\eta_j)m_j$.

% Let $\mathcal{T}_j$ be the set of time slots that job $j$ is executing.
% We use $\hat{t}_j$ to denote the completion time slot for job $j$.
% Note that if $y_s^j[t]>0$ over some server $s$ in time slot $t$, then job $j$ is being processed, thus we can use $\mathbbm{1}\{y_s^j[t]>0\}$ as the decision variable to indicate whether the job is running or not.
To ensure that there are exactly $G_j$ number of GPUs scheduled to job $j$ during its training time,
% and the allocated GPUs can be migrated throughout the entire training process,
we have:

\begin{align}
    %  \label{eqn:gpu}&\sum_{s\in\mathcal{S}}\sum_{g\in\mathcal{G}_j}y_{gs}^j[t] = G^j\cdot x_j, \quad\forall d_j \leq t\leq \hat{t}_j,j\in\mathcal{J}, \\
    \label{eqn:gpu}&\sum_{s\in\mathcal{S}}y_{js}{\color{red}[t]} = G_j, \quad \forall j\in\mathcal{J}, t\leq T_j.
    %  \label{eqn:gang}&y_{gs}^j[t]=y_{gs}^j[t+1], \quad \forall d_j\leq t<\hat{t}_j, g\in\mathcal{G}_j, s\in\mathcal{S},  j\in\mathcal{J}.
\end{align}
% We use $F_j\triangleq E_jG_jM_j$ to denote the total number of mini-batch training iterations for job $j$. 
% % which is specified by the user on submission.\footnote{In practice, to prevent spending excessively long time to wait the DNN training process to converge, a maximum number of iterations is usually set by the user.}
% In the DDL training setting, each worker (GPU) then needs to train $E^j\triangleq F^j/G_j$ if $G^j$ number of workers are scheduled for job $j$.
% Here we estimate the training iterations with the possible maximum number of GPUs can be deployed (we will show later that at least $G^j-1$ GPUs will be scheduled for each job).
% Since in practice, the model usually converges when only around 40\% of specified training iterations are conducted\cite{cite}.
% In other words, even with at most one fewer worker actually placed, the model typically can have good enough performance with the fewer number of training iterations.
% To make sure the total number of iterations trained for job $j$ over the entire training horizon does not exceed the specified number of iterations, which indicates that there is no extra utility to train more than $E^j$ iterations, we have:
% \begin{align}
%     \label{eqn:iter}&\sum_{t\in\mathcal{T}}e^j[t]\leq E^j,\quad\forall j\in\mathcal{J}.
%     % \label{eqn:iter}&\sum_{t\in\mathcal{T}}\frac{1}{t_f^jb^j\!+\!t_b^j\!+\!a^j\!+\!k[t]b^jm^j\!+\!(k[t]\!-\!1)\eta^j m^j}\!\geq\!E^jx_j,\quad\forall j\in\mathcal{J}.    
% \end{align}

%{\bf 2) Chosen Server  Modeling: }
%We use a binary variable $\chi_s$ to indicate whether server $s$ is chosen to schedule GPUs in the current interval.
%Note that as long as some GPU is placed to server $s$, then $\chi_s=1$, thus we can have the following equation:
%\begin{align}
%    &\label{eqn:chi_s}\chi_s=\mathbbm{1}\{\sum_{j\in\mathcal{J}}y_{js}\geq 1\},\quad \forall s\in\mathcal{S}.
%\end{align}

{\bf 3) Resource Constraint Modeling:} We use a binary variable $\chi_s[t]$ to indicate whether server $s$ is chosen to schedule GPUs in the current interval in time slot $t$.
We use $N_s$ to denote the maximum number of GPUs can be scheduled to server $s\in\mathcal{S}$.
To ensure that the allocated GPUs do not exceed each server's capacity, we have:
\begin{align}
    \label{eqn:cap}&\sum_{j\in\mathcal{J}}y_{js}{\color{red}[t]}\leq N_s\chi_s{\color{red}[t]}, \quad\forall s\in\mathcal{S}, t\leq T_j.
\end{align}
We can know from the above equation that if server $s$ is not chosen to do the scheduling in time slot $t$ ($\chi_s[t]=0$), then no GPUs could be placed on the server. 


 {\bf 4) Completion Time Modeling:} We use $T_j$ to denote the completion time slot for job $j$.
 In each time slot $t$, the number of mini-batch iterations can be completed is $\frac{t'}{t_j[t]}$, where $t'$ is the time duration for each time slot $t$ (e.g., 10 minutes).
The smallest time slot that finishes at lest $F_j$ iterations is the completion time for job $j$, we have:
\begin{align}
%\sum_{t\in\mathcal{T}_j}\frac{t'}{t_j[t]}=F_j, \quad \forall j\in\mathcal{J}.
T_j=\arg\min_t \{\sum_{t\in\mathcal{T}}\frac{t'}{t_j[t]}\geq F_j\}, \quad \forall j\in\mathcal{J}.
\end{align}

Next, to ensure the jobs will not be interrupted and the placement scheme remains unchanged during its training process, we have

\begin{align}
y_{js}[t]=\begin{cases}
0, \quad\forall i\in\mathcal{S},j\in\mathcal{J},t>T_j,\\
y_{js}[t-1],  \quad\forall i\in\mathcal{S},j\in\mathcal{J},t\leq T_j.
\end{cases}
\end{align}


Finally, to define the decision variables domain, we have:

\begin{align}
    \label{eqn:int}&y_{js}[t] \in\mathbb{Z}^+, \chi_s[t]\in\{0,1\},
    \forall s\in\mathcal{S}, j\in\mathcal{J},t\in\mathcal{T}.
\end{align}

%{\color{red}
%\begin{align}
%y_{js}[t]=y_{js}[t-1], \forall t\leq T_j, y_{js}[t]=0, \forall t > T_j, s\in\mathcal{S}, j\in\mathcal{J}.
%\end{align}
%}

% Note that for job $j$, its completion time $\hat{t}_j$ corresponds to the latest time-slot where there remain some active workers allocated for it.
% Therefore, we have:
% \begin{align}
%     \label{eqn:t}&\hat{t}_j = \arg\max_{t\in\mathcal{T}}\{\sum_{s\in\mathcal{S}}\sum_{g\in\mathcal{G}_j}y_{gs}^j[t]>0\},\quad\forall j\in\mathcal{J}.
% \end{align}

% Lastly, to ensure that there is no workers allocated before $j$'s arrival, we have:
% \begin{align}
%   \label{eqn:pri_arr}&y_{s}^j[t]=0,\quad\forall t<d_j, s\in\mathcal{S},j\in\mathcal{J}.
%   \label{eqn:pri_arr}&y_{s}^j[t]\in \mathbb{Z}^+,\quad\forall t\in\mathcal{T}, s\in\mathcal{S},j\in\mathcal{J}.
%   &y_{s}^j[t]\in \mathbb{Z}^+\text{ and }  \label{eqn:pri_arr}y_{s}^j[t]\leq G^j ,\quad\forall t\in\mathcal{T}, s\in\mathcal{S},j\in\mathcal{J}.
% \end{align}



%To obtain the time completion time for job $j$, we check the largest time slot that $\sum_{s\in\mathcal{S}}y_{js}[t]>0$, i.e.,
%\begin{align}
%T_j=\arg\max_t\{\sum_{s\in\mathcal{S}}y_{js}[t]>0\}, \quad\forall j\in\mathcal{J}.
%\end{align}

%Also, to ensure the job is not preempted once get started, we have:
%\begin{align}
%t_j[t]>0,
%\end{align}



{\bf 3) Objective Function and Problem Statement: } 
% We use the function  $f_j(\sum_{t\in\mathcal{T}}e^j[t])$ to denote the concave utility function for job $j$, which can deliver the results with respect to partial training iterations $\sum_{t\in\mathcal{T}}e^j[t]$.
In this paper, our goal is to minimize the overall operations cost, including the execution cost and the fragmentation cost, for all jobs from the system's perspective.
% We let $c_1$ be the time unit price paid by users, and let $c_2$ be the time unit operations cost.
We let $c$ be the time unit execution cost for running the GPUs in the cluster.
Let $E_j$ be the number of epochs to be trained for job $j$, and then  $F_j=E_jG_jM_j$ is the number of mini-batch iterations to be trained for job $j$.
The term ${\color{red}c\sum_{j\in\mathcal{J}}T_j}$ corresponds to the overall execution cost associated with each job, which is proportional to the training time.
% Thus $c\sum_{j\in\mathcal{J}}F_jt_j$ will be the total benefit by running GPUs, where $c\triangleq c_1-c_2$.
Also the term ${\color{red}\mu\sum_{t\in\mathcal{T}}\sum_{s\in\mathcal{S}}(N_s\chi_s[t]-\sum_{j\in\mathcal{J}}y_{js}[t])}$ is the fragmentation cost, which is measured by the difference between the number of allocated GPUs and the number of available GPUs from each selected server $s$, and $\mu$ is a penalty coefficient for unused GPUs.
On one hand, the system tends to avoid the resource contention to minimize the overall execution cost, i.e., spreading jobs over all servers.
On the other hand, the system also tends to pack jobs into servers to reduce the fragmentation cost.
Hence, to minimize the operations cost of the objective function, the system tends to find a balance between spread jobs over servers and exploit all available GPU resources for each selected server.
% In other words, the system tries to avoid too much server fragmentation, which can save internal communication for coming jobs that require larger number of GPUs.
Putting all constraints and the objective function together, the offline distributed DDL job scheduling problem~DDLJS can be formulated as:
\begin{align*}
{\bf DDLJS: } \underset{\mathbf{y,\chi}}{\text{ Minimize }} &c\sum_{j\in\mathcal{J}}T_j+\mu\sum_{t\in\mathcal{T}}\sum_{s\in\mathcal{S}}(N_s\chi_s[t]-\sum_{j\in\mathcal{J}}y_{js}[t])\\
    \text{subject to } 
    &\text{Constraints}  (\ref{eqn:k_j})-(\ref{eqn:int}).  
\end{align*}
It can be seen that Problem~DDLJS is a mixed integer nonlinear program (MINLP), which is NP-hard in general.
It involves both non-deterministic and indicator function in constraint~(\ref{eqn:k_j}), which are not amenable for conventional optimization techniques.
Overcoming these challenges constitutes the main subjects in the next section.
To conclude this section, we summarize the key notation used in this paper in Table~\ref{table:notation} for easy reference

\begin{table}[t!]
\centering
\caption{Notation.}
\label{table:notation}
\begin{tabular}{|c|l|}\hline
$\mathcal{J}$ & The set of active jobs in the current scheduling interval \\ \hline
% $\tilde{t}_{j}$ & Completion time for job $j$ \\ \hline
$t_j^f$ &Average FP time to train a sample for job $j$ \\ \hline
$t_j^b$ &Average BP time to train a mini-batch for job $j$ \\ \hline
%$f_j(\cdot)$ & Job $j$'$s$ utility function \\ \hline
$M_j$ & Mini-batch size for job $j$ \\ \hline
$m_j$ & Gradient size at each mini-batch iteration for job $j$ \\ \hline
$\mathcal{S}$ & Set of servers in the GPU cluster\\ \hline 
$\chi_s$ & Binary variable to indicate whether server $s$ is chosen or not \\ \hline
$E_{j}$ & Number of training epochs for job $j$ \\ \hline
%$M_{i}$ & Number of mini-batches in a data chunk for job $i$ \\ \hline
$N_s$ & Capacity of GPUs resource on server $s$ \\ \hline
$\mathcal{G}_j$ &Set of GPUs requested by job $j$ \\ \hline
$G_j$ &Number of GPUs requested by job $j$ \\ \hline
$F_j$ &Number of mini-batch iterations to be trained for job $j$ \\ \hline
$\mathcal{S}_j$ &Set of servers used to place GPUs job $j$ \\ \hline
$y_{js}$ &Number of GPUs scheduled to server $s$ for job $j$ \\ \hline
$x_{js}$ &\begin{tabular}[c]{@{}l@{}}Binary variable to indicate whether job $j$ introduces external\\ communication in server $s$ \end{tabular}\\ \hline
$z_{jgs}$ & \begin{tabular}[c]{@{}l@{}} Binary variable to indicate whether server $s$ is selected\\ to schedule GPU $g$ for job $j$ or not\end{tabular}\\ \hline
$k_j$ &\begin{tabular}[c]{@{}l@{}}The maximum number of concurrent running jobs over all \\servers associated with job $j$\end{tabular} \\ \hline
$p_j$ &\begin{tabular}[c]{@{}l@{}}The maximum number of inter-connect communication jobs \\over all servers associated with job $j$\end{tabular}\\ \hline
%$\alpha$ &\begin{tabular}[c]{@{}l@{}}The coefficient to characterize the number of concurrent \\running communication tasks from number of concurrent \\inter-connect communication running jobs\end{tabular}\\ \hline
%$b_j$ &Transmission time per byte for job $j$\\\hline
%$\tau_j$ &Computation time per byte for job $j$\\\hline
%$a_j$ &\begin{tabular}[c]{@{}l@{}}The latency time caused by communication overhead \\(e.g., ACK time for message transmission) for job $j$\end{tabular}\\\hline
%$d_j$ & Constant defined as $a_j+(\tau_j-\eta_j)m_j++t_j^fM_j+t_j^b$ \\\hline
%$e_j$ &Constant defined as $(b_j+\eta_j)m_j$\\\hline
%$t_j$ &Per-worker-per-iteration time for job $j$\\\hline
%$\mu$ &Penalty coefficient for unused GPUs for the selected sever\\\hline
\end{tabular}
\vspace{-.2in}
\end{table}

\section{Initial Approach}
Without loss of generality, we assume $T_1\leq T_2\hdots \leq T_j \leq\hdots\leq T_J$.

\begin{align*}
T_1&=F_1t_1^{(1)}\\
T_2&=T_1+\big(F_2-\frac{T_1}{t_2^{(1)}}\big)t_2^{(2)}=F_1t_1^{(1)}\big(1-\frac{t_2^{(2)}}{t_2^{(1)}}\big)+F_2t_2^{(2)}\\
T_3&=T_2+\big(F_3-\frac{T_1}{t_3^{(1)}}-\frac{T_2-T_1}{t_3^{(2)}}\big)t_3^{(3)}\\
%&=F_1t_1^{(1)}\bigg((1-\frac{t_3^{(3)}}{t_3^{(2)}})(1-\frac{t_2^{(2)}}{t_2^{(1)}})-\frac{t_3^{(3)}}{t_3^{(1)}}\bigg)\\
%&+F_2t_2^{(2)}(1-\frac{t_3^{(3)}}{t_3^{(2)}})+F_3t_3^{(3)}\\
&\hdots\\
T_j&=T_{j-1}+\big(F_j-\frac{T_1}{t_j^{(1)}}-\frac{T_2-T_1}{t_j^{(2)}}-\hdots-\frac{T_{j-1}-T_{j-2}}{t_j^{(j-1)}}\big)t_j^{(j)}\\
&\hdots\\
T_J&=T_{J-1}+\big(F_J-\frac{T_1}{t_J^{(1)}}-\frac{T_2-T_1}{t_J^{(2)}}-\hdots-\frac{T_{J-1}-T_{J-2}}{t_j^{(J-1)}}\big)t_J^{(J)}
\end{align*}

\begin{align*}
&\sum_{t\in\mathcal{T}}\sum_{j\in\mathcal{J}[t]}(t-\frac{t}{\tau_j[t]}\tau_j^0)\\
&=J*(T_1-\frac{T_1}{\tau_1[t]}\tau_1^0)+(J-1)*(T_2-T_1-\frac{T_2-T_1}{\tau_2[t]}\tau_2^0)\\
&+\hdots+(J-j+1)(T_j-T_{j-1}-\frac{T_j-T_{j-1}}{\tau_j[t]}\tau_j^0)\\
&+\hdots+(T_J-T_{J-1}-\frac{T_{J}-T_{J-1}}{\tau_J[t]}\tau_J^0)\\
&\leq r*\sum_{k=0}^{J-1}(J-k)(T_{k+1}-T_k)
\end{align*}
where $r=max_{k,t}(1-\frac{\tau_k^0}{\tau_k[t]})$ and $T_0=0$.

\begin{align*}
&\sum_{s\in\mathcal{S}}y_{js}=G_j, \quad \forall j\in\mathcal{J}[t],\\
&\sum_{j\in\mathcal{J}[t]}y_{js}\leq N_s, \quad\forall s\in\mathcal{S}.
\end{align*}




==> Sec5_Algorithm/Sec5_Algorithm_backup.tex <==
% !TEX root = ../ML_Networking_INFOCOM'20.tex

\section{Solution Approach and Problem Reformulation} \label{sec:alg}
In this section, we describe the key components of our scheduling algorithm design for solving Problem~DDLJS, which is structured into tree steps from Sections...
We present the theoretical performance results in Section...

% \subsection{Handling Non-Deterministic Eqn.~(\ref{eqn:k_j})}
\subsection{Challenges in Solving Problem~DDLJS}
The first obstacle to solve Problem~DDLJS stems from the non-deterministic structure in constraint~(\ref{eqn:k_j}).
We let 
\begin{align}
\label{eqn:xjs2}x_{js}\!=\!\begin{cases}
\mathbbm{1}\{1\leq y_{js}\leq G_{j}-1\}, \forall s\!\in\!\mathcal{S}, j\!\in\!\mathcal{J}, &\hspace{-0.1in}\text{if }G_j\!>\!1,\\
0,&\hspace{-0.1in}\text{if }G_j\!=\!1.
\end{cases}
\end{align}
%$x_{js}\triangleq\mathbbm{1}\{1\leq y_{js}\leq G_{j}-1\}, \forall s\in\mathcal{S}, j\in\mathcal{J}$.
We observe that $k_j=0$ only if $y_{js}=G_j,\exists s\in\mathcal{S}$, which corresponds to intra-connect communication jobs (single-GPU job is the special case).
The maximum number of inter-connect communication jobs over all servers $p_j$ can be computed as $\max_{s\in\mathcal{S}}\sum_{j'\in\mathcal{J}} x_{j's}$. 
Notice that $x_{js}$ will be increased by one only if $y_{js}\in[1,G_{j}-1],\forall s\in\mathcal{S}, j\in\mathcal{J}$ and $G_j\neq 1$.
With the linear proportional assumption, we can have the following equivalent formulation for constraint~(\ref{eqn:k_j}):
\begin{align*}
    k_j=\begin{cases}
    0, \quad \text{if } y_{js}=G_j, \exists s\in\mathcal{S},\\
    \alpha \max_{s\in\mathcal{S}}\sum_{j'\in\mathcal{J}}x_{j's}, \quad \text{o.w.}
    \end{cases}
\end{align*}
We can see that $k_j=0$ implies $x_{js}=0$ since $y_{js}=G_j, \exists s\in\mathcal{S}$. 
%and for the special case when $G_j=1$, $x_{js}=0$ still holds.
Since $x_{js}\geq 0$ and $\alpha\in(0,1)$, we can further simplify $k_j$ as follows:
\begin{align*}
    k_j=\alpha\max_{s\in\mathcal{S}}\sum_{j'\in\mathcal{J}}x_{j's}.
\end{align*}
% We can see from the above equation that $k_j$ with initial value $0$ will only be increased by one when some server $s$ is scheduled to place GPUs from job $j$ but it does not contain all its GPUs.
We can see from the above equation that $k_j$ involves the "max`` structure, which can be removed  by the following equivalent transformation:
\begin{align}
    \label{eqn:k_j_reformulate}&k_j\geq \alpha\sum_{j'\in\mathcal{J}}x_{j's}, \quad \forall s\in\mathcal{S}, j\in\mathcal{J}.
    % &k_j\geq 0,\quad \forall j\in\mathcal{J}\nonumber.
\end{align}

% \subsection{Handling Indicator Functions in Eqns.~(\ref{eqn:k_j})(\ref{eqn:chi_s})}
After solving the non-deterministic structure in Eqn.~(\ref{eqn:k_j}), it still remains difficult to directly solve Problem~DDLJS due to the indicator functions in Eqns.~(\ref{eqn:k_j})(\ref{eqn:chi_s}).
In the literature, a commonly used technique is to use big-$M$ to reformulate indicator function to a series of linear constraints, and solve it using LP solver.
However, it is well-known that indicator constraints present the drawback of having a weak continuous relaxation, and might lead to numerical issues \cite{Belotti16:indicatorfunction}.
In order to circumvent the limitations, we observe that the original problem~(\ref{Problem:primal}) can be converted into the following equivalent formulation, where we interpret it from the perspective of GPU instead of job placement.

\subsection{Problem Reformulation}
We use $\mathcal{G}_j$ to denote the set of GPUs that required by user $j$.
Recall that $|\mathcal{G}_j|=G_j$.
We let $z_{jgs}, \forall g\in\mathcal{G}_j,s\in\mathcal{S}, j\in\mathcal{J}$ encode the placement scheme of job $j$, where $z_{jgs}=1$ if server $s$ is selected to host GPU $g$ of job $j$; otherwise it is $0$.
We first simply the objective function as follows:
%We further can simply the objective function as follows:
\begin{align*}
&c\sum_{j\in\mathcal{J}}F_jt_j+\mu\sum_{s\in\mathcal{S}}(N_s\chi_s-\sum_{j\in\mathcal{J}}\sum_{g\in\mathcal{G}_j}z_{jgs})\\
&=c\sum_{j\in\mathcal{J}}F_j(d_j+h_jk_j)+\mu\sum_{s\in\mathcal{S}}N_s\chi_s-\mu\sum_{s\in\mathcal{S}}\sum_{j\in\mathcal{J}}\sum_{g\in\mathcal{G}_j}z_{jgs}\\
&=c\sum_{j\in\mathcal{J}}F_jd_j+c\sum_{j\in\mathcal{J}}F_jh_jk_j-\mu\sum_{j\in\mathcal{J}}G_j+\mu\sum_{s\in\mathcal{S}}N_s\chi_s
\end{align*}

We use $\gamma_{js}$ to denote whether any GPU of job $j$ is allocated to server $s$ ($\gamma_{js}=1$) or not ($\gamma_{js}=0$).
Then our original problem can be reformulated as the following equivalent problem:
\begin{align}
   \underset{\mathbf{z,x,k,\chi}} {\text{Minimize }} &c\sum_{j\in\mathcal{J}}F_jh_jk_j+\mu\sum_{s\in\mathcal{S}}N_s\chi_s\label{Problem:primal}\\
    \text{subject to }
    &\sum_{s\in\mathcal{S}}z_{jgs}=1, \quad\forall j\in\mathcal{J}, g\in\mathcal{G}_j,\label{eqn:gpu2}\\
    &\sum_{j\in\mathcal{J}}\sum_{g\in\mathcal{G}_j}z_{jgs}\leq N_s,\quad\forall s\in\mathcal{S},\label{eqn:cap2}\\
%    &\chi_{s}\geq z_{jgs}, \quad\forall j\in\mathcal{J}, g\in\mathcal{G}_j, s\in\mathcal{S},\label{eqn:chi_s2}\\    
    &\gamma_{js}\geq z_{jgs}, \quad \forall  j\in\mathcal{J}, g\in\mathcal{G}_j, s\in\mathcal{S},\label{eqn:gamma}\\
    &\chi_{s}\geq \gamma_{js}, \quad\forall j\in\mathcal{J}, s\in\mathcal{S},\label{eqn:chi_s2}\\
    &x_{js}\geq \gamma_{js}-z_{jgs}, \quad \forall j\in\mathcal{J}, g \in\mathcal{G}_j, s\in\mathcal{S},\label{eqn:xjs}\\
%    &x_{js}\geq z_{jgs}\!-\!z_{jg's}, \forall j\in\mathcal{J}, g,g'\!\in\!\mathcal{G}_j, s\!\in\!\mathcal{S},\label{eqn:xjs}\\
    &z_{jgs}, x_{js},\chi_s,\gamma_{js}\in\{0,1\}, k_j\geq 0,\nonumber\\
    &\hspace{1.2in}\forall j\in\mathcal{J}, g\in\mathcal{G}_j, s\in\mathcal{S},\label{eqn:int2}\\
    &\text{Constraint}~(\ref{eqn:k_j_reformulate})\nonumber.
\end{align}

Note that in the objective, we further omit the constants terms, which does not affect the optimal solutions derived by solving the above problem.
Constraint~(\ref{eqn:gpu2}) ensures that each job's GPU is placed to exactly one server, which guarantees exactly $G_j$ workers will be scheduled to job $j$.
Constraint~(\ref{eqn:cap2}) ensures that the total number of GPUs scheduled over all jobs to server $s$ should not exceed its capacity.
Constraint~(\ref{eqn:gamma}) indicates whether any GPU of job $j$ is placed to server $s$.
Constraint~(\ref{eqn:chi_s2}) indicates the server $s$ is chosen (i.e., $\chi_s=1$) as long as some job places its GPU to it, implying $\sum_{j\in\mathcal{J}}y_{js}\geq 1$.
Constraint~(\ref{eqn:xjs}) is equivalent to Eqn.~(\ref{eqn:xjs2}) (refer to Lemma~\ref{lem:equivalence}).


\begin{lem}\label{lem:equivalence}
Problem~DDLJS and Problem~(\ref{Problem:primal}) are equivalent, i.e., a feasible solution to the former has a corresponding same feasible solution to the latter, and vice verse.
\end{lem}
\begin{proof}
First, it is obvious that Constraints~(\ref{eqn:gpu2}) and (\ref{eqn:cap2}) are equivalent to Constraints~(\ref{eqn:gpu}) and (\ref{eqn:cap}), respectively.

Next, we show the equivalence between Constraints~(\ref{eqn:gamma})(\ref{eqn:chi_s2}) and (\ref{eqn:chi_s}). 
We can know that $\chi_s\geq \gamma_{js}\geq z_{jgs}$, thus we only need to show it is equivalent to Eqn.~(\ref{eqn:chi_s}). 
On one hand, we know that as long as there exists some job $j$ that places its GPU to the server $s$, i.e., $z_{jgs}=1$, then $\sum_jy_{js}\geq 1$ since $y_{js}\geq1$.
On the other hand, from Constraint~(\ref{eqn:chi_s}), we know that as long as server $s$ is chosen to schedule GPUs,
i.e., $\sum_jy_{js}\geq 1$, then there must exist some job $j$ that schedules its GPU $g$ to the server $s$, implying $z_{jgs}=1$.
Thus, the equivalence between these two constraints are proved.

Lastly, we show that Constraint~(\ref{eqn:xjs}) is the same as Eqn.~(\ref{eqn:xjs2}).
We consider the following three cases for job $j$:

%{\em 1) }The job only requires one GPU (i.e., $G_j=1$), then $z_{jg's}=z_{jgs}$, which implies that $x_{js}\geq 0$ based on Constraint~(\ref{eqn:xjs}), meaning $x_{js}$ can be $0$ or $1$.
%However, In order to minimize the objective value, the system tends to minimize $k_j$ that decreases as $x_{js}$ decreases, and as a result, $x_{js}$ will be set to $0$.
%% which comply with $\mathbbm{1}\{1\leq y_{js}\leq G_j-1\}$.
%
%{\em 2) }There exists some server $s$ that host all its workers (i.e., $y_{js}=G_j$ and $G_j>1$), then $z_{jgs}=1, \forall g\in\mathcal{G}_j$, which implies that $x_{js}\geq 0$. 
%%based on Constraint~(\ref{eqn:xjs}), meaning $x_{js}$ can be $0$ or $1$.
%And with the same reason in case {\em 1)}, $x_{js}$ will be set to $0$.
%
%{\em 3) }There exists at lease two servers to host its workers (i.e., $1\leq y_{js}\leq G_j-1, \forall s\in\mathcal{S}_j$ and $G_j>1$), then $z_{jgs}-z_{jg's}=1, \exists g,g'\in\mathcal{G}_j, s\in\mathcal{S}_j$, implying $x_{js}\geq 1$, and as a result, $x_{js}$ will be set to $1$.

{\em 1) }The job only requires one GPU (i.e., $G_j=1$), then $\gamma_{js}=1$ and $\gamma_{js}-z_{jgs}=0$, which implies that $x_{js}\geq 0$ based on Constraint~(\ref{eqn:xjs}), meaning $x_{js}$ can be $0$ or $1$.
However, In order to minimize the objective value, the system tends to minimize $k_j$ that decreases as $x_{js}$ decreases, and as a result, $x_{js}$ will be set to $0$.
% which comply with $\mathbbm{1}\{1\leq y_{js}\leq G_j-1\}$.

{\em 2) }There exists some server $s$ that host all its workers (i.e., $y_{js}=G_j$ and $G_j>1$), then $z_{jgs}=1, \forall g\in\mathcal{G}_j$, which implies that $x_{js}\geq 0$. 
%based on Constraint~(\ref{eqn:xjs}), meaning $x_{js}$ can be $0$ or $1$.
And with the same reason in case {\em 1)}, $x_{js}$ will be set to $0$.

{\em 3) }There exists at lease two servers to host its workers (i.e., $1\leq y_{js}\leq G_j-1, \forall s\in\mathcal{S}_j$ and $G_j>1$), then $\gamma_{js}-z_{jgs}=1, \exists g\in\mathcal{G}_j, s\in\mathcal{S}_j$, implying $x_{js}\geq 1$, and as a result, $x_{js}$ will be set to $1$.


We can see from all the cases above that $x_{js}$ in Constraint~(\ref{eqn:xjs}) is $1$ if and only if $x_{js}$ in Eqn.~(\ref{eqn:xjs2}) is $1$, and vice verse, and the proof is complete.
\end{proof}
% Several remarks for Lemma~\ref{lem:equivalence} are in order:
Notice that the first two cases correspond to jobs that use intra-connect communication, which will not introduce resource contention between servers; while the last case involves inter-connect communication, which needs to be counted to the concurrent number of communication tasks.







% Recall that $x_{j's}$ is $0$ only when $y_{j's}=0$ or $y_{j's}=G_{j'}$; otherwise it is $1$.
% We let $l_{js}\triangleq\{y_{js}\geq 1\}$, and let $u_{js}\triangleq\{y_{js}\leq G_j-1\}$.
% We first convert the indicator function as follows:
% \begin{align}
%     &y_{js}\geq 1+G_j(l_{js}-1), \forall s\in\mathcal{S}, j\in\mathcal{J},\label{eqn:y1}\\
%     &y_{js}\leq G_j-1+G_j(1-u_{js}),\forall s\in\mathcal{S}, j\in\mathcal{J},\label{eqn:y2}\\
%     &x_{js}\leq l_{js},\forall s\in\mathcal{S}, j\in\mathcal{J},\label{eqn:x1}\\
%     &x_{js}\leq u_{js}, \forall s\in\mathcal{S}, j\in\mathcal{J}\label{eqn:x2},\\
%     &l_{js},u_{js}, x_{js}\in\{0,1\},\forall s\in\mathcal{S}, j\in\mathcal{J}\label{eqn:lux}.
% \end{align}
% From Eqn.~(\ref{eqn:y1}), we have $l_{js}=0$ when $z_{js}=0$; similarly, from Eqn.~(\ref{eqn:y2}), we have $u_{js}=0$ when $z'_{js}=G_j$.
% And Eqns.~(\ref{eqn:x1})(\ref{eqn:x2}) imply that $x_{js}=\min\{l_{js},u_{js}\}$.
% In other words, $x_{js}=0$ only if both $l_{js}=0$ (corresponds to the case that no job $j$'s GPUs are placed to the server $s$) and $u_{js}=0$ (corresponds to the case that all job $j$'s GPUs are placed to the server $s$), which comply with the calculation of $k_j$ since no resource contention is introduced under these two cases.
% Notice that single-GPU jobs will never compete for the bandwidth with other jobs, meaning $x_{js}$ should be $0$ for the server $s$ where its GPU is scheduled.
% Under this case, $x_{js}=\mathbbm{1}\{1\leq y_{js}\leq 0\}$, which is impossible to be satisfied, implying $x_{js}=0$.
% Thus, it is still valid even with special case that jobs only require one GPU.
% % In addition, we can infer from Eqns.~(\ref{eqn:x1}) and (\ref{eqn:x2}) that

% % \begin{align}
% %     &k_j\leq \alpha\sum_{j'\in\mathcal{J}}l_{j's},\forall j\in\mathcal{J},\label{eqn:k_j_up1}\\
% %     &k_j\leq \alpha\sum_{j'\in\mathcal{J}}u_{j's},\forall j\in\mathcal{J}\label{eqn:k_j_up2},
% % \end{align}
% % which we obtain the upper bound of $k_j$, and as a result, the objective value will still be bounded.

% We notice that  $\sum_{j\in\mathcal{J}}y_{js}\geq 1$ as long as the server $s$ is chosen by some job $j$, which is associated with $x_{js}$.
% However, $x_{js}=0$ when $y_{js}=G_j$, which shows that we need to have this special case included.
% Here, we introduce the equation $z_{js}=\mathbbm{1}\{y_{js}\geq G_j\}$ to include the border case, where $y_{js}=G_j$, then $z_{js}=1$.
% Analogously, 
% % we let $z_{js}=\mathbbm{1}\{y_{js}\geq 1\}, \forall s\in\mathcal{S}, j\in\mathcal{J}$.
% % , and let $G\triangleq\max_{j\in\mathcal{J}}G_j$.
% we can transform the indicator function in Eqn.~(\ref{eqn:chi_s}) to a set of following linear equations:
% \begin{align}
%     &y_{js}\geq G_j+G_j(z_{js}-1), \forall s\in\mathcal{S},\label{eqn:sum_y}\\
%   &\chi_s\geq z_{js}, \forall s\in\mathcal{S},j\in\mathcal{J}, \label{eqn:chi_s_2}\\
%     &\chi_s\geq x_{js}, \forall s\in\mathcal{S},j\in\mathcal{J},\label{eqn:chi_s_3}\\
%     &\chi_s, z_{js}\in\{0,1\}, \forall s\in\mathcal{S},j\in\mathcal{J} \label{eqn:zs}.
% \end{align}
% % \begin{align}
% %     \label{eqn:sum_y}&\sum_{j\in\mathcal{J}}y_{js}\geq 1+G(z_s-1), \forall s\in\mathcal{S},\\
% %     \label{eqn:chi_s_2}&\chi_s=z_s, \forall s\in\mathcal{S},\\
% %     &z_s\in\{0,1\}, \forall s\in\mathcal{S}, \label{eqn:zs}.
% % \end{align}

% Combine Eqns.~(\ref{eqn:sum_y})-(\ref{eqn:chi_s_3}), we can have that $\chi_s=1$ when $1\leq y_{js}\leq G_j, \forall s\in\mathcal{S}, \exists j\in\mathcal{J}$.
% However, it is not guaranteed from Eqns.~(\ref{eqn:y1})(\ref{eqn:y2}) that $l_{js}=1$ when $y_{js}=0$, and $u_{js}=1$ when $y_{js}\leq G_j-1$ since they are still valid with $l_{js}=0$ and $u_{js}=0$.
% % Also from Eqn.~(\ref{eqn:sum_y}), $z_s$ is not guaranteed to have value $1$ when $\sum_{j\in\mathcal{J}}y_{js}\geq 1$.
% Thus, we add a dummy term $-\frac{\mu}{J}\sum_{j\in\mathcal{J}}\sum_{s\in\mathcal{S}}x_{js}$ to the objective function, which will enforce the system to set $l_{js}$ and  $u_{js}$ to $1$ due to the minimization objective function.
% Also, $z_{js}$ can be either $0$ or $1$ when $y_{js}= G_j$.
% Similarly, we add another dummy term $-\frac{\mu}{J}\sum_{j\in\mathcal{J}}\sum_{s\in\mathcal{S}}z_{js}$ to force the system to set $z_{js}$ to $1$ when $y_{js}=G_j$ since it can reduce the objective value.

% \subsection{Problem Reformulation}
% After we handle with the non-amenable constraints


\section{An Offline Fractional Algorithm}\label{sec:frac}
\begin{figure}[t]
    \centering
    \includegraphics[width=0.45\textwidth]{Figures/fig_relaxation.eps}
    \caption{Example of too loose relaxation bound.}\label{fig:relaxation}
%        \vspace{-.1in}
\end{figure}

It is clearly that Problem~(\ref{Problem:primal}) is a Mixed integer linear program (MILP), which is NP-hard in general.
We first relax the integer constraints to continuous values to obtain the fractional solution, which serves as a lower bound to the discrete solution.
However, when we relax the binary variables to continuous values between 0 and 1, the system tend to assign same fractional value for all GPUs to make $x_{js}$ to 0, which also could make $\chi_s$ small, even they distribute across servers and may introduce resource contention.
In other words, Eqns.~(\ref{eqn:gamma})-(\ref{eqn:xjs}) are too loose to capture the inter-connect communication case, and thus lead to very small $k_j$ and $\chi_s$.
And as a result, the gap between the fractional solution and integer solution can be large.

Consider one scenario as indicated in Fig.~\ref{fig:relaxation} to show that the relaxed linear program solution can be a very loose bound.
In order to distinguish jobs' GPUs, we index them as  1 and 2.
%If only integer number of workers are allowed to be scheduled to each server, one placement scheme is shown in Fig.~\ref{fig:placement}(a), where both jobs use the external communication to perform the training.
Suppose the integer placement scheme is shown as in Fig.~\ref{fig:relaxation}(a), i.e., server 1 and 2 host one GPU from both jobs.
Then $x_{js}=1, j=1,2, s=1,2$, and  $k_1=k_2=2\alpha$.
However, if we relax the integer constraints and the fractional number of workers is allowed to be scheduled to each server, one placement scheme is shown in Fig.~\ref{fig:relaxation}(b).
We can see from the figure that each worker of the job is split into halves and is placed to server 1 and 2 (i.e., $z_{jgs}=0.5, j=1,2, g=1,2, s=1,2$).
According to Eqn.~(\ref{eqn:xjs}), $x_{js}=0, j=1,2, s=1,2$ and $k_1=k_2=0$, which is equivalent to the intra-connect communication case.
However, if we do not distinguish between GPUs of each job and merge two half GPUs of the same job in the same server into one complete GPU, the fractional placement scheme actually corresponds to the inter-connect communication case, and is equivalent to the integer placement scheme.
%In other words, $x_{11}$, $x_{12}$, $x_{23}$ and $x_{24}$ should not be $0$.
Therefore, the fractional solution is a very loose bound to its corresponding integer solution.



\subsection{Improvement of Relaxation Bound}
In order to strengthen the relaxation, we add the following constraints to Problem~(\ref{Problem:primal}):

\begin{align}
%    &\sum_{s'\in\mathcal{S}\setminus\{s\}}z_{jgs'}\geq 1-z_{jgs}, \quad\forall j\in\mathcal{J}, g\in\mathcal{G}_j,s \in\mathcal{S},\label{eqn:add1}\\
    &\sum_{g\in\mathcal{G}_j}z_{jgs}\geq G_j(1-x'_{js}),  \quad\forall j\in\mathcal{J}, s \in\mathcal{S},\label{eqn:add2}\\
%    &x_{js}\geq z_{jgs}\cdot x'_{js},  \quad\forall j\in\mathcal{J}, g\in\mathcal{G}_j,s \in\mathcal{S},\label{eqn:add3}\\
%    &x_{js}\geq (1-\frac{\sum_{g\in\mathcal{G}_j}z_{jgs}}{G_j})z_{jgs}, \quad\forall j\in\mathcal{J}, g\in\mathcal{G}_j,s \in\mathcal{S}\label{eqn:add2},\\
%    &x_{js}\geq (1-\sum_{s'\in\mathcal{S}\setminus\{s\}}z_{jgs'}) x'_{js}, \forall j\in\mathcal{J}, g\in\mathcal{G}_j,s \in\mathcal{S},\label{eqn:add4}\\
%    &\chi_s\geq \sum_{s'\in\mathcal{S}\setminus\{s\}}z_{jgs'}, \quad\forall j\in\mathcal{J}, g\in\mathcal{G}_j,s \in\mathcal{S},\label{eqn:add5}\\
    &\chi_s\geq 1-\sum_{s'\in\mathcal{S}\setminus\{s\}}z_{jgs'}, \quad\forall j\in\mathcal{J}, g\in\mathcal{G}_j,s \in\mathcal{S},\label{eqn:add5}\\
% &\chi_s\geq 1-\gamma_{js}, \quad\forall j\in\mathcal{J}, s \in\mathcal{S},\label{eqn:add5}\\
    &x_{js}\geq \chi_sx'_{js},\quad\forall j\in\mathcal{J}, s \in\mathcal{S},\label{eqn:add6}\\
%    &x_{js}\geq \chi_sx'_{js},\quad\forall j\in\mathcal{J}, s \in\mathcal{S},\label{eqn:add6}\\
    &x'_{js}\in\{0,1\}, \quad\forall j\in\mathcal{J}, s \in\mathcal{S}\label{eqn:add7}.
\end{align}
%where $H_j=\min\{N_s,G_j\}$.
%Recall that $\sum_{g\in\mathcal{G}_j}z_{jgs}\leq H_j$.
 From Constraint~(\ref{eqn:gpu2}), we know that $\sum_{s'\in\mathcal{S}\setminus\{s\}}z_{jgs'}=0$ implies  $z_{jgs}=1$ (i.e., server $s$ is selected to host job $j$'s GPU $g$), and $\sum_{s'\in\mathcal{S}\setminus\{s\}}z_{jgs'}=1$ implies  $z_{jgs}=0$ (i.e., server $s$ is not selected to host job $j$'s GPU $g$).
% ; otherwise $z_{jgs}=0$ (i.e., server $s$ is not chosen to schedule job $j$'s GPU $g$).
 From Constraint~(\ref{eqn:add2}), we know that if $\sum_{g\in\mathcal{G}_j}z_{jgs}=G_j$ (i.e., jobs using intra-connect communication), then $x'_{js}$ could be either 0 or 1.
  However, in order to minimize $x_{js}$ (Eqn.~(\ref{eqn:add6})) to minimize $k_j$,  $x'_{js}$ will be set to 0.
 If $1\leq \sum_{g\in\mathcal{G}_j}z_{jgs}\leq G_j-1$ (i.e., jobs using inter-connect communication), then $x'_{js}=1$.
 And if $\sum_{g\in\mathcal{G}_j}z_{jgs}=0$ (i.e., server $s$ is not chosen to host job $j$'s GPUs), then $x'_{js}=1$.
 
% First, we check the correctness of Constraint~(\ref{eqn:add3}).
% Note that $x_{js}$ is determined by the product of $z_{jgs}$ and $x'_{js}$, and based on the above discussion, we have: 1) $x_{js}\geq 0$ if server $s$ is not selected to schedule job $j$'s GPU $g$ ($z_{jgs}=0$) or intra-connect communication is used ($x'_{js}=0$); 2) $x_{js}\geq 1$ if server $s$ is chosen to schedule job $j$'s GPU $g$ ($z_{jgs}=1$) and inter-connect communication is used ($x'_{js}=1$), this shows its correctness.
% 
% Second, we check the correctness of Constraint~(\ref{eqn:add4}).
% Analogously, $x_{js}$ is determined by the produce of $1-\sum_{s'\in\mathcal{S}\setminus\{s\}}z_{jgs'}$ and $x'_{js}$.
% We have: 1) $x_{js}\geq 0$ if server $s$ is not selected to schedule job $j$'s GPU $g$ ($1-\sum_{s'\in\mathcal{S}\setminus\{s\}}z_{jgs'}=0$) or intra-connect communication is used ($x'_{js}=0$); 2) $x_{js}\geq 1$ if server $s$ is chosen to schedule job $j$'s GPU $g$ ($1-\sum_{s'\in\mathcal{S}\setminus\{s\}}z_{jgs'}=1$) and inter-connect communication is used ($x'_{js}=1$), thus shows its correctness.
 
First, we check the correctness of Constraint~(\ref{eqn:add5}).
%Recall that $\chi_s$ is the binary variable to indicate whether server $s$ is selected to schedule jobs or not.
If server $s$ is chosen, i.e., $\sum_{s'\in\mathcal{S}\setminus\{s\}}z_{jgs'}=0$, implying $\chi_s\geq 1$; otherwise, $\sum_{s'\in\mathcal{S}\setminus\{s\}}z_{jgs'}=1$, then $\chi_s\geq 0$, which is conformal to the definition of $\chi_s$.

Next, we check the correctness of Constraint~(\ref{eqn:add6}).
Note that $x_{js}$ is determined by the produce of $\chi_s$ and $x'_{js}$.
 We have: 1) $x_{js}\geq 0$ if server $s$ is not selected to schedule job $j$'s GPU $g$ ($\chi_s=0$) or intra-connect communication is used ($x'_{js}=0$); 2) $x_{js}\geq 1$ if server $s$ is chosen to schedule job $j$'s GPU $g$ ($\chi_s=1$) and inter-connect communication is used ($x'_{js}=1$), thus shows its correctness.
 
 
 After adding these constraints, we next show that they could strengthen the relaxation bound, basically, we need to show that the bound of $x_{js}$ and $\chi_s$ are larger compared to those in the original Problem~(\ref{Problem:primal}).
We observe that either $z_{jgs}$ or $1-\sum_{s'\in\mathcal{S}\setminus\{s\}}z_{jgs'}$ should be larger than 0.5 since we have $z_{jgs}+\sum_{s'\in\mathcal{S}\setminus\{s\}}z_{jgs'}=1$.
In other words, $\chi_s\geq 0.5$, which is tightened from 0.
Also, based on Eqn.~(\ref{eqn:add2}), when server $s$ is chosen to schedule GPU $g$ from job $j$ using inter-connect communication, then $x'_{js}\geq 1-\sum_{g\in\mathcal{G}_j}z_{jgs}/G_j$.
As a result, $x_{js}\geq 0.5\times (1-\sum_{g\in\mathcal{G}_j}z_{jgs}/G_j)$, which is tightened from 0.
%In addition, $\chi_s\geq 0.5$ according to Eqns.~(\ref{eqn:chi_s2})(\ref{eqn:add5}), thus it also gets larger compared to 0.
Therefore, the fractional solution bound is improved.

\subsection{Solving Bilinear Constraints}
 
% 
% \subsection{Strengthen Technique One}
%
%In order to strength the relaxation, we introduce the following bilinear constraint to Problem~(\ref{Problem:primal}):
%
%\begin{align*}
%    x_{js}\geq (1-z_{jgs})\chi_s, \quad\forall j\in\mathcal{J}, g\in\mathcal{G}_j,s\in\mathcal{S}.
%\end{align*}
%The rational behind is that for the selected servers, we add some virtual worker represented by 1, and as long as $z_{jgs}\neq 1, \forall g\in\mathcal{G}_j$ (i.e., not use internal communication), it will add the non-zero value to $x_{js}$, which can improve the relaxation bound. 
%We take Fig.~\ref{fig:placement}(b) as an example, the shaded workers are the added virtual workers to each selected server (server 1 and 2 in this example).
%Then $1-z_{jgs}=0, j=1,2, g=1,2, s=1,2$, and $\chi_s>0$ for the selected servers, thus we have $x_{js}>0,j=1,2,s=1,2$ instead of $x_{js}=0, j=1,2,s=1,2$.
%And as a result, the fractional solution bound is improved.
%In order to solve such bilinear constraint, we let $z'_{js}=z_{jgs}\chi_s$.
%Traditionally, in order to solve the bilinear constraint, the McCormick inequalities\cite{McCormick76:McCormick} will be leveraged to convert $z'_{js}$ into a set of following linear constraints:
%
%\begin{align}
%    &z'_{js}\geq z_{jgs}+\chi_s-1,\quad\forall j\in\mathcal{J}, g\in\mathcal{G}_j,s\in\mathcal{S},\label{eqn:bilinear1}\\
%    &z'_{js}\leq z_{jgs},\quad\forall j\in\mathcal{J}, g\in\mathcal{G}_j,s\in\mathcal{S},\\
%       &z'_{js}\leq \chi_s,\quad\forall j\in\mathcal{J}, g\in\mathcal{G}_j,s\in\mathcal{S},\\
%    &z'_{js}\geq 0,\quad\forall j\in\mathcal{J}, g\in\mathcal{G}_j,s\in\mathcal{S}\label{eqn:bilinear2}.
%%    &x_{js}\geq \chi_s-z'_{js},\quad\forall j\in\mathcal{J}, g\in\mathcal{G}_j,s\in\mathcal{S}.
%\end{align}
%The strongest possible relaxation of the non-convex domain of the bilinear constraint is its convex hull, and has been shown to be a polyhedron\cite{Rikun97:convex-envelope}.
% In general, the McCormick relaxation may strictly contain the convex hull, leading to weaker relaxation bounds.
% However, when the bounds on the variables are all between 0 and 1, then the McCormick relaxation is equivalent to the convex hull\cite{Ryoo01:boundsformultilinear}, thus the convex envelop for the bilinear constraint domain in our case is the convex hull.
% 
% Therefore, we can obtain the following linear program after we strength the relaxation:
% \begin{align}
% \text{Minimize } &c\sum_{j\in\mathcal{J}}F_je_jk_j+\mu\sum_{s\in\mathcal{S}}N_s\chi_s\label{Problem:relax}\\
%    \text{subject to }
%    &x_{js}\geq \chi_s-z'_{js},\\
%    &z_{jgs},x_{js},\chi_s\in[0,1], k_j\geq 0, \forall j\in\mathcal{J}, g\in\mathcal{G}_j, s\in\mathcal{S},\nonumber\\
%    &\text{Constraints}~(\ref{eqn:t_j})(\ref{eqn:k_j_reformulate})(\ref{eqn:cap2})-(\ref{eqn:xjs})(\ref{eqn:bilinear1})-(\ref{eqn:bilinear2})\nonumber.
% \end{align}
% 
% Note that as long as $z_{jgs}\neq 1, \forall g\in\mathcal{G}_j$ (corresponds to internal communication case), $x_{js}>0$, which implies that the added bilinear constraint makes the bound tighter.


%\begin{align*}
%    &z'_{js}\geq 2z_{jgs}-1,\quad\forall j\in\mathcal{J}, g\in\mathcal{G}_j,s\in\mathcal{S},\\
%    &z'_{js}\leq z_{jgs},\quad\forall j\in\mathcal{J}, g\in\mathcal{G}_j,s\in\mathcal{S},\\
%    &z'_{js}\geq 0,\quad\forall j\in\mathcal{J}, g\in\mathcal{G}_j,s\in\mathcal{S},\\
%    &x_{js}\geq 4z_{jgs}-4z'_{js},\quad\forall j\in\mathcal{J}, g\in\mathcal{G}_j,s\in\mathcal{S}.
%\end{align*}

%{\color{red} The bound is still loose since the fractional values of $x_{js}$ can be arbitrary small, which makes the performance ratio less interesting.
%This issue I think is caused by the indicator function, which has the weak continuous relaxation problem in essence.}
%Here, we consider bilinear functions of the form\cite{Luedtke12:multilinear}:
%
%\begin{align*}
%f(q)=\sum_{\{i,j\}\in E}q_iq_j,
%\end{align*}
%for $q_i,q_j\in[0,1]$, where $E$ is a subset of unordered pairs of distinct indices in $N=\{1,\hdots,n\}$.
%We let $u_{ij}\triangleq q_iq_j, \forall \{i,j\}\in E$.
%Traditionally, in order to solve such bilinear function $u_{ij}$, the McCormick inequalities\cite{McCormick76:McCormick} will be leveraged to bound each term $q_iq_j$:
%\begin{align*}
%&u_{ij}\geq q_i+q_j-1,\quad\forall \{i,j\}\in E,\\
%&u_{ij}\leq q_i, \quad\forall \{i,j\}\in E,\\
%&u_{ij}\leq q_j, \quad\forall \{i,j\}\in E,\\
%&u_{ij}\geq 0,\quad\forall \{i,j\}\in E.
%\end{align*}

%We point out here that the strongest possible relaxation of the non-convex domain of the bilinear constraint is its convex hull, and has been shown to be a polyhedron\cite{Rikun97:convex-envelope}.
%In general, the McCormick relaxation may strictly contain the convex hull, leading to weaker relaxation bounds.
%However, when the bounds on the variables are all between 0 and 1, then the McCormick relaxation is equivalent to the convex hull\cite{Ryoo01:boundsformultilinear}, thus the convex envelop for the bilinear constraint domain in our case is the convex hull.
%After adding extra Constraints~(\ref{eqn:add1})-(\ref{eqn:add6}), we can see that Problem~(\ref{Problem:primal}) is a non-convex optimization problem involving bilinear functions \cite{Luedtke12:multilinear}, which is defined as $f: [l,u]\rightarrow \mathbb{R}$, where
%\begin{align*}
%f(x)=\sum_{i\in\mathcal{I}}a_i\prod_{k\in\mathcal{K}_i}q_j,
%\end{align*}
%and $[l,u]=\{q\in\mathbb{R}^n|l\leq q\leq u\}$ as well as $|\mathcal{K}_i|\leq 2,\forall i\in\mathcal{I}$.
%
%The first challenge stems from the non-linear constraint~(\ref{eqn:add3}).
%We let $z'_{js}=z_{jgs}\cdot x'_{js}$, which is a bilinear function with single term (i.e., $|\mathcal{I}|=1$).
%%In order to solve such bilinear constraint, we let $z'_{js}=z_{jgs}\cdot x'_{js}$.
%Traditionally, in order to solve such bilinear function, the McCormick inequalities\cite{McCormick76:McCormick} will be leveraged to convert $z'_{js}$ into a set of following linear constraints:

After adding extra Constraints~(\ref{eqn:add2})-(\ref{eqn:add7}), we can see that Problem~(\ref{Problem:primal}) is a non-convex optimization problem involving bilinear functions that has the above form.
We let $z'_{js}=\chi_sx'_{js}$.
Traditionally, in order to solve such bilinear function $u_{ij}$, the McCormick inequalities\cite{McCormick76:McCormick} will be leveraged to bound $z'_{js}$.
%and let $\zeta_{js'}=z_{jgs'}x'_{js}$.
%We thus can obtain the following McCormick inequalities by specializing the above formulation:

%\begin{align}
%    &z'_{js}\geq z_{jgs}+x'_{js}-1,\quad\forall j\in\mathcal{J}, g\in\mathcal{G}_j,s\in\mathcal{S},\label{eqn:bilinear1}\\
%    &z'_{js}\leq z_{jgs},\quad\forall j\in\mathcal{J}, g\in\mathcal{G}_j,s\in\mathcal{S},\\
%       &z'_{js}\leq x'_{js},\quad\forall j\in\mathcal{J}, g\in\mathcal{G}_j,s\in\mathcal{S},\\
%    &z'_{js}\geq 0,\quad\forall j\in\mathcal{J}, g\in\mathcal{G}_j,s\in\mathcal{S}\label{eqn:bilinear2}.
%%    &x_{js}\geq \chi_s-z'_{js},\quad\forall j\in\mathcal{J}, g\in\mathcal{G}_j,s\in\mathcal{S}.
%\end{align}
%We next deal with constraint~(\ref{eqn:add4}), which involves the general bilinear function.
%We let $z''_{js}=\sum_{s'\in\mathcal{S}\setminus\{s\}}z_{jgs}x'_{js}$.
We thus can replace Eqn.~(\ref{eqn:add6}) with following McCormick inequalities:
\begin{align}
&x_{js}\geq z'_{js}, \quad \forall j\in\mathcal{J}, s\in\mathcal{S},\\
&z'_{js}\geq \chi_s+x'_{js}-1,\quad\forall j\in\mathcal{J}, s\in\mathcal{S},\label{eqn:bilinear1}\\
&z'_{js}\leq \chi_s,\quad\forall j\in\mathcal{J}, s\in\mathcal{S},\label{eqn:bilinear2}\\
&z'_{js}\leq x'_{js},\quad\forall j\in\mathcal{J}, s\in\mathcal{S},\label{eqn:bilinear3}\\
&z'_{js}\geq 0,\quad\forall j\in\mathcal{J}, s\in\mathcal{S}\label{eqn:bilinear4}.
\end{align}

%{\em 2) } Similarly, we replace Egn.~(\ref{eqn:add4}) with following equations:
%\begin{align}
%&x_{js}\geq x'_{js}-\sum_{s'\in\mathcal{S}\setminus\{s\}}\zeta_{js'}, \quad \forall j\in\mathcal{J}, s\in\mathcal{S},\\
%&\zeta_{js'}\geq z_{jgs'}+x'_{js}\!-\!1,\forall j\!\in\!\mathcal{J}, g\!\in\!\mathcal{G}_j,s\!\in\!\mathcal{S},s'\!\in\!\mathcal{S}\!\setminus\!\{s\},\label{eqn:bilinear3}\\
%&\zeta_{js'}\leq z_{jgs'},\quad\forall j\in\mathcal{J}, g\in\mathcal{G}_j,s'\in\mathcal{S}\setminus\{s\},\\
%&\zeta_{js'}\leq x'_{js},\quad\forall j\in\mathcal{J},s\in\mathcal{S}, s'\in\mathcal{S}\setminus\{s\},\\
%&\zeta_{js'}\geq 0,\quad\forall j\in\mathcal{J},s'\in\mathcal{S}\setminus\{s\}\label{eqn:bilinear4}.
%\end{align}

Several important remarks are in order:

{\em 1): } If server $s$ is not selected ($x'_{js}=1$ and $\chi_s=0$), then $z'_{js}\geq \chi_s+x'_{js}-1=0$, implying $x_{js}\geq z'_{js}=0$, thus $x_{js}=0$.

{\em 2): } If server $s$ is selected and intra-connect communication is performed ($x'_{js}=0$ and $\chi_s=1$), then $z'_{js}\geq \chi_s+x'_{js}-1= 0$, implying $x_{js}\geq z'_{js}=0$, thus $x_{js}=0$.

{\em 3): } If server $s$ is selected and inter-connect communication is performed ($x'_{js}>0$ and $\chi_s>0$), then $z'_{js}\geq \chi_s+x'_{js}-1\geq 0.5+1-\sum_{g\in\mathcal{G}_j}z_{jgs}/G_j-1\geq 0.5-\sum_{g\in\mathcal{G}_j}z_{jgs}/G_j$, implying $x_{js}\leq 0.5$.
% implying $x_{js}\geq z'_{js}$, which implies $x_{js}\leq 0.5$. {\color{red}The convex hull operation actually worsen the bound of $x_{js}$.}
It shows that the McCormick relaxation technique actually worsen the bound of $x_{js}$, but $\chi_s$ is not influenced.


We point out here that the strongest possible relaxation of the non-convex domain of the bilinear constraint is its convex hull, and has been shown to be a polyhedron\cite{Rikun97:convex-envelope}.
In general, the McCormick relaxation may strictly contain the convex hull, leading to weaker relaxation bounds.
However, when the bounds on the variables are all between 0 and 1, then the McCormick relaxation is equivalent to the convex hull\cite{Ryoo01:boundsformultilinear}, thus the convex envelop for the bilinear constraint domain in our case is the convex hull.

After the McCormick transformation and continuous relaxation, Problem~(\ref{Problem:primal}) becomes a linear program, which can be solved efficiently by LP solvers (e.g., Gurobi) to obtain the fractional solution.
 

 \section{Dependent Rounding Scheme}\label{sec:rounding}
 
The fractional solution returned by solving Problem~(\ref{Problem:primal}) is for the relaxed program.
The number of GPUs of each job should take non-negative integer values in each server.
% It is highly challenging to round Problem~(\ref{problem:pt}) due to its complicated packing and cover constraints as well as equality constraint~(\ref{ctr:gpu}) involved, making it impossible to round to integers efficiently.
% Therefore, we relax the equality constraint~(\ref{ctr:gpu}), i.e., $\sum_{s\in\mathcal{S}}y_s^j[t]\leq G^j$, to do the rounding.
% However, we will show later that the summation of rounded integers is at least $G^j-1$.
% In other words, from the cloud provider's perspective, the efficient training achieved at the cost of at most one extra GPU needs to be added to the submitted job.
We need to round the fractional solution $z_{jgs}$, $\forall j\in\mathcal{J},g\in\mathcal{G}_j, s\in\mathcal{S}$ into integer solution while not to violate Constraints~(\ref{eqn:gpu2})(\ref{eqn:cap2}).
In addition, we need to take the $\chi_s$ and $k_j$ into consideration to minimize the gap between the fractional solution and the integer solution after rounding to offer a better performance ratio.
Note that the variables are dependent on each other due to those coupling constraints.
The traditional independent rounding scheme where each variable is rounded up or down independently may well lead to constraint violation.
Hence we design a novel dependent rounding scheme by exploring the inherent dependence among variables.
 
 \begin{figure}[t]
    \centering
    \includegraphics[width=0.48\textwidth]{Figures/fig_round.eps}
    \caption{Example on fraction merge before rounding.}\label{fig:round}
%        \vspace{-.1in}
\end{figure}
 
 
 Recall that after the continuous relaxation, the system tends to break down each GPU into similar fractional values in order to minimize $x_{js}$ based on Eqn.~(\ref{eqn:xjs}).
 In other words, each GPU of the job may distribute its partial values over multiple servers, and the server may contain its each GPU's partial value. 
 As an example illustrated in Fig.~\ref{fig:round}(a), where job 1 requires three GPUs and job 2 requires two GPUs.
 In order to distinguish GPUs, we index them as $1, 2,\hdots, n$.
 Before we rounding the fractional solution, we first merge these partial values of the same job to maintain the capacity constraint of each server.
 As we can see from Fig.~\ref{fig:round}(b), after we perform the value fusion, in each server, at most one partial value for each job will occur.
 

 We let $\hat{y}_{js}\triangleq\lfloor\sum_{g\in\mathcal{G}_j}z_{jgs}\rfloor, \forall j\in\mathcal{J}, s\in\mathcal{S}$.
 Let $\hat{z}_{js}\triangleq \sum_{g\in\mathcal{G}_j}z_{jgs}-\hat{y}_{js}, \forall j\in\mathcal{J}, s\in\mathcal{S}$ , i.e., the remaining fractional value after the merge operation of job $j$ in server $s$.
 Let $\hat{N}_s\triangleq \max\{1,N_s-\sum_{j\in\mathcal{J}}\hat{y}_{js}\}, \forall s\in\mathcal{S}$, i.e., the remaining capacity of server $s$ (if the remaining capacity is less than 1, then round it up to 1).
 Let $L_j=\sum_{s\in\mathcal{S}}\hat{z}_{js}$ be the number of tasks (GPUs) associated with job $j$, then the total number of tasks to be scheduled is $L=\sum_{j\in\mathcal{J}}L_j$.
 We use $\mathcal{L}=\{\mathcal{L}_1,\hdots,\mathcal{L}_J\}$ to denote the ordered set of tasks to be rounded, where $\mathcal{L}_j$ is the set of tasks related to job $j$.
% We reduce the problem to Generalized Assignment Problem (GAP), where the number of jobs is $L=\sum_{j\in\mathcal{J}}\sum_{s\in\mathcal{S}}\hat{z}_{js}$.
We reduce the problem to Generalized Assignment Problem (GAP), where the number of tasks to be scheduled is $L$ and the number of machines is $S$.
% and use $\mathcal{H}, H$ to denote the set and number of machines to be scheduled, respectively i.e., servers that has fractional placement.
% We use $N_h$ to denote the remaining capacity of machine $h$, i.e., $N_h=N_s, \forall s\in\mathcal{H}$.
 We use $C_{ls}$ to denote the cost of assigning task $l$ to server $s$,  and we let $C_{ls}=G_j-\hat{y}_{js}$.
 The rational behind is in order to minimize $k_j$, intra-connect communication should be preferred, i.e., servers that already host most GPUs should have preference to schedule the rest fractional GPUs.
 We also use binary variable $\zeta_{ls}$ to indicate whether task $l$ is placed to server $s$ ($\zeta_{ls}=1$) or not ($\zeta_{ls}=0$).
 Then, the GAP problem we consider is as follows:
 \begin{align}
\underset{\zeta}{\textbf{GAP: }\text{Minimize  }}&\sum_{s\in\mathcal{S}}\sum_{l\in\mathcal{L}}C_{ls}\zeta_{ls}\leq \beta\nonumber\\
 \text{subject to }&\sum_{s\in\mathcal{S}}\zeta_{ls}=1, \quad \forall l\in\mathcal{L},\label{eqn:assignment}\\
 &\sum_{l\in\mathcal{L}}\zeta_{ls}\leq \hat{N}_s, \quad \forall s\in\mathcal{S},\label{eqn:capacity}\\
 &\zeta_{ls}\geq 0, \quad \forall l\in\mathcal{L}, s\in\mathcal{S}\nonumber.
%&\zeta_{ls}=0, \quad \text{if } 1> \hat{N}_s, \forall l\in\mathcal{L}, s\in\mathcal{S}\nonumber.
 \end{align}
 We next leverage ST rounding\cite{Shmoys93:GAP} to obtain the integral solution from the fractional solution.
 We first construct a weighted bipartite graph $G=\langle \mathcal{L}, \mathcal{S}, E\rangle$ based on $\zeta_{ls}$ as follows:
 
 {\em Step 1: } One side of the bipartite graph consists of task nodes: $\mathcal{L}=\{u_l | l=1,\hdots,L\}$, and the other side of the contains server nodes: $\mathcal{S}=\{v_{s\gamma} | s=1,\hdots, S, \gamma=1,\hdots,\Gamma_s\}$, where $\Gamma_s=\lceil \sum_{l\in\mathcal{L}}\zeta_{ls}\rceil$.
 Basically, we assign $\Gamma_s$ task nodes to server $s$.
 
 {\em Step 2: } For each server $s$, we can view server nodes $v_{s\gamma}$ as unit capacity bins, and view $\zeta_{ls}, \forall l\in\mathcal{L}$ as pieces of tasks scheduled to these bins.
 We keep placing pieces into bin node $v_{s1}$ one by one until placing piece $l$ exceed the unit capacity, then partial of $l$ will be placed to $v_{s1}$ to reach its capacity, and the remaining fraction will be placed to next bin $v_{s2}$.
 The process is continued until all pieces are scheduled to bins.
 
 {\em Step 3: } We add edge $(u_l,v_{s\gamma})$ to $E$ if a fraction of task $l$ is placed to bin $v_{s\gamma}$.
 We use $y'(u_l,v_{s\gamma})$ to denote the fraction of task $l$ places to bin $v_{s\gamma}$, and set the cost of this edge to $C_{ls}$.
 
 Note that the vector $y'$ is a fractional matching in bipartite graph $G$ that exactly matches all task nodes.
 There exists an integral matching with objective value at most $\beta$ according to matching theory\cite{Lovasz09:matchingtheory}, which also exactly matches all task nodes.
 We summarize the rounding procedure in Algorithm~\ref{alg:round}:
 \begin{algorithm}
\SetAlgoLined
\nonl\textbf{Input:} $\zeta_{ls},\forall l,s$\;
\nonl\textbf{Initialization:} $\bar{\zeta}_{ls}=0,\forall l,s$\;
Build a bipartite graph $G=\langle \mathcal{L}, \mathcal{S}, E\rangle$ based on $\zeta_{ls}$ as illustrated above\;
Find an integer matching that exactly matches all job nodes in $G$ with the minimum GAP objective value\;
If task $l$ is mapped to server $s$, then update $\bar{\zeta}_{ls}=1$\;
\Return $\bar{\zeta}_{ls},\forall l,s$\;
\caption{Rounding Algorithm.}
 \label{alg:round}
\end{algorithm} 

After the rounding, we update the integral solution $y_{js}=\hat{y}_{js}+\sum_{l\in\mathcal{L}_j}\bar{\zeta}_{ls},\forall j,s$.
Then we can obtain the integral $k_j, \forall j$ and $\chi_s,\forall s$ based on $y_{js},\forall j,s$.

 
 Next, we provide the theoretical analysis with respect to our algorithms.
 
 {\em 1) Feasibility Discussion:}
 
 \begin{thm}\label{thm:feasibility}
 The integral solution returned by Algorithm~\ref{alg:round} guarantees Constraint~(\ref{eqn:assignment}) to be satisfied, and the violation of the capacity constraint~(\ref{eqn:capacity}) is at most twice of $\hat{N}_s$, i.e., $\sum_{l\in\mathcal{L}}\bar{\zeta}_{ls}\leq 2\hat{N}_s, \forall s\in\mathcal{S}$.
 \end{thm}
 \begin{proof}
 Recall that Algorithm~\ref{alg:round} generates an integral matching that exactly matches all task nodes, thus Constraint~(\ref{eqn:assignment}) is satisfied.
 In order to show the violation of capacity constraint~(\ref{eqn:capacity}) is at most twice of $\hat{N}_s$.
 Note that the total GPU resource consumption of tasks scheduled to server $s$ by any integral matching in $G$ is no greater than $\sum_{\gamma=1}^{\Gamma_s}1$.
% We consider the following two cases:
% 
% {\em i): } $\hat{N}_s<1$, then $\Gamma_s=\lceil \sum_{l\in\mathcal{L}}\zeta_{ls} \rceil=1$.
% 
% Clearly, $\sum_{\gamma=1}^{\Gamma_s}1\leq 1$.
% 
% {\em ii): } 
And it is clear that $1\leq \hat{N}_s$, then we have:
 \begin{align*}
 \sum_{\gamma=2}^{\Gamma_s}1&=\sum_{\gamma=1}^{\Gamma_s-1}1= \sum_{\gamma=1}^{\Gamma_s-1}\sum_{l:(u_l,v_{s\gamma})\in E}y'(u_l,v_{s\gamma})\\
 &\leq \sum_{\gamma=1}^{\Gamma_s}\sum_{l:(u_l,v_{s\gamma})\in E}y'(u_l,v_{s\gamma})=\sum_{l\in\mathcal{L}}\zeta_{lh}\leq \hat{N}_s.
 \end{align*}
 Hence we have $\sum_{\gamma=1}^{\Gamma_s}1=1+\sum_{\gamma=2}^{\Gamma_s}1\leq 2\hat{N}_s$, and the proof is complete.
 \end{proof}

 
 {\em 2) Time Complexity:}
 
 \begin{thm}\label{thm:time}
 The time complexity of our algorithm is $O(S^3+SJ^2\log J)$, which is polynomial.
 \end{thm}
 \begin{proof}
 Our algorithm consists of three main steps: i) Solving the LP relaxation of Problem~(\ref{Problem:primal}) can be approximately bounded by $O(S^3)$ if we use a polynomial time LP solver (e.g., Vaidya's algorithm\cite{Vaidya87:LP}); 
% ii) Constructing GAP problem based on the returned fractional solution takes $O(\sum_{j\in\mathcal{J}}G_j)=O(J)$; 
 ii) The ST rounding in Algorithm~\ref{alg:round} takes $O(SJ^2\log J)$\cite{Shmoys93:GAP};
 iii) Update the integral solution $y_{js}$ and obtain the integral $k_j$ and $\chi_s$ takes $O(SJ)$.
 Therefore, the time complexity of our algorithm is $O(S^3+SJ^2\log J)$, which is polynomial.
 \end{proof}
 
 
 \begin{lem}
\label{lem:relation} Let  $A(\mathbf{x})\!=\!\frac{\sum_{k=1}^nf(k,\mathbf{x})}{\sum_{k=1}^ng(k,\mathbf{x})}$, and $B(\mathbf{x})\!=\!\sum_{k=1}^n\frac{f(k,\mathbf{x})}{g(k,\mathbf{x})}$.
If both $f(\cdot)$ and $g(\cdot)$ are non-negativity, then we have $A(\mathbf{x})\leq B(\mathbf{x})$.
\end{lem}

\begin{proof}
$\frac{f(k,\mathbf{x})}{\sum_{k=1}^ng(k,\mathbf{x})}\leq\frac{f(k,\mathbf{x})}{g(k,\mathbf{x})}$, since $g(k,\mathbf{x})\leq\sum_{k=1}^ng(k,\mathbf{x})$.
Thus $A(\mathbf{x})=\frac{\sum_{k=1}^nf(k,\mathbf{x})}{\sum_{k=1}^ng(k,\mathbf{x})}=\sum_{k=1}^n\frac{f(k,\mathbf{x})}{\sum_{k=1}^ng(k,\mathbf{x})}\leq\sum_{k=1}^n\frac{f(k,\mathbf{x})}{g(k,\mathbf{x})}=B(\mathbf{x})$.
\end{proof}
 
 
 {\em 3) Approximation Ratio:}  The approximation is the worst-case ratio between the objective value achieved by our algorithm and the objective ratio achieved by some off-line optimal algorithm.
 
 
 \begin{thm}\label{thm:ratio}
Our algorithm is $N^{\max}/N^{\min}+2$-approximation, where $ N^{\max}=\max_{j,s}\{N_s,G_j\}$ and $N^{\min}=\min_j\{1-\sum_gz_{jgs}/G_j)\}$.
 \end{thm}
 
 \begin{proof}
 We let $\bar{k}_j, \bar{\chi}_s$ and $\bar{k}_j^*, \bar{\chi}_s^*$ be the integral solution returned by our solution and the optimal integral solution obtained by some offline algorithm.
 Let $\hat{k}_j, \hat{\chi}_s$ be the fractional solution by solving Problem~(\ref{Problem:primal}) after continuous relaxation without McCormick inequality operation.
 Note that $\bar{k}_j\leq\alpha N^{\max}$, where $ N^{\max}=\max_{j,s}\{N_s,G_j\}$ since the largest number of concurrent running jobs is bounded by both the server's capacity and the number of GPUs required, and $\bar{\chi}_s\leq 1$.
 Note that if $\hat{k}_j=0$, then we have $\bar{k}_j=0$, thus we consider the inter-connect communication jobs, i.e., $\hat{k}_j>0$. 
And we have $\hat{k}_j\geq \alpha \sum_{j'}x_{j's}\geq \alpha\sum_{j'}(1-\sum_gz_{jgs}/G_j)=\alpha N^{\min}$, where $N^{\min}\!=\!\min_j\{1-\sum_gz_{jgs}/G_j\}$, and $\hat{\chi}_s\geq 1/2$.
 With Lemma~\ref{lem:relation}, the approximation ratio can be computed as:
 \begin{align*}
 &\frac{c\sum_{j\in\mathcal{J}}F_je_j\bar{k}_j+\mu\sum_{s\in\mathcal{S}}N_s\bar{\chi}_s}{c\sum_{j\in\mathcal{J}}F_je_j\bar{k}_j^*+\mu\sum_{s\in\mathcal{S}}N_s\bar{\chi}_s^*}\\
 &\leq \frac{c\sum_{j\in\mathcal{J}}F_je_j\bar{k}_j}{c\sum_{j\in\mathcal{J}}F_je_j\bar{k}_j^*}+\frac{\mu\sum_{s\in\mathcal{S}}N_s\bar{\chi}_s}{\mu\sum_{s\in\mathcal{S}}N_s\bar{\chi}_s^*}\\
 &\leq \frac{c\sum_{j\in\mathcal{J}}F_je_j\bar{k}_j}{c\sum_{j\in\mathcal{J}}F_je_j\hat{k}_j}+\frac{\mu\sum_{s\in\mathcal{S}}N_s\bar{\chi}_s}{\mu\sum_{s\in\mathcal{S}}N_s\hat{\chi}_s}\\
 &\leq \frac{N^{\max}}{N^{\min}}+2.
 \end{align*}
 \end{proof}
 
 
 
 










==> Supporting_Preambles/jackmac.tex <==
%>From snoeyink%cs.ubc.ca@cs.Technion.AC.IL Wed Nov  3 08:18:27 1993
%Received: from csmail.cs.technion.ac.il by math.tau.ac.il (5.67/math.tau-930921)
	%id AA17625; Wed, 3 Nov 93 08:18:23 +0200
%Received: from csc (csc.cs.technion.ac.il) by csmail.cs.Technion.AC.IL (4.1/3.14)
	%id AA14244; Wed, 3 Nov 93 01:19:10 IST
%Received: from csa by csc (4.1/3.14)
	%id AA24688; Wed, 3 Nov 93 01:19:48 IST
%Received: from grolsch.cs.ubc.ca by csa (4.1/3.14)
	%id AA20525; Wed, 3 Nov 93 01:11:28 IST
%Return-Path: <snoeyink@cs.ubc.ca>
%Received: from cascade.cs.ubc.ca by grolsch.cs.ubc.ca with SMTP id AA13516
  %(5.65c/IDA-1.3.5 for alon@cs.Technion.AC.IL); Tue, 2 Nov 1993 13:56:34 -0800
%Date: Tue, 2 Nov 1993 13:56:34 -0800
%From: Jack Snoeyink <snoeyink%cs.ubc.ca@cs.Technion.AC.IL>
%Message-Id: <199311022156.AA13516@grolsch.cs.ubc.ca>
%Received: by cascade.cs.ubc.ca (4.1/SMI-4.1)
	%id AA21873; Tue, 2 Nov 93 13:56:33 PST
%To: alon@cs.Technion.AC.IL
%In-Reply-To: Alon Efrat's message of Sun, 31 Oct 93 23:38:48 IST <9310312138.AA19880@csc>
%Subject: LaTex Macros
%Status: RO
%Content-Length: 19065
%X-Lines: 638
%
%
%I'm in oberwolfach w/ micha, so I';ll just send you this and answer
%your questions on it when I get back to vancouver next week...
%
    %o                                    Jack
  %_/\_.
%(')>-(`)                          snoeyink@cs.ubc.ca
%----figbox.tex----

% 12 Oct 90 LaTeX figure boxing macros  by Jack Snoeyink
%					w/ ideas from John Hershberger
%					and code from Tom Rokicki
%%%%%%%%%%%%%%%%%
% 
% This file contains two classes of macros for dealing with figures in
% Latex documents:  
%  \figbox (and its relatives) take a box containing a figure or table
%    or whatever, caption it, and either place it on the page and wrap the
%    text around it or let it float (as usual).
%  \boxeps and \boxps take encasulated or plain postscript from a file
%    and put it in a box for use by \figbox
%
%%%%%%%%%%%%%%%%
%
% The most important macro for dealing with boxes is:
%
% \figbox: caption a box as a figure or table and place it in the margin
% 	(a marginal box) or float it (a floating box).
% 	Wide marginal boxes are promoted to one column floats; wide one
% 	column floats are promoted to two column floats.
%
% Usage: \figbox [*htblr] {box} {style} {label} {caption}
%
% The optional argument default is [htb].  Other choices
%   * two column (must come first),
%   h here, t top, b bottom (as in latex),
%   l left, r right (marginal boxes that do not float)
%
% NB: Left and right marginal boxes will not overlap in height.
%
% Two column figures default to htb unless some other 
%   	options follow the *.
%   They can also be specified by style {figure*} or {table*}.
%
% box is a box containing a figure or table.
% style is the caption style {figure}, {figure*}, {table}, or {table*}.  
% label is the label assigned.
%	if empty, the figure will not be labeled.
% caption is of the form {}, {Caption} or {[short caption] Long caption},
%       where the short caption goes into the list of figures/tables.
%	if empty, the figure will not be captioned or labeled.
% 
% The lower level macro \captionbox, described much later, can be used
% to combine two or more captioned figures into a single marginal or
% floating box.
%
%%%%%%%%%%%%%%%%
%
% options defined by macros are: \captionstyle \boxcaptionstyle
% \maxfigfraction \figboxhang \figboxmargin 
%
% \captionstyle is executed for all floating box captions
% \boxcaptionstyle is executed for all marginal box captions.
%	Default \raggedright
% \maxfigfraction is the maximum fraction of a column that can be taken up
% 	by a marginal box before it gets converted to a float.
% 	Default .6
% dimen \figboxhang is the distance a marginal box hangs into the margin.
%	Default 0pt
% dimen \figboxmargin is the width of space between the text and a
% 	marginal box. 
%	Default .15in
%
%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%
%
% The most important macros for turning postscript into boxes are:
% 
% \boxeps: Form a box containing encapsulated postscript from a file at a
%	given scale.
% \boxps: Form a box containing postscript from a file at a given scale, 
% 	width, and height.
% 
%
% Usage: \boxeps[local commands] {file} {scale}
%	 \boxps[local commands] {file} {scale} {width} {height}
%
% The optional local commands are executed after scaling. As described
% 	below, they are useful for setting origins, non-uniform scaling, etc?
% file is the filename in the \figuredirectory and without the .ps
% 	extension.
% scale is a real number: 1 to use the drawn size.  0.9 to use 90% of
% 	drawn size.  Can be changed by local commands. (see below)
% width and height are dimensions of the box produced by \boxps.
%
%%%%%%%%%%%%%%%%
%
% options: \DVIscaling \figuredirectory \missingfigure \boxer
% local commands: \horizscale \vertscale
%
% \DVIscaling is the number the dvi to ps converter considers a unit
% 	scaling transformation.  Default: 1 for dvi2ps  --- 100 for
% 	some of Rokicki's versions of dvips.
%
% \globalscaling is the scaling applied to every picture --- useful
% 	for making double size figures for journals.  Default: 1
%
% \figuredirectory is the pathname where figure postscript files are kept.
%	Default: ./figure
%
% \missingfigure{file} is executed when the file is not found.
%	Default: \def\missingfigure#1{\hbox{Missing figure #1.ps}}
%
% \boxer is the command used by \boxps to make a box of the desired size
% 	containing the figure.  Possible commands depend on the origin of
% 	the figure, and include \llboxer \lcboxer \ulboxer and \ccboxer.
% 	(ll = lower left, ul = upper left, cc = dead center, etc.)
%	\boxer can be defined in the local commands or globally.
%
% Local commands \horizscale, and \vertscale can scale the picture
% 	horizontally and vertically by different factors.  \scale
% 	scales the picture uniformly.  Scales accumulate.
%
%%%%%%%%%%%%%%%%



%%%%%%%%%%%%%%%%
%
% Default options
%

\def\captionstyle{}
\def\boxcaptionstyle{\raggedright}

\def\maxfigfraction{.6}% 	--- max frac of column for marg figure

\newdimen\figboxmargin%		--- margin between text and picture
\figboxmargin = .15in

\newdimen\figboxhang%		--- amount to hang picture into margin
\figboxhang = 0pt

\def\DVIscaling{1}%		--- for dvi2ps
\def\globalscaling{1}%		--- for scaling everything
\def\figuredirectory{./figures}%--- where to find the .ps files 
\let\boxer=\llboxer%		--- default origin in lower left for non-
%				      encapsulated postscript figures

\def\missingfigure#1{\hbox{Missing figure #1.ps}}


%%%%%%%%%%%%%%%%
%
% Use latex internals
%
\catcode `\@=11
\special{! /@scaleunit 1 def }

\newbox\figurebox

\def\figbox{%	[place] box style label caption
\@ifnextchar[{\figboxaux}{\figboxaux[htb]}}

%
% Parse position parameters and try appropriate placement
%
\long\def\figboxaux[#1#2]#3#4#5#6{%	--- want left margin figure?
\writepict{{#3}{#4}{#5}{#6}}%		--- save figure if journalpicts
\setbox\figurebox\hbox{#3}%
\if l#1\tryleftbox{#4}{#5}{#6}%
\else%					--- want right margin figure?
\if r#1\tryrightbox{#4}{#5}{#6}%
\else%					--- want one or two column figure?
\if *#1\checktwocoloptions#2]{\box\figurebox}{#4*}{#5}{#6}%
\else\tryonecol[#1#2]{#4}{#5}{#6}%
\fi
\fi
\fi\ignorespaces}

%
% Try a placement; promote if too wide
%

\long\def\tryleftbox#1#2#3{%		--- does left margin figure fit?
\ifdim\wd\figurebox>\maxfigfraction\columnwidth \tryonecol[htb]{#1}{#2}{#3}%
\else\leftbox{\captionbox{\box\figurebox}{#1}{#2}{#3}}\fi}

\long\def\tryrightbox#1#2#3{%	--- does right margin figure fit?
\ifdim\wd\figurebox>\maxfigfraction\columnwidth \tryonecol[htb]{#1}{#2}{#3}%
\else\rightbox{\captionbox{\box\figurebox}{#1}{#2}{#3}}\fi}

\def\checktwocoloptions{%	--- make sure twocol has htb or p
\@ifnextchar]{\floatbox[htb}{\floatbox[}}

\long\def\tryonecol[#1]#2#3#4{%	--- does one column figure fit?
\ifdim\wd\figurebox>\columnwidth \floatbox[#1]{\box\figurebox}{#2*}{#3}{#4}%
\else\floatbox[#1]{\box\figurebox}{#2}{#3}{#4}\fi}

%
% Do the work for a floating box.
%
% \floatbox[place]{box} {style} {label} {caption}
%

\long\def\floatbox[#1]#2#3#4#5{%
\begin{#3}[#1]
\hbox to \hsize{\hfil#2\hfil}
\captionandlabel{#3}{#4}{#5}
\end{#3}
}


%
% Make a caption the width of the box with given style. 
%
%\captionbox {box} {style} {label} {[optshortcap] caption}
%
% options: \boxcaptionstyle 
%
%%%%%%%%%%%%%%%%
%
% This can be used with box commands (\hbox, \vbox, \mbox, and the like),
% along with \figbox with an empty caption, to place two or more captioned
% boxes in a single marginal or floating box.   
%
% e.g. \figbox{\hbox{
%		     \captionbox{ \boxeps{fig1}1} {figure} {f1} {a figure}
%		     \hskip 1in
%		     \captionbox{ \boxeps{tab1}1} {table} {t1} {a table}
%		    }} {figure} {ignored-label} {}
%

\long\def\captionbox#1#2#3#4{% box style label {[optshortcap] caption}
\setbox\figurebox\hbox{#1}%
\parbox[t]{\wd\figurebox}{%
\bigskip\box\figurebox
\let\captionstyle=\boxcaptionstyle
\captionandlabel{#2}{#3}{#4}
\bigskip
}}

%				--- caption and label if label is nonempty
\def\captionandlabel#1#2#3{% 	--- {style} {label} {caption}
\def\testit{#3}%
\ifx\testit\empty\else%		--- if non empty caption
\writecapt{{#1}{#2}{#3}}%	--- save for journal figs
\captypeunstarred#1*.%		--- remove optional stars
\getcaption#3\endc@ption%       --- parse the caption
\def\testit{#2}%		--- check for empty label
\ifx\testit\empty\else\label{#2}\fi
\fi}

\def\captypeunstarred#1*#2.{%	--- remove two-column star from style
\def\@captype{#1}}

%
% Parse the caption of the form {caption} or {[short] long caption} 
%

\def\getcaption{\@ifnextchar[{\getcaptwo}{\getcapone}}
\long\def\getcapone#1\endc@ption{\caption[#1]%
{\def\baselinestretch{1}\Large\normalsize\captionstyle\ignorespaces #1}}
\long\def\getcaptwo[#1]#2\endc@ption{\caption[#1]%
{\def\baselinestretch{1}\Large\normalsize\captionstyle\ignorespaces #2}}

%
% Do the right thing with an already captioned marginal box
%
% \leftbox{box}
% \rightbox{box}
%
% options: \figboxmargin \figboxhang \figuredirectory

\newdimen\figboxht
\newcount\figboxn


\newcount\figboxlines%		--- picture height in number of lines
\newdimen\figboxwid%		--- picture width

\newif\ifisleftbox

\long\def\leftbox#1{%
\setbox\figurebox\hbox{#1}\global\isleftboxtrue
\startmarginbox
\vadjust{\smash{\rlap{\hskip\hsize\hskip\figboxhang
\llap{\raise.7\baselineskip\box\figurebox\hskip\rightskip}}}}%
\endmarginbox%
}

\long\def\rightbox#1{%
\setbox\figurebox\hbox{#1}\global\isleftboxfalse
\startmarginbox
\smash{\llap{\raise.7\baselineskip\box\figurebox\hskip\figboxmargin}}%
\endmarginbox%
}

\def\startmarginbox{%
\ifvmode\passpict\let\endmarginbox=\indent
\else\message{WARNING: marginbox in not in vmode}\hfilneg\ \passpict
\let\endmarginbox=\relax\fi
%
\figboxht=\dp\figurebox%	 actual height
\advance\figboxht by 1.3\baselineskip% round up
\vskip\figboxht\penalty-300\vskip-\figboxht% filbreak trick
\divide\figboxht by\baselineskip%      how many lines?
\global\figboxlines=\figboxht
%
\global\figboxwid=\wd\figurebox
\global\advance\figboxwid by \figboxmargin
\global\advance\figboxwid by -\figboxhang
\setmypar\noindent}
%

%
% Useful macros
%
% for lengthening (and shortening) picture space
%
\def\addlines#1{\global\advance\figboxlines by #1\myparshape}
\def\zerolines{\origpar\global\figboxlines=0\myparshape}

%
% for passing any marginal figures
%
\def\passpict{\par\ifnum\figboxlines>1\vskip\figboxlines\baselineskip
\zerolines\fi}

\def\emptybox#1#2{\hbox to #1{\vbox to #2{\vss}\hss}}

%%%%%%%%%%%%%%%%%%%%%
%\par hacking  
% We define our own version of Tex's \par and tell Latex it is the original

\global\let\origpar=\@@par%	--- Latex's saved version of Tex's \par
\global\let\dopar=\origpar
\global\def\@@par{\dopar}
\@setpar{\dopar}

\def\setmypar{\global\let\dopar=\mypar
\global\prevgraf=0\myparshape}

\def\mypar{\origpar\global\advance\figboxlines by -\prevgraf%
\global\prevgraf=0\myparshape}

\def\myparshape{\relax%
\ifnum\figboxlines>1\theparshape \else
\global\hangindent=0pt\global\hangafter=1%  these sometimes get restored...
\global\let\dopar=\origpar\fi}

\def\theparshape{%
\ifisleftbox\global\hangindent=-\figboxwid 
\else\global\hangindent=\figboxwid \fi
\global\hangafter=-\figboxlines \global\advance\hangafter by 1%
}


%%%%%%%%%%%%%%%%
%
%  Macros to make the list of figures and captions used by journals
%
%  To use, execute \journalpicts{scalefactor} at the beginning of the
%  file.  All figbox figures and tables will be written to a .pic file
%  and all captions to a .cap file.  On \enddocument, these files are
%  read in and the lists of figures and captions are produced.
%  
%  For non-english versions, or to add other types of floats, the
%  macro \definefnum should be changed.
%

\def\definefnum#1{%		--- ugly latex hacking to get the
%		 			right figure/table name 
\def\fnum@figure{Figure \ref{#1}}%
\def\fnum@table{Table \ref{#1}}%
\def\fnum@code{Algorithm \ref{#1}}%
}

\def\writepict#1{}
\def\writecapt#1{}

%%%%%%%%%%%%%%%%
% \journalpicts{globalscalefactor} writes all pictures and captions to
% 	files and modifies \enddocument to read these files and
% 	produce lists of enlarged figures and of captions
% 

\def\journalpicts#1{% 		global scale factor
\newwrite\pictfile
\newwrite\captfile
%
\openout\pictfile\jobname.pic
\openout\captfile\jobname.cap
%
\gdef\writepict##1{\unexpandedwrite\pictfile{\doit##1}}%
\gdef\writecapt##1{\unexpandedwrite\captfile{\doit##1}}%
%
\global\let\ENDdocument=\enddocument
\gdef\enddocument{\DOjournalpicts{#1}\ENDdocument}
}

%
%	generate enlarged figures 1 per page and list captions
%
\def\DOjournalpicts#1{{%
\def\writepict##1{}\closeout\pictfile
\def\writecapt##1{}\closeout\captfile
\@fileswfalse%			--- turn off toc, lof, and so on.
%
\onecolumn
\def\globalscaling{#1}
\def\doit##1##2##3##4{%		--- print a picture on blank page
%					{box}{style}{label}{caption}
\figboxaux[t]{\hss##1\hss}{##2}{}{}%
\vspace*{1in}
\definefnum{##3}%		--- use Figure \ref{label} or Table \ref{label}
\captionandlabel{##2}{}{##4}
\clearpage}%
%
\input\jobname.pic
%
\def\doit##1##2##3{%		--- print caption
%					{style}{label}{caption}
\definefnum{##2}%		--- use Figure \ref{label} or Table \ref{label}
\captionandlabel{##1}{}{##3}}%
%
\raggedright\let\captionstyle=\raggedright
\def\@makecaption##1##2{##1: ##2\par}%  --- Be sure captions aren't centered
%
\input\jobname.cap
}}%				--- to be followed by \enddocument



%%%%%%%%%%%%%%%%
%
%  Box macros
%
%%%%%%%%%%%%%%%%
%
% \boxeps[local commands] {file} {scale}
%
% options \DVIscaling \figuredirectory \scale \horizscale \vertscale
% \missingfigure \globalscaling
%
% \boxps[local commands] {file} {scale} {width} {height}
%
% \scale \horizscale \vertscale 

%
%  Various `boxers' --- which one is used depends on where the origin
%  of the picture is.  If you are using the bounding boxes of
%  encapsulated postscript, just use the default \llboxer.  Otherwise,
%  you have to figure out where the origin is and set \boxer appropriately.
%

\def\llboxer#1{\vbox to \figboxht{\vfil\hbox to \figboxwid{#1\hfill}}}
\def\lcboxer#1{\vbox to \figboxht{\vfil\hbox to \figboxwid{\hfill#1\hfill}}}
\def\oldboxer#1{\vbox to \figboxht{\vfil
		      \hbox to \figboxwid{\hfill\llap{#1\hskip4.25in}\hfill}}}
\def\ulboxer#1{\vbox to \figboxht{\hbox to \figboxwid{#1\hfill}\vfil}}
\def\ccboxer#1{\vbox to \figboxht{\vfil
			\hbox to \figboxwid{\hfill#1\hfill}\vfil}}

% a macro to strip the pt off a dimension
%
{\catcode`\p=12\catcode`\t=12
\gdef\removedimen#1pt{#1}}

\def\defscaled#1#2{#2=\DVIscaling#2%
\xdef#1{\expandafter\removedimen\the#2}}

\def\DVIspace{ }
\newdimen\hscalefactor
\newdimen\vscalefactor

\def\scale#1{\horizscale{#1}\vertscale{#1}}
\def\horizscale#1{\hscalefactor=#1\hscalefactor\figboxht=#1\figboxht}
\def\vertscale#1{\vscalefactor=#1\vscalefactor\figboxwid=#1\figboxwid}

%%%%%%%%%%%%%%%%
%

\def\boxps{%
\@ifnextchar[{\boxpsaux}{\boxpsaux[\relax]}}

\def\boxpsaux[#1]#2#3#4#5{%
{\figboxwid#4\figboxht#5\hscalefactor=1pt\vscalefactor=1pt%
\scale{#3}%
\scale{\globalscaling}%
#1%
\defscaled\DVIhscale\hscalefactor
\defscaled\DVIvscale\vscalefactor
\boxer{\special{psfile=\figuredirectory/#2.ps \DVIspace
		hscale=\DVIhscale\DVIspace 
		vscale=\DVIvscale}}}%
}


%%%%%%%%%%%%%%%%
% The following is from tex/inputs/epsf.tex by Tom Rokicki
% with slight modifications by Jack Snoeyink.
%
%   Written by Tomas Rokicki of Radical Eye Software, 29 Mar 1989.
%
%   Include an ecapsulated postscript graphic.
%   Works by finding the bounding box comment.
%
\newread\Epsffilein
\newif\ifEpsffileok
\newif\ifEpsfbbfound

\newdimen\pspoints
\pspoints=1in
\divide\pspoints by 72


\def\boxeps{%
\@ifnextchar[{\boxepsaux}{\boxepsaux[\relax]}}
\def\boxepsaux[#1]#2#3{%
%
%   The first thing we need to do is to open the
%   PostScript file, if possible.
%
\openin\Epsffilein=\figuredirectory/#2.ps 
\ifeof\Epsffilein\message{I couldn't open \figuredirectory/#2.ps }%
\missingfigure{#2}
\else
%
%   Okay, we got it.  Now we scan lines until we find one
%   that doesn't start with a percentage sign.  We're
%   looking for the bounding box comment.
%
   {\Epsffileoktrue\Epsfbbfoundfalse
    \catcode`\%=11 \catcode`\\=11
    \catcode`\{=11 \catcode`\}=11
    \catcode`\$=11 \catcode`\^=11
    \catcode`\&=11 \catcode`\#=11
    \catcode`\~=11 \catcode`\_=11
    \loop
       \read\Epsffilein to \Epsffileline
       \ifeof\Epsffilein\Epsffileokfalse\else
%
%   Now we check to make sure the first character is a % sign,
%   and that the rest are `%BoundingBox:' if necessary.
%
          \expandafter\Epsfaux\Epsffileline . .\\%
       \fi
   \ifEpsffileok\repeat
   \ifEpsfbbfound
	\figboxht=\Epsfury\pspoints
	\advance\figboxht by-\Epsflly\pspoints
	\figboxwid=\Epsfurx\pspoints
	\advance\figboxwid by-\Epsfllx\pspoints
   \else
	\message{No bounding box comment in \figuredirectory/#2.ps }%
	\figboxwid=2in\figboxht=1in%
   \fi%
   \immediate\closein\Epsffilein
   \hscalefactor=1pt\vscalefactor=1pt%
   \scale{#3}%
   \scale{\globalscaling}%
   #1%
%
   \defscaled\DVIhscale\hscalefactor
   \defscaled\DVIvscale\vscalefactor
%
   \hscalefactor=-\Epsfllx\hscalefactor
   \hscalefactor=1.00375\hscalefactor%	--- 72.27/72 = TeXpoints/PSpoints
   \defscaled\DVIhoffset\hscalefactor
%
   \vscalefactor=-\Epsflly\vscalefactor
   \vscalefactor=1.00375\vscalefactor%	--- 72.27/72 = TeXpoints/PSpoints
   \defscaled\DVIvoffset\vscalefactor
%
   \llboxer{\special{psfile=\figuredirectory/#2.ps \DVIspace
		hoffset=\DVIhoffset\DVIspace
		voffset=\DVIvoffset\DVIspace
                hscale=\DVIhscale\DVIspace 
                vscale=\DVIvscale}} }%
\fi
}%
%
%   We need these for comparison purposes.
%
{\catcode`\%=11 \global\let\Epsfpar=\par
\global\let\Epsfpercent=%\global\def\Epsfbblit{%BoundingBox:}}%
%
%   This is our function that checks for `%BoundingBox:' and grabs the
%   values if they are found.
%
\long\def\Epsfaux#1#2 #3\\{\relax\ifx#1\Epsfpercent
   \def\testit{#2}\ifx\testit\Epsfbblit
      \Epsfsize #3 . . . .\\%
      \global\Epsffileokfalse
      \global\Epsfbbfoundtrue
   \fi\else\ifx#1\Epsfpar\else\global\Epsffileokfalse\fi\fi}%
%
%   Here we grab the values and stuff them in the appropriate definitions.
%
\def\Epsfsize#1 #2 #3 #4 #5\\{\global\def\Epsfllx{#1}\global\def\Epsflly{#2}%
   \global\def\Epsfurx{#3}\global\def\Epsfury{#4}}%




\catcode`\@=12 			% done with with internals

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% For backward compatability
%
% \pic file; height in inches; width in inches; caption\par
% \picsc file; ht (in); wid (in); scale; caption\par
%
% \mpic file; height in inches; width in inches; caption\par
% \mpicsc file; ht (in); wid (in); scale; caption\par
%
%%%%%%%%%%%%%%%%

\def\pic#1;#2;#3;#4\par{\picsc#1;#2;#3;1;#4\par}% file; wd; ht; caption 

\def\picsc#1;#2;#3;#4;#5\par{% file; wd; ht; scale; caption
\figbox[htb]{\boxeps{#1}{#4}%{#2in}{#3in}%
}{figure}{#1}{%
% (#1: #2x#3 sc #4) % 			Uncomment for debugging
#5}}


\def\mpic#1;#2;#3;#4\par{\mpicsc#1;#2;#3;1;#4\par}% file; wd; ht; caption 

\def\mpicsc#1;#2;#3;#4;#5\par{% file; wd; ht; scale; caption
\figbox[l]{\boxeps{#1}{#4}%{#2in}{#3in}%
}{figure}{#1}{%
% (#1: #2x#3 sc #4) % 			Uncomment for debugging
#5}}




